Post-Quantum VRF and its Applications in Future-Proof Blockchain System

A verifiable random function (VRF in short) is a powerful pseudo-random function that provides a non-interactively public verifiable proof for the correctness of its output. Recently, VRFs have found essential applications in blockchain design, such as random beacons and proof-of-stake consensus protocols. To our knowledge, the first generation of blockchain systems used inherently inefficient proof-of-work consensuses, and the research community tried to achieve the same properties by proposing proof-of-stake schemes where resource-intensive proof-of-work is emulated by cryptographic constructions. Unfortunately, those most discussed proof-of-stake consensuses (e.g., Algorand and Ouroborous family) are not future-proof because the building blocks are secure only under the classical hard assumptions; in particular, their designs ignore the advent of quantum computing and its implications. In this paper, we propose a generic compiler to obtain the post-quantum VRF from the simple VRF solution using symmetric-key primitives (e.g., non-interactive zero-knowledge system) with an intrinsic property of quantum-secure. Our novel solution is realized via two efficient zero-knowledge systems ZKBoo and ZKB++, respectively, to validate the compiler correctness. Our proof-of-concept implementation indicates that even today, the overheads introduced by our solution are acceptable in real-world deployments. We also demonstrate potential applications of a quantum-secure VRF, such as quantum-secure decentralized random beacon and lottery-based proof of stake consensus blockchain protocol.

==> body/Picnic.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex

Unique signatures are unique and deterministic. Meaning, that for any given pair of public key and message, there can only be one valid signature. It's not possible to have two different signatures validating against the same public key and message. In this section, we discuss how to design the quantum secure signature with the uniqueness.


\subsection{Post-Quantum Signature}





\par\noindent\textbf{Quantum-secure signature}.
To design a quantum-safe signature scheme, we are inspired by the spirit of hash-based \textit{signature from Fiat-Shamir}~\cite{EC:AABN02} for Schnorr signature. In a nutshell, Schnorr's signature scheme was proven unforgeable only against weak chosen-message attack under the $q$-SDH assumption, where the adversary must submit all of his signature queries in advance of the public key generation.
The detailed is specified as follows.
%Let $\G=\inner{g}$ be a cyclic group of prime order $q$, where $\abs{q}=\secp$, and $\hashH:\set{0, 1}^*\to \Zq$ be a hash function modeled as random oracle.
\begin{itemize}
  \item $(\pk,\sk)\gets\KeyGen(1^{\secp})$. Choose $x\in_R \Zq$, output $(\sk, \pk):=(x, g^x)$.
  \item $\sigma\gets\Sign(\sk, \msgm)$. Choose $r\in_R\Zq$, let $c\gets \hashH(a=g^r\|\msgm)$ and $\pi:=\sk\cdot c+r\pmod{q}$. Output $\sigma:=(\pi, c)$.
  \item $\Vrfy(\pk, \msgm, \sigma)$. Parse $\sigma$ as $(\pi, c)$. Compute $c'\gets \hashH(\pk^{-c}\cdot g^{\pi}\|\msgm)$. Output $c=c'$.
\end{itemize}
To summarize,
we consider a (weakly complete) quantum secure identification protocol (or $\Sigma$ protocol) $P$ and $V$, Fiat-Shamir approach gives a post-quantum,
the methodology of the signature from Fiat-Shamir is as follows.
\begin{itemize}
  \item $\Gen(1^{\secp})$, $\sk:=\Fishsrt \gets R$, and $\vk:=\Fishpk=\OWF(\sk)$.
  \item $\Sign(\sk,\msg)$, it takes as input the $\sk$ and a message $\msg$, and it generates
  \begin{itemize}
    \item $(\aaa, \stt)\gets \Com(\sk:=\Fishsrt, \opstr:=\rand)$,

    \item $c\gets \textcolor{black}{\hashH(\aaa\|\msg)}$, where $\|$  denotes concatenation.
    \item and it generates $\zzz\gets\Prove(\sk:=\Fishsrt,\stt, \ccc)$.
  \end{itemize}
  If $\zzz$ is not valid, it runs another round. It keeps running until $\zzz$ is valid. Finally it return the signature $\sigma:=(\aaa, \ccc, \zzz)$.

  \item   $\Vrfy(\vk, \msg, \sigma)$, it rejects if there has $\Vrfy(\vk:=y, \msg, (\aaa,\zzz,\textcolor{black}{ \hashH(\msg \| \aaa)}))=0$.
\end{itemize}


In short, the OWF function family $\set{f_k}_{k\in K_{\secp}}$ used for key generation in both signature schemesthe public key is an image $y=f(x)$ of a one-way function $f$ and secret key $x$, and a signature is a non-interactive zero-knowledge proof $\zkproof$ of $x$, that incorporates a message to be signed.

\begin{theorem}[\cite{C:LiuZha19}]
For a weakly complete secure quantum identification protocol with unpredictable commitment, Fiat-Shamir heuristic gives a secure post-quantum digital signature in the quantum random oracle model.
\end{theorem}




%\begin{itemize}
%  \item $\Gen$ $\sk:=\Fishsrt \gets R$, and $\vk:=\Fishpk=\OWF(\Fishsrt)$
%  \item $\Sign(\sk,\msg)$
%  \begin{itemize}
%    \item sample a randomness $\strrand:=\rand$
%    \item $\aaa=\Com(\sk:=\Fishsrt, \strrand:=\rand)$,
%    \item $\zzz=\Open(\rand,\Fishsrt,\textcolor{red}{\hashH(\msg, \aaa)})$, (\ie, response).
%    \item output signature $\sigma:=\zkproof:=(\aaa, \zzz)$
%  \end{itemize}
%  \item $\Vrfy(\vk, \msg, \sigma)$ reject if $\Vrfy((\aaa,\zzz),\textcolor{red}{ \hashH(\msg, \aaa)})=0$
%\end{itemize}




Very recently, Picnic signature is proposed recently by Chase \etal~\cite{CCS:CDGORR17} and designed to provide security against attacks by quantum computers, in addition to attacks by classical computers, where the security is primarily based on the existence of a zero-knowledge proof system $\ZKBpp$, and symmetric key primitives like one-way hash functions and block ciphers, and the signature size strongly depends on the number of multiplications in the circuit describing that one-way function. The building blocks does not require number-theoretic, or structured hardness assumptions. The generic description of  Picnic signature is as depicted as follows. % in the Figure~\ref{fig:Fish-signature.}.

%In general, Picnic is similar to Schnorr's signature scheme, and the Thus, following the methodology Schnorr signature and quantum-secure signature, the Picnic signature is specified as follows.



\begin{itemize}
\item $\Gen(1^{\secp})$.
\begin{enumerate}
  \item Choose a secret key $\Fishsrt\gets \calD$ and a random key $\rkey\gets \calK$ for the pseudo-random function $\hashF$, then compute $\Fishpk=\hashF_{\rkey}(\Fishsrt)$.
  \item Set $\pk\gets \Fishpk$, then return $\sk\gets (\Fishpk, \Fishsrt)$.
\end{enumerate}

\item $\Sign(\sk, \msg)$.
\begin{enumerate}
  \item Parse the secret key $\sk$ as two partes \ie, $\Fishsrt$ and $\Fishpk$.

  \item Then compute the zero-knowledge proof (\ie, $\Sigma$-protocol)
  $\zkproof:=(\aaa, \zzz)\gets \Prove_{\hashH}(1^{\secp}, (\Fishpk, \msg), \Fishsrt)$,

where the statement of $\Sigma$-protocol is $\strstmt:=(\Fishpk, \msg)$ and the witness is $\strwits:=\Fishsrt$.

  \item Last return $\Fishsign \gets \zkproof$, where internally the challenge is computed as $\strchlg:=\chlg\gets \hashH(\aaa, \msg)$.
\end{enumerate}



\item $\Vrfy(\pk,\msg, \Fishsign)$.
\begin{enumerate}
  \item Parse $\pk$ as $\Fishpk$, and $\Fishsign$ as $\zkproof = (\aaa, \zzz)$.
  \item  Return $1$ if the following holds, and 0 otherwise:
    $
      \Verify_{\hashH}(1^{\secp}, (\Fishpk,\msg), \zkproof)=1
    $
    where internally the challenge is computed as $\strchlg:=\chlg\gets \hashH(\aaa, \msg)$.
\end{enumerate}
\end{itemize}
Here we remark that, in Picnic, $\Prove$ is implemented with $\ZKBpp$, but the usage of Unruh's transform~\cite{EC:Unruh15} is to achieve post-quantum security in the Quantum Random Oracle Model (QROM). For the generation of the proof, the methodology of $\ZKBoo$~\cite{USENIX:GiaMadOrl16}, $\ZKBpp$~\cite{CCS:CDGORR17}, and Ligero~\cite{CCS:AHIV17} can be leveraged, which are efficient non-interactive zero-knowledge proofs of knowledge (NIZKPoKs) for Boolean circuits based on symmetric-key primitives alone, using the ``MPC-in-the-head'' paradigm of Ishai \etal~\cite{STOC:IKOS07}.
However, Picnic signature cannot provide the uniqueness property.
%Here we remark that in both schemes (\eg, Fish and Picnic). $\Prove$ is implemented with $\ZKBpp$, in Fish it is made non-interactive with Fiat-Shamir transformation, while in Picnic, using Unruh's transform~\cite{EC:Unruh15}.
%\zlidel{The OWF function family $\set{f_k}_{k\in K_{\secp}}$ used for key generation in both signature schemes is instantiated with LowMC. Concretely, we instantiate $\set{f_k}$ using a block cipher with $f_k(x):=\Enc(k,x)$, where $\Enc(k,x)$ denotes the LowMC encryption of a single block $k\in \set{0,1}^{\secp}$ with respect to key $x\in\set{0,1}^{\secp}$.}
%\par\noindent\textbf{Unique signature from classical assumption}.



\subsection{Quantum-Safe Signature with Uniqueness}
\par\noindent\textbf{Unique signature from non-quantum resistant assumptions}.
Boneh-Lynn-Shacham (BLS) signature is an representative unique signature scheme. Let $\G=\inner{g}$ be a cyclic group of prime order $q$, where $\abs{q}=\secp$, and $\hashH:\set{0, 1}^*\to \Zq$ be a hash function modeled as random oracle. Given the private key $x$, and some message $\msgm$, the signer computes the signature by hashing the bit-string $\msgm$, as $h=\hashH(\msgm)$, and output the signature $\sigma=h^{x}$. During the verification phase, given a signature $\sigma$ and a public key $g^{x}$, the verifier verifies that $e(\sigma, g)=e(\hashH(\msgm), g^{x})$. However, BLS signature cannot guarantee the security during the quantum era.





In order to integrate the uniqueness property into the quantum-secure signature scheme, we are walking this research line of Goldwasser and Ostrovsky~\cite{C:GolOst92} who introduced the notation of a unique signature.  Then we develop a new quantum-safe signature armed with a zero-knowledge proof for arithmetic circuits and $\OWF$. The main goal of our construction is designed to provide a quantum-safe signature with uniqueness properties compared with the previous hash-based signature.
The detailed constriction is depicted in Figure~\ref{fig:our-signature}.






















\mybox{Generic description our unique signature.}{white!40}{white!10}{
\small
%\scriptsize
%\smallskip
%\vspace{-5pt}
\begin{itemize}
\item $\uKeyGen(1^{\secp})$.
\begin{enumerate}
  \item Choose a secret key $\Oursk \gets \calD$ and a random key $\rkey\gets \calK$ for the pseudo-random function $\hashF$, then compute $\Ourpk=\hashF_{\rkey}(\Oursk)$.
  \item Set $\pk\gets \Ourpk$, then return $\sk \gets (\Ourpk, \Oursk)$.
\end{enumerate}

\item $\uSign(\sk, \msg)$.
\begin{enumerate}
  \item Parse the secret key $\sk$ as two partes \ie, $\Oursk$ and $\Ourpk$.
  \item Compute and return
  \begin{equation*}
    \Oursign_0 \gets \hashH(\sk:=(\Ourpk, \Oursk), \msg).
  \end{equation*}


  \item Then compute the zero-knowledge proof
      \begin{enumerate}
        \item validate and assert $\Ourpk\overset{?}{=}\hashF_{\rkey}(\Oursk) $;
        \item validate and assert $\Oursign_0\overset{?}{=}\hashH(\sk,\msg)$;
        \item if the validations pass, then return the proof that is computation integrity proof
      \begin{equation*}
        \zkproof:=(\aaa, \zzz)\gets \Prove_{\hashH}(1^{\secp}, (\Ourpk, {\Oursign_0}), \Oursk),
      \end{equation*}
where the statement of ZKP is $\strstmt:=(\Ourpk, {\Oursign_0})$ and the witness is $\strwits:=\Oursk$.
      \end{enumerate}





  \item Last return the signature $\Oursign \gets (\Oursign_0, \zkproof)$, where internally the challenge is computed as $\strchlg:=\chlg\gets \hashH(\aaa, {\Oursign_0})$.
\end{enumerate}



\item $\uVrfy(\pk,\msg, \Oursign)$.
\begin{enumerate}
  \item Parse $\pk$ as $\Ourpk$, and $\Oursign$ as $\Oursign_0$ and $\zkproof = (\aaa, \zzz)$.
  \item  Return $1$ if the following holds, and 0 otherwise:
    \begin{equation*}
      \Verify_{\hashH}(1^{\secp}, (\Ourpk, {\Oursign_0}), \zkproof)=1
    \end{equation*}
    where internally the challenge is computed as $\strchlg:=\chlg\gets \hashH(\aaa, {\Oursign_0})$.
\end{enumerate}
\end{itemize}


}{Generic description our unique signature.~\label{fig:our-signature}}

%%
For a validly generated public key, each input $\msg$ to the signature with the uniqueness has at most one hash output $\Oursign$ that can be proven to be correct. In other words, regarding uniqueness of $\Oursign$, there do not exist values $(\pk,\msgm,\Oursign_1, \Oursign_2)$ such that $\Vrfy(\pk,\msg, \Oursign_1)=\Vrfy(\pk,\msg, \Oursign_2)=1$. Further, the ZKP is used to prove knowledge of $\rkey$ so that $\Ourpk=\hashF_{\rkey}(\Oursk)$. Similarly, in our construction, $\Sigma$ protocol proves that the secret $\Oursk$ used to compute the signature $\Oursign$ is pre-image of $\Ourpk$ (without revealing $\Oursk$), so effectively we have a unique signature functionality.
Formally, the computational trusted uniqueness definition~\ref{def:uniqueness} is as follows.

\par\noindent\textbf{Consistency}. If the signature $\sigma$ is well-formed, then the verification returns $1$. Our scheme is based on Picnic signature and Schnorr's signature is used for reference. Thus, we ignore the rigorous analysis. Further, to our knowledge, a unique signature must be a strongly unforgeable signature\footnote{But a strongly unforgeable signature is not necessarily a unique signature}.





\par\noindent\textbf{Uniqueness}. Informally, if there are two signatures $(\sigma_1, \sigma_2)$ for the same message $\msgm$ under a key pair $(\pk,\sk)$, then it is a unique signature iff $\sigma_1=\sigma_2$.

\begin{lemma}[Computational Uniqueness, Adopted from~\cite{EPRINT:GNPR16}]\label{def:uniqueness}
A VRF satisfies $(t,\epsilon)$-trusted uniqueness if for all adversaries $\Adv$ whose running and description size are bounded by $t$, for a random validly chosen key pair $(\pk,\sk)\gets \KeyGen(1^{\secp})$, then there exists
\begin{multline*}
%\footnotesize
\small
\left| \Pr\left[
       \begin{array}{c}
    \beta_1 \neq \beta_2 \; \wedge 1=\\
    \Vrfy(\pk,\alpha,\beta_1,\pi_1)
    \end{array}
      \middle|
        \begin{array}{c}
  (\pk,\sk)\gets \KeyGen(1^{\lambda});\\
  (\alpha,\beta_1, \pi_1)\gets \Adv(\pk,\sk);\\
  (\beta_2,\pi_2)\gets\Prove(\sk, \alpha)
         \end{array}
        \right] \right|
          \leq \negl(\lambda).
\end{multline*}
\end{lemma}

%\begin{equation*}
%      \left| \Pr\left[
%       \begin{array}{c}
%    \beta_1 \neq \beta_2 \; \wedge 1=\\
%    \Vrfy(\pk,\alpha,\beta_1,\pi_1)
%
%    \end{array}
%      \middle|
%        \begin{array}{c}
%  (\pk,\sk)\gets \KeyGen(1^{\lambda});\\
%  (\alpha,\beta_1, \pi_1)\gets \Adv(\pk,\sk);\\
%  (\beta_2,\pi_2)\gets\Prove(\sk, \alpha)
%         \end{array}
%        \right] \right|\\
%          \leq \negl(\lambda).
%\end{equation*}




\noindent\textbf{Sketched Proof}. The proof is by contradiction. Suppose an adversary, given the secret key $\sk:=(\Ourpk, \Oursk)$ who can come up with some output
two signatures $(\Oursign_1, \Oursign_2)$ for the same message $\msgm$ under a secret-public key pair $(\sk:=(\pk,\Oursk), \pk:=\hashF_{\rkey}(\Oursk))$, then we have
\begin{equation}\label{eq:unique}
  \Verify_{\hashH}(1^{\secp}, (\Ourpk, {\Oursign_{1,0}}), \zkproof_1)=1=
  \Verify_{\hashH}(1^{\secp}, (\Ourpk, {\Oursign_{2,0}}), \zkproof_2)
\end{equation}
where $\zkproof_i:=(\aaa, \zzz)\gets \Prove_{\hashH}(1^{\secp}, (\Ourpk, {\Oursign_{i,0}}), \Oursk)$ for $i=1,2$. Because $\Oursign_i$ is from two parts, one is $\Oursign_{i,0}=\hashH(\sk,\msg)$ and another is $\zkproof_i:=(\aaa, \zzz)\gets \Prove_{\hashH}(1^{\secp}, (\Ourpk=\hashF_{\rkey}(\Oursk), {\Oursign_{i,0}}), \Oursk)$. Thus, if the Eq.~(\ref{eq:unique}) holds, it must be $\Oursign_{1,0}=\Oursign_{2,0}$ and $\zkproof_1=\zkproof_2$ unless $\pk:=\Ourpk$ is not obtained by $\hashF_{\rkey}(\Oursk)$.











\draft{

In a word, zero-knowledge protocol is to prove knowledge of $sk$ so that
\zli{input the new works here}

\zli{OWF Selection?}

%\subsubsection{Signature form Fiat-Shamir}

%Inspired by the remarks of Algorand from unique signature to VRFs~\cite{Algorand16}, and the relationship between unique signature and VRFs discussed by Lysyanskaya~\cite{C:Lysyanskaya02}.


%\noindent\textbf{Informal: Signature form Fiat-Shamir}
%
%\begin{figure}[ht]
%  \centering
%  \includegraphics[width=0.6\textwidth]{{Fiat-Shamir-Heuristic.PNG}}
%  \vspace{-10pt}
%  \caption{Fiat-Shamir-Heuristic}\label{fig:Fiat-Shamir-Heuristic}
%\end{figure}


\mybox{Generic description the Fish and Picnic signature.}{white!40}{white!10}{
\small
%\scriptsize
%\smallskip
%\vspace{-5pt}
\begin{itemize}
\item $\Gen(1^{\secp})$.
\begin{enumerate}
  \item Choose a secret key $\Fishsrt\gets \calD$ and a random key $\rkey\gets \calK$ for the pseudo-random function $\hashF$, then compute $\Fishpk=\hashF_{\rkey}(\Fishsrt)$.
  \item Set $\pk\gets \Fishpk$, then return $\sk\gets (\Fishpk, \Fishsrt)$.
\end{enumerate}

\item $\Sign(\sk, \msg)$.
\begin{enumerate}
  \item Parse the secret key $\sk$ as two partes \ie, $\Fishsrt$ and $\Fishpk$.

  \item Then compute the zero-knowledge proof (\ie, $\Sigma$-protocol)
      \begin{equation*}
        \zkproof:=(\aaa, \zzz)\gets \Prove_{\hashH}(1^{\secp}, (\Fishpk, \msg), \Fishsrt),
      \end{equation*}
where the statement of $\Sigma$-protocol is $\strstmt:=(\Fishpk, \msg)$ and the witness is $\strwits:=\Fishsrt$.

  \item Last return $\Fishsign \gets \zkproof$, where internally the challenge is computed as $\strchlg:=\chlg\gets \hashH(\aaa, \msg)$.
\end{enumerate}



\item $\Vrfy(\pk,\msg, \Fishsign)$.
\begin{enumerate}
  \item Parse $\pk$ as $\Fishpk$, and $\Fishsign$ as $\zkproof = (\aaa, \zzz)$.
  \item  Return $1$ if the following holds, and 0 otherwise:
    \begin{equation*}
      \Verify_{\hashH}(1^{\secp}, (\Fishpk,\msg), \zkproof)=1
    \end{equation*}
    where internally the challenge is computed as $\strchlg:=\chlg\gets \hashH(\aaa, \msg)$.
\end{enumerate}
\end{itemize}

Here we remark that in both schemes (\eg, Fish and Picnic). $\Prove$ is implemented with $\ZKBpp$, in Fish it is made non-interactive with Fiat-Shamir transformation, while in Picnic, using Unruh's transform~\cite{EC:Unruh15}. In Picnic, $\Prove$ is implemented with $\ZKBpp$, but the usage of Unruh's transform is to achieve post-quantum security in the Quantum Random Oracle Model (QROM).
% namely  Honest-verifier Zero-knowledge.Fish: building upon Fiat-Shamir.

}{Generic description the Fish and Picnic signature.~\label{fig:Fish-signature.}}
}




==> body/PoS-structure.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex
%%%
%%%
\begin{figure}[ht]
\begin{threeparttable}
%\scalebox{.5}
\resizebox{.98\linewidth}{!}{
\begin{tikzpicture}[%
    every node/.style={
        font=\scriptsize,
        % Better alignment, see https://tex.stackexchange.com/questions/315075
        text height=1ex,
        text depth=.25ex,
    },
    Line/.style = {-angle 90, shorten >=2pt},
    inner sep=0.5mm,
    nofill/.style={circle,draw=cyan},
    filled/.style={circle, draw=cyan, fill=cyan},
    ys/.style = {yshift=#1}
]


% draw horizontal line
%\draw[->] (0,0) -- (10,0);
% place axis labels
%\node[anchor=north] at (3,0) {};
%\node[anchor=north] at (4,0) {};
%\node[anchor=north] at (5,0) {};
%\node[anchor=north] at (6,0) {};
%\node[anchor=north] at (8.5,0) {};

\linespread{1}
\coordinate (a) at (0mm,0);
\coordinate[right=13mm of a]    (b);
\coordinate[right=13mm of b]    (c);
\coordinate[right=13mm of c]    (d);
\coordinate[right=13mm of d]    (e);
\coordinate[right=13mm of e]    (f);
\coordinate[right=13mm of f]    (g);
\coordinate[right=13mm of g]    (h);
%\coordinate[right=18mm of h]    (i);
%\coordinate[right=18mm of i]    (j);
%\coordinate[right=18mm of j]    (k);
%\coordinate[right=18mm of k]    (l);
% draw horizontal line
\draw[Line,-latex,->] (a)--(h) node [below right]{Time(Slot)};
% draw vertical lines
\foreach \x in {0,1.3,...,9.1}{
    \draw (\x cm,3pt) -- (\x cm,0pt);
}
\draw(a) -- node[below,yshift=-2mm] {~slot~0}  (b)
                -- node[below,yshift=-2mm] {~slot~1}  (c)
                -- node[below,yshift=-2mm] {~slot~2}  (d)
                -- node[below,yshift=-2mm] {~$\cdots$~}  (e)
                -- node[below,yshift=-2mm] {~slot~N}  (f)
                -- node[below,yshift=-2mm] {~slot~0}(g)
                -- node[below,yshift=-2mm] {~slot~1}(h);

%
%                -- node[below,yshift=-2mm] {~slot~2}(i)
%                -- node[below,yshift=-2mm] {~$\cdots$~} (j);
%                -- node[below,yshift=-2mm] {~slot~N} (k);
%                -- node[below,yshift=-2mm] {~slot~N} (l);

\draw(a) -- node[above,yshift=2mm] {SL~0}  (b)
                -- node[above,yshift=2mm] {SL~1}  (c)
                -- node[above,yshift=2mm] {SL~2}  (d)
                -- node[above,yshift=2mm] {~$\cdots$~}  (e)
                -- node[above,yshift=2mm] {SL~N}  (f)
                -- node[above,yshift=2mm] {SL~0}(g)
                -- node[above,yshift=2mm] {SL~1}(h);

%% draw scale above
\coordinate (a0) at (0mm,-9mm);
\coordinate[right=13mm of a0]    (b0);
\coordinate[right=13mm of b0]    (c0);
\coordinate[right=13mm of c0]    (d0);
\coordinate[right=13mm of d0]    (e0);
\coordinate[right=13mm of e0]    (f0);
\coordinate[right=13mm of f0]    (g0);
\coordinate[right=13mm of g0]    (h0);
\coordinate[right=13mm of h0]    (i0);
%\coordinate[right=10mm of i0]    (j0);
\draw[myRed,Line,dashed,thick,-latex,->] (a0)--(h0) node [below right, yshift=-2mm]{Time(Epoch)};
%\draw[myRed,Line,dashed,thick,-latex] (-0.1,-0.5) -- (8.9,-0.5);
% draw vertical lines
\draw (a0) node[below, red]{} node[above] {} -- ++(0, 60pt) ;
\draw (b0) node[above, red] {} -- ++(0, 3pt);
\draw (c0) node[above, red] {} -- ++(0, 3pt) ;
\draw (d0) node[above, red] {} -- ++(0, 3pt) ;
\draw (e0) node[above, red] {} -- ++(0, 3pt) ;
\draw (f0) node [below, red]{} node[above] {} -- ++(0, 60pt) ;
% draw curly braces and add their labels
\draw[decorate,decoration={brace,amplitude=5pt,mirror,raise=4pt},yshift=0pt] (a0) -- (f0)
    node[anchor=south,midway,below=6pt,  yshift=-2mm] {Epoch~M};



% draw scale above
\node [rectangle,draw=blue,thick, above right=10mm and 3mm of a] (a1) {BC~0};
\node [rectangle,draw=blue,thick, right=9mm of a1] (b1) {BC~1};
\node [rectangle,draw=blue,thick, right=8mm of b1] (c1) {BC~2};
\node [right=7mm of c1] (d1) {$\cdots$};
\node [rectangle,draw=blue,thick, right=7mm of d1] (e1) {BC~N};

\draw[very thick,dashed,blue, ->] (b1.west) to (a1.east);
\draw[very thick,dashed,blue, ->] (c1.west) to (b1.east);
\draw[very thick,dashed,blue, ->] (d1.west) to (c1.east);
\draw[very thick,dashed,blue, ->] (e1.west) to (d1.east);


\node [above right=9mm and 4mm of a1] (a2) {};

\draw[thick,->] (a2) to node[midway,sloped,left,rotate=296]{$f\cdot \rltstake_i$} (a1) ;
\end{tikzpicture}
}
\begin{tablenotes}
    \footnotesize

  \item[-] Let $f$ be the probability that an honest party holding all the stake will be selected to be a (slot) leader for a given slot.
  \item[-] $f\cdot \rltstake_i$ is the expected number of honest stakeholders that are qualified in a round to extend the longest chain, where $\rltstake_i$ implies the relative stakes quotas of the honest party.
      \end{tablenotes}

\end{threeparttable}

\caption{Proof of Stake Cryptographic Puzzle}\label{fig:PoS}
\end{figure}
%






==> body/PoSanalysis.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex


%
%\par\noindent\textbf{Observations}.
%An observation is that some related classical PoS works, such as snow white~\cite{EPRINT:BenPasShi16a,FC:DaiPasShi19}, iChang~\cite{EPRINT:FanZho17}, Algorand~\cite{Algorand16} with follow-up works~\cite{SOSP:GHMVZ17,EPRINT:CGMV18} and DFINITY~\cite{DFINITY}, are with similar block structures, and the core of cryptographic puzzles (either PoW or PoS) is same to in a way. In particular,
%
%\par\noindent{\textbf{Snow White}.}
%%
%In snow white, Bentov, Pass, and Shi~\cite{EPRINT:BenPasShi16a} and its follow-up result~\cite{FC:DaiPasShi19} define a valid block and a valid blockchain as a tuple
%$$\blockB:=(\prehash, \txs, \strtime, \nonce, \pk, \sigma, \hash).$$
%Notably, the block $\blockB$ is a valid block iff 
%\begin{enumerate*}
%  \item $\Sigma.\Vrfy_{\pk,\sid}((\prehash, \txs, \strtime, \nonce );\sigma)=1$,
%  \item and $\hash=\hfuncH(\prehash,\txs, \strtime, \nonce, \pk, \sigma)$.
%\end{enumerate*}
%
%
%
%
%
%
%
%\par\noindent{\textbf{iChang}.}
%%
%iChang is proposed by Fan and Zhou~\cite{EPRINT:FanZho17}. They require if the PoS-player is chosen, then the following hash inequality holds:
%\begin{equation*}
%  \hfuncH(\hash(\blockB_i),\strround, \pk, \sigma)< \target
%\end{equation*}
%where $\sigma:=\uSign_{\sk}(\hvalH_i, \strround)$ is the unique signature, and $\hvalH_i:=\hash(\blockB_i)$. Thus, the new block $\blockB_{i+1}$ is defined as
%\begin{equation*}
%  \blockB_{i+1}:= \inner{\hvalH_i, \strround, \pk, \sigma}.
%\end{equation*}
%
%\par\noindent{\textbf{Algorand}.}
%Algorand is introduced by Micali~\cite{Algorand16} using the \VRF.
%%
%%\noindent{\textbf{The Idealized Public Ledger.}}
%Algorand tries to mimic the following payment system, based on an idealized public ledger.
%%\noindent\text{The Initial Status.}
%In a nutshell, money is associated with individual public keys (privately generated and
%owned by users). Letting $\pk_1, \cdots, \pk_j$ be the initial public keys and $a_1, \cdots, a_j$ their respective initial amounts of money units, then the initial status is
%\begin{equation*}
%  \state_0=(\pk_1,a_1), (\pk_2,a_2), \cdots, (\pk_j, a_j).
%\end{equation*}
%Furthermore, the block structure is as follow,
%\begin{equation*}
%  \blockB_\roundr =(\roundr, \pay_\roundr, \Sign_i(Q_{\roundr-1}), \hashH(\blockB_{r-1})).
%\end{equation*}
%In Algorand, the block $\blockB_r$ corresponding to a round $r$ specifies: $r$ itself; the set of payments of round $r$, $\pay_r$; a quantity $Q_r$, to be explained, and the hash of the previous block, $\hfuncH({\blockB}_{(r-1)})$.
%
%Thus, starting from some fixed block $\blockB$, we have a traditional blockchain:
%$
%  \blockB^1=(1,\pay^1,Q^0, \hfuncH(\blockB^0)), \blockB^2=(2,\pay^2,Q^1, \hfuncH(\blockB^1)), \blockB^3=(3,\pay^3,Q^2, \hfuncH(\blockB^2)), \cdots
%$.

%
%
%\noindent\text{Payments.}
%Let $\pk$ be a public key currently having $a \leq 0$ money units, $\pk'$ another public
%key, and $a'$ a non-negative number no greater than $a$. Then, a (valid) payment $\pay$ is a digital signature, relative to $\pk$, specifying the transfer of $a'$ monetary units from $\pk$ to $\pk'$, together with some additional information. In symbols,
%\begin{equation*}
%  \pay := \sigma=\strSig_{\pk}(\pk, \pk', a', I, \hfuncH(I)),
%\end{equation*}
%where $I$ represents any additional information deemed useful but not sensitive (e.g., time
%information and a payment identifier),  and any additional information deemed sensitive (\eg,
%the reason for the payment, possibly the identities of the owners of $\pk$ and the $\pk'$, and so on). We refer to $\pk$ (or its owner) as the payer, to each $\pk'$ (or its owner) as a payee, and to $a'$ as the amount of the payment $\pay$.
%
%
%
%\noindent\text{The Magic Ledger.}
%In the Idealized System, all payments are valid and appear in a tamper-proof list $L$ of sets of payments ``posted on the sky'' for everyone to see:
%%
% \begin{equation*}
%   L=\pay^1,\pay^2,\cdots
% \end{equation*}
%
%Each block $\pay^{r+1}$ consists of the set of all payments made since the appearance of block
%$\pay^{r}$. In the ideal system, a new block appears after a fixed (or finite) amount of time.
%

%
%
%
%\noindent\text{Blocks and Proven Blocks.}
%In Algorand, the block $\blockB^r$ corresponding to a round $r$ specifies: $r$ itself; the set of payments of round $r$, $\pay^r$; a quantity $Q^r$, to be explained, and the hash of the previous block, $\hfuncH({\blockB}^{(r-1)})$. In a nutshell, the block structure is as follow,
%\begin{equation*}
%  \blockB_\roundr =(\roundr, \pay_\roundr, \Sign_i(Q_{\roundr-1}), \hashH(\blockB_{r-1})).
%\end{equation*}
%
%
%Thus, starting from some fixed block $\blockB$, we have a traditional blockchain:
%$
%  \blockB^1=(1,\pay^1,Q^0, \hfuncH(\blockB^0)), \blockB^2=(2,\pay^2,Q^1, \hfuncH(\blockB^1)), \blockB^3=(3,\pay^3,Q^2, \hfuncH(\blockB^2)), \cdots
%$.
%
%
%Notably, in iChang protocol~\cite{EPRINT:FanZho17}, Fan and Zhou mimic the PoW consensus protocol and adopt the round $\strround$ notation to analysis the players whether can find a solution (\ie, PoS block) with probability $p$ for honest player in every round, instead of the method of epoch and slot in Ouroboros series works~\cite{EC:GarKiaLeo15,C:KRDO17,CCS:BGKRZ18,EPRINT:KKKZ18}. But, essentially, the notation of round $\strround$ in ~\cite{EPRINT:FanZho17} is same as the notation $\slot$ in Ouroboros~\cite{EC:GarKiaLeo15}. Below, in our protocol, inspired by the iChang~\cite{EPRINT:FanZho17} and Ouroboros~\cite{EC:GarKiaLeo15}, if the PoS-player is chosen, then the following hash inequality holds
%\begin{equation*}
%  \hashH(\state_i:=h_{i-1}=\hashH(\blockB_{i-1}), \data_i, \slot_i, \pk_i, \sigma_i)< \stake_i \cdot\tgtT,
%\end{equation*}
%%
%where a signature $\sigma=\uSign_{\sk_i}(\state_i:=\hashH(\blockB_{i-1}),\data_i,\slot_i)$ computed under $\sk_i$ corresponding to the stakeholder $U_i$ generating the block, for convenience, we abbreviate the signature to $\sigma:=\uSign_{\sk}(h_i, \slot_i)$ for $h_i=\hashH(\blockB_{i-1})$. In this setting, the new block $\blockB_i$ is defined as  the following block structure:
%\begin{eqnarray*}
%% \nonumber to remove numbering (before each equation)
%  \blockB_i &=& (\state_i, \data_i, \slot_i, \pk, \sigma_i) \\
%   &=& (\state_i:=h_{i-1}=\hashH(\blockB_{i-1}), \data_i, \slot_i, \pk, \sigma_i).
%\end{eqnarray*}


%\begin{equation*}
%  \blockB_i=(\state_i, \data_i, \slot_i, \pk, \sigma_i):=(\state_i:=h_{i-1}=\hashH(\blockB_{i-1}), \data_i, \slot_i, \pk, \sigma_i).
%\end{equation*}


\subsection{Overview of PoS Protocol}

The informal description of our designed post-quantum PoS protocol has been illustrated in the Introduction: assume the longest post-quantum for a PoS-player consists of the following ordered post-quantum block, $\blockB_1, \blockB_2, \cdots, \blockB_i$. In our setting, we let round denote the current time (or round number).
%




{
\par\noindent\textbf{Blockchain Protocol}.
To describe the post-quantum PoS protocol, we follow the framework of blockchain-based PoS presented by~Scafuro, Siniscalchi, and Visconti~\cite{PKC:ScaSinVis19} which followed the verbatim from~\cite{EC:PasSeeshe17,TCC:GoyGoy17}. In more detail, a blockchain protocol consists of 4 polynomial-time algorithms
$$
(\UpdateState, \GetRecords, \Broadcast, \GetHash).
$$
\begin{itemize}
  \item $\bar{\state}\gets\UpdateState(1^\secp, \state)$: it takes as input the security parameter $\secp$, state $\state$ and outputs the update state $\bar{\state}$. More concretely,  before executing the cryptographic PoS puzzle, each stakeholder $U_i$ in the setting first to initialize his own state $\state_i:=h_{i-1}=\hashH(\blockB_{i-1})$.












  \item $\blockB\gets \GetRecords(1^\secp, \bar{\state})$: it takes as input the security parameter $\secp$ and state $\bar{\state}$. It outputs the longest ordered sequence of valid blocks $\blockB$ (or simply blockchain) contained in the state variable, where each block in the chain itself contains an unordered sequence of records messages. More concretely, depending on our settings, if the stakeholder $U_i$ holds at least 2\% of total stakes, then he will automatically become the elector $E_i$. Then, the elector $E_i$ proceeds the algorithm as follows:

      \begin{enumerate}
        \item the elector $E_i$ is enable to become the leader who has the right to create the next block with the quota stake $\stake_i$ and the probability $\probld_i = {\stake_i}/{\sum_{k=1}^n \stake_k}$ for $i\in [N]$.


        \item next, each elector $E_i$ begins to execute his quantum-resistant signature scheme       $\sigma_i=\uSign_{\sk_i}(\state_i:=\hashH(\blockB_{i-1}),\data_i,\slot_i)$ under $\sk_i$ corresponding to the elector $E_i$ generating the block.

        \item then, each elector is struggling to become the next block creator by testing whether satisfies the following inequality, \ie, cryptographic PoS puzzle
\begin{equation}\label{eq:pos}
  \hashH(\state_i:=\hashH(\blockB_{i-1}), \data_i, \slot_i, \pk_i, \sigma_i)< \stake_i \cdot\tgtT.
\end{equation}
where the target value $\tgtT$ is fixed and ``posted on the sky'', but different elector $E_i$ has different $\stake_i$, thus, if the elector who has more stakes, then $\stake_i \cdot\tgtT$ is larger and he is more likely to be the creator for the next block.


     \item  if the elector $E_i$ passes the inequality~\ref{eq:pos} firstly, then he becomes the leader $\leader_i $ and is entitled to the new coming block $\blockB$.




      \end{enumerate}










  \item $\Broadcast(1^\secp, \record)$: it takes as input a security parameter $\secp$ and a message $\msg$, and broadcasts the message over the network to all nodes executing the blockchain protocol. It does not give any output.


  \item $\GetHash(1^\secp, \blockB)$: it takes as input a security parameter $1^{\secp}$ and a blockchain $\blockB$, and outputs the description of a collision-resistant hash function $\hfuncH(\cdot)$ publicly available in $\blockB$.
\end{itemize}
}

%\subsection{Quantum-Safe PoS Consensus}

\par\noindent\textbf{Realization of PoS}.
Following the approach of Algorand~\cite{Algorand16} and Ouroboros~\cite{C:KRDO17}, we use our constructed quantum-resistant \VRF to elect a new committee,  and we assume the PoS-player holds the signing-verification key pair $(\vsk, \vpk)$ for \VRF. When a node is chosen to validate the next block, it will check and make sure that all the transactions within that block are valid. If everything is as it should be the node will Validate the block, and add it to the chain. The node then receives the fees that are associated with the block.




%In this work, we follow the methodology of iChang opposed by Fan and Zhou~\cite{EPRINT:FanZho17}. In a nutshell, we consider a unique post-quantum signature scheme $(\uKeyGen, \uKeyVrfy, \uSign, \uVrfy)$, and assume the PoS-player holds the signing-verification key pair $(\sk, \pk)$.
%In a nutshell, our proposed quantum-resistant PoS follows the methodology of iChang~\cite{EPRINT:FanZho17} whose core work is inspired by Algorand~\cite{Algorand16} and Ouroboros~\cite{C:KRDO17}, thus,








%Pass, Seeman, and Shelat~\cite{EC:PasSeeshe17}, Goyal, and Goyal~\cite{TCC:GoyGoy17}
















Below, we detail the security for Subsection~\ref{subsec:secruityanalysis}. 
\subsection{Security Analysis}\label{subsec:secruityanalysis}

To analyze our proposed quantum-resistant PoS consensus protocol, for convenience, we provide a weaker proof strategy for three main properties, \eg, chain growth, chain quality, and common prefix (or chain consistency). In particular, we adopt the same strategy of~\cite{EC:GarKiaLeo15} to analyze chain growth and chain quality while we adopt the same strategy of~\cite{C:KRDO17} to prove common prefix due to the issues of blockchain fork.






\par\noindent\textbf{Notations}.
For convenience, the analysis is in the ``flat, static difficulty'' model where each PoS-player holds a unit of stake and the total number of stakeholders is fixed, and the security properties hold under the assumption of an honest majority. Further, as mentioned before, our blockchain protocol can be viewed as a variant of Bitcoin Backbone~\cite{EC:GarKiaLeo15} and Ouroboros~\cite{C:KRDO17}. Thus, we list parameters that will be used in the following security analysis as shown in Table~\ref{tab:table1}.




{
\begin{table}[h!]
%\begin{sidewaystable}[h!] % <--
\small
\begin{center}
\begin{threeparttable}

    \caption{Parameters.}
    \label{tab:table1}
    \begin{tabular}{c*{1}{l}}
      \toprule % <-- Toprule here
      \multirow{2}{*}{\textbf{Params}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Notations}}} \\
      &\\
      [0.5ex]
      \midrule % <-- Midrule here
      $n$ & the total number of stakeholders.\\
        \rowcolor[gray]{0.9}
      $t$ & the corrupted number of stakeholders.\\
      $\stake$& stakes held by stakeholder  \\
      \rowcolor[gray]{0.9}
      $\astkratio$ & adversary stake ration \\
      \rowcolor[gray]{0.9}
      & $\astkratio:=\sum_{j\in\setS(\Adv)}\stake_j/ \sum_k^n \stake_k$ \\
      $\hstkratio$ & honest party stake ration with $\hstkratio=1-\astkratio$\\
      \rowcolor[gray]{0.9}
      $\probld$ & probability of leader succeeds \\
      \rowcolor[gray]{0.9}
      & in creating a PoS in a slot\\

      $\targetT$ & the target hash value for solving PoS\\
      \rowcolor[gray]{0.9}
      $\rltstake_i$ & sum of stakes held by honest stakeholders\\
      $\probhld$ & probability of honest leader succeeds\\
       & in creating a PoS in a slot\\
      \rowcolor[gray]{0.9}
      $ \advstake_i$& \footnotesize{stakes controlled by the adversary }\\
      \rowcolor[gray]{0.9}
      & \ie, $\advstake_i:=\sum_{j\in\setS(\Adv)}\stake_j$\\

      $\totstake_i$ & total skates in our setting \\ & $\totstake_i=\rltstake_i+\advstake_i$\\

      \hdashline
      \rowcolor[gray]{0.9}
      $\secp$ & security parameter \\
      $\compp$ & common prefix parameter-- consecutive blocks \\
      \rowcolor[gray]{0.9}
      $\cqp$ & chain quality parameter \\
      $\cgp$ & chain growth parameter\\
      \rowcolor[gray]{0.9}
      $\sysp\in (0,1)$ & system parameter, \ie, quality of concentration  \\
      \rowcolor[gray]{0.9}
      & of random variables in typical executions  \\
      $\ell$ & the length of the longest chain at round $\roundr$\\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
    \begin{tablenotes}
        \footnotesize
  \item[-] {in essence, $\rltstake_i$ is corresponding to the quata $q(n-t)$ in PoW. $q(n-t)$ implies the query quotas of the honest party.}
  \item[-]  $\rltstake:= \totstake-\advstake  =\sum_k^n \stake_k- \sum_{j\in\setS(\Adv)}\stake_j$
  \item[-]  $\hstkratio:=\rltstake_i/  \totstake  =\rltstake_i/ \sum_k^n \stake_k =1- \sum_{j\in\setS(\Adv)}\stake_j/ \sum_k^n \stake_k=1-\astkratio$
  \item[-]  $\probhld_i= 1 - (1-\probld_i)^{\rltstake_i} \geq \probld_i\cdot \rltstake_i/ (1+\probld_i\cdot \rltstake_i)$
  \item[-]  $1 - \probhld_i= (1-\probld_i)^{\rltstake_i}$, and $\probld_i\cdot (1 - \probhld_i)=\probld_i\cdot (1-\probld_i)^{\rltstake_i}$

      \end{tablenotes}

\end{threeparttable}

\end{center}
%\vspace{-3em}
%\end{sidewaystable}
\end{table}
}
Here, we remark that, the \textit{relative stake} $\rltstake_i$ is determined by a parameter $f$ of the protocol which we refer to as the active slots coefficient. Specifically,
$
    \probhld_i=1-(1-\probld_i)^{\rltstake_i}.
$



\noindent\textbf{Stake Fraction}.
To our knowledge, in any PoS-based protocol, ideally, the number of blocks mined by any party directly depends on its stake, or in other words, \textit{voting power} is proportional to the amount of stake with a party.







\noindent\textbf{Events}, $\Ep[X_i], \Ep[Y_i], \Ep[Z_i]$.
Before analyzing the security analysis, we first define the following events. In more detail,

\begin{itemize}
  \item [-] $\Ep[X_i]$, it means at least one honest party expects to gain the number of blocks at one round (\ie, slot) $\Ep[X_i]=\probhld_i$.
  \item [-] $ \Ep[Y_i]$, it means one and only one honest party expects to gain the number of blocks at one round (\ie, slot) $\Ep[Y_i]=(\probld_i \cdot \rltstake_i) \cdot (1-\probld_i)^{\rltstake_i} \geq \probhld_i(1-\probhld_i)$.

  \item [-] $\Ep[Z_i]$, it means the adversary expects to gain the number of blocks at one round
  $\Ep[Z_i]=\probld_i \cdot \advstake_i$. Notably, $\totstake_i=\rltstake_i+\advstake_i$, $\advstake_i$ is stakes controlled by the adversary.
   %which is corresponding to $qt$ in PoW.
\end{itemize}





\noindent\textbf{Bounded Events.} In order to analyze length bounds of the chain, we define the following bounds for three events respectively.

\begin{itemize}
  \item  The probability that at least one honest party computes a solution at a given round. We denote this parameter by $\probld_i$ and we have the lower and upper bound of $\Ep[X_i]$,
      \begin{eqnarray*}
        \Ep[X_i] &=& \probhld_i > (1 - \probhld_i) \probld_i \cdot \rltstake_i,  \\
        \Ep[X_i] &=& 1-(1-\probld)^{\rltstake_i}<  \probld_i \cdot \rltstake_i.
      \end{eqnarray*}



      where $\probld_i$ is the probability Leader Selection Process~\cite{EC:GarKiaLeo15}, $\probhld_i=1-(1-\probld_i)^{\rltstake_i}$ from the notes of Table~\ref{tab:table1}. %$\rltstake_i \approx_{PoW} q(n-t)$
  \item  The probability that one and only one (or exactly) honest party computes a solution at given round, then regarding the honest parties we have the upper bound of $\Ep[Y_i]$,
  \begin{equation*}
    \Ep[Y_i]=(\probld_i\cdot  \rltstake_i )\cdot (1-\probld_i)^{\rltstake_i} \geq \probhld_i(1-\probhld_i).
  \end{equation*}

  \item With respect to the expected number of blocks, the adversary can compute in a single round and we note the bound
\begin{equation*}
  \Ep[Z_i]=\probld_i \cdot \advstake_i = \astkratio \cdot \probld_i  \cdot \totstake_i < \frac{t}{n-t}\cdot \frac{\probhld_i}{1-\probhld_i}.
\end{equation*}

%$\advstake_i$ is corresponding $q(n-t)$ in PoW.


\end{itemize}







\subsubsection{Chain Growth}
%\par\noindent\textbf{Chain Growth}.
Intuitively, the chain growth property states that the chains of honest players should grow linearly to the number of rounds. In our setting, we are mimicking the bitcoin backbone by using a unique signature to act the role of a cryptographic puzzle solution. Hence, in the following proof, we can follow the proof of the strategy of \cite{EC:GarKiaLeo15} to analyze the property of chain growth.

\begin{definition}[Chain Growth Property ($\Qcg$), adopted from~\cite{EC:GarKiaLeo15}]
The chain growth property $\Qcg$ with parameter $\hstkratio:=1-\astkratio\in \R$ and round $\rounds\in \N$ states that for any honest party $P$ with chain $\chainC$, it holds that for any $\rounds$ there are at least $\hstkratio\cdot \stake$ blocks added to the chain of $P$.
\end{definition}



\begin{lemma}[Chain Growth Lemma]\label{lemma:chain-growth}
If an honest party has a chain of length $\chainlength$ at round $\roundr$, then every honest party has adopted a chain of length at least $\chainlength+\sum^{\rounds-1}_{i=\roundr}X_i$ by round $\rounds\geq \roundr$.
\end{lemma}

%\par\noindent\textbf{Sketched Proof}.
\begin{proof}[Sketch Proof]
The total number of block-cores from malicious players are bounded by the proportion of stakes they control. Since we assume that the honest players control more stakes than the malicious players, for the same core-chain, the malicious players cannot contribute more block-cores than the honest players. This will give us the chain quality property.
%
      \begin{equation*}
        Z(S) < \cqp\cdot X(S)
      \end{equation*}
\text{~by~assuming~a~contradiction~}
\begin{equation*}
Z(S)\geq  \cqp \cdot Y(S).
\end{equation*}
\end{proof}


\begin{theorem}[Chain Growth]\label{theorem:chain-growth}%\zlinote{refer to Ourobours}
The protocol satisfies the chain growth property with parameters $\hstkratio:=1-\astkratio$, $\rounds\in \N$ throughout an epoch of $R$ slots with probability at least $1-\exp(-\Omega(\sysp^2\rounds)+\ln R)$ aghast an adversary holding an $\astkratio-\sysp$ portion of the total stake for system parameter $\sysp\in \set{0,1}$.
\end{theorem}
We detail our security analysis in the Appendix Subsection~\ref{Appsubsec:chaingrowth}.



\subsubsection{Chain Quality}
%\par\noindent\textbf{Chain Quality}.
The property of chain quality aims at expressing
the number of honest blocks' contributions that are contained in a sufficiently long and continuous part of an honest chain. In our work, we follow the same spirit of Ouroboros to define the security properties for our proposed a quantum resistant PoS blockchain protocol.





\begin{definition}[Chain Quality Property $\Qcq$]
The chain quality $\Qcq$ with parameters $\mu\in \R$ and $\chainlength\in \N$ state that for any honest party $P$ with chain $\chainC$, it holds that for any $\chainlength$ consecutive blocks of $\chainC$ the ratio of honest blocks is at least $\mu$.
\end{definition}

%\begin{lemma}[Chain Quality Lemma]
%\zlinote{Do not need this lemma}
%\end{lemma}

\begin{proof}[Sketch Proof]
The total number of block-cores from malicious players are bounded by the proportion of stakes they control. Since we assume that the honest players control more stakes than the malicious players, for the same core-chain, the malicious players cannot contribute more block-cores than the honest players. This will give us the chain quality property.
%
      \begin{equation*}
        Z(S) < \cqp\cdot X(S)
      \end{equation*}
\text{~by~assuming~a~contradiction~}
\begin{equation*}
Z(S)\geq  \cqp \cdot Y(S).
\end{equation*}
\end{proof}

\begin{theorem}[Chain Quality]\label{theorem:chain-quality}
Let $\astkratio-\sysp$ be the adversarial stake ratio. The protocol satisfies the chain quality property with parameters $\mu\cdot (\astkratio-\sysp)=\astkratio/(1-\astkratio)$ and $\chainlength\in \N$ through an epoch of $R$ slots with probability at least
\begin{equation*}
  1-\exp(-\Omega(\sysp^2\cdot (\astkratio\cdot\chainlength))+\ln R).
\end{equation*}

\end{theorem}
We detail our security analysis in the Appendix Subsection~\ref{Appsubsec:chainquality}.
 
 
\subsubsection{Common Prefix}

\begin{definition}[Common Prefix Property ($\Qcp$)]
The common prefix property $\Qcp$ with parameter $\secp\in \N$ states that for any pair of honest players $P_1$, $P_2$ adopting the chains $\chainC_1$, $\chainC_2$ at round $\roundr_1\leq \roundr_2$ respectively, it holds that $\chainprefix_1 \preceq \chainC_2$ and $\chainprefix_2 \preceq \chainC_1$.
\end{definition}

\begin{lemma}[Common Prefix Lemma]\label{lemma:common-prefix}
If assume a typical execution and consider two chains $\chainC_1$ and $\chainC_2$. If
$\chainC_1$ is adopted by an honest party ar round $\roundr_1$, and $\chainC_2$ is either adopted by an honest party at round $\roundr$ or diffused at round $\roundr$ and has $\strlen(\chainC_2)\leq \strlen(\chainC_1)$, then $\chainprefix_1 \preceq \chainC_2$ and $\chainprefix_2 \preceq \chainC_1$ for $\compp$ consecutive blocks and $\secp$ consecutive rounds, \ie, $\secp\leq \compp/2 p$.
\end{lemma}

%\par\noindent\textbf{Sketched Proof}. 
\begin{proof}[Sketch Proof]
Below we sketch the proof and please refer to ~\cite[Lemma~14]{EC:GarKiaLeo15} for more concrete proof.
%
Assume, towards a contradiction, an execution in which the assumptions of the lemma hold, but either $\chainprefix_1 \npreceq \chainC_2$ or $\chainprefix_2 \npreceq \chainC_1$ for $\compp\geq 2\secp p$.
Consider the last block on the common prefix of $\chainC_1$ and $\chainC_2$ that was computed by an honest party and $\roundr^*$ be the round on which it was computed (if no such block exists for let $\roundr^*=0$). Define the set of rounds $\setS=\set{i: \roundr^*< i< \roundr}$. We claim that
\begin{equation*}
  Z(S)\geq Y(S).
\end{equation*}
However, $Z(S)\geq Y(S)$ contradicts  $Z(S) < Y(S)$.
\end{proof}

\begin{theorem}[Common Prefix]\label{theorem:common-prefix}
The probability of the protocol, when expected with a $(1-\sysp)/2$ fraction of adversarial stake, conflicts the common prefix property with parameter $\compp$ throughout an epoch of $R$ slots is no more that $\exp(-\Omega(\sqrt{\compp})+\ln{R})$; the constant hidden by the $\Omega(\cdot)$ notation depends only on $\sysp$.
\end{theorem}

==> body/Preliminary-Blockchain.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex

%Preliminaries and Bitcoin background will be provided in this section.  In Section~\ref{sec:model} we review the model of protocol execution. After that, we provide basic definitions in blockchain ledger systems in Section \ref{sec:gkl-block}. Finally, in Section~\ref{sec:ledger-properties}, we review the security analysis framework by Garay et al.~\cite{EC:GarKiaLeo15}.

%\subsection{Verifiable Random Function}


In this section, we review and list some definitions and notations that will be used in the following main contents.
%
We begin by reviewing the standard definition of digital signature schemes, the security notion of EU-CMA~\cite{SIAMCOMP:GolMicRiv88} and the main property of uniqueness. We then define two security notions for function families required for our reduction. The first is the well known pseudo-randomness property. The second is key one-wayness which states that it is hard to find a key $\signkey$ such that the function $\hashF_{\signkey}$ maps a given input $x$ to a given output $y$.

%
%\begin{definition}[Digital Signature Scheme]
%A digital signature scheme $\sig = (\Gen, \Sign, \Vrfy)$ is a triple of $\PPT$ algorithms:
%\begin{itemize}
%  \item $\Gen(1^{\secp})$
%  \item $\Sign(\signsk,\msg)$ output a signature $\sigma$ under the secret key $\signsk$ for a message $\msg$.
%
%  \item $\Vrfy$ ($\vrfproof$)
%\end{itemize}
%
%
%
%\end{definition}






%
%
%\noindent{\textbf{Digital Signing.}}
%Digital signatures allow users to authenticate information to each other without sharing any sharing any secret keys. A digital signature scheme consists of three fast algorithms: a probabilistic key generator $\Gen$, a signing algorithm $\Sign$, and a verification algorithm $\Vrfy$. In short, given a security parameter $\secp$, a sufficiently high integer, a user $i$ uses $\Gen$ to produce a pair of $\secp$-bit keys (i.e., strings): a ``public'' key $\pk_i$ and a matching ``secret'' signing key $\sk_i$.
%
%
%Crucially, a public key does not ``betray'' its corresponding secret key. That is, even given knowledge of $\pk_i$, no one other than $i$ is able to compute $\sk_i$ in less than astronomical time.
%
%
%
%
%User $i$ uses $\sk_i$ to digitally sign messages. For each possible message (binary string) $\msg$, $i$ first hashes $\msg$ and then runs algorithm $\Sign$ on inputs $\hfuncH(\msg)$ and $\sk_i$ so as to produce the $k$-bit string
%
%\begin{equation*}
%  \sigstr_{\pk_i}(\msg)=\Sign(\hfuncH(\msg), \sk_i).
%\end{equation*}
%
%
%where $\hfuncH$ has 256-bit long outputs.
%%Where we denote $i$'s signature of a string $\msg$ by $\Sigstr_i(\msg)$.
%
%The binary string $\sigstr_{\pk_i}(\msg)$ is referred to as $i$'s digital signature of $\msg$ (relative to $\pk_i$), and can be more simply denoted by $\sigstr_i(\msg)$, when the public key $\pk_i$ is clear from context.
%
%
%
%
%
%Everyone knowing $\pk_i$ can use it to verify the digital signatures produced by $i$. Specifically, on inputs (a) the public key $\pk_i$ of a player $i$, (b) a message $\msg$, and (c) a string $\sigstr:=\sigstr_i(\msg)$, that is, $i$'s alleged digital signature of the message $\msg$, the verification algorithm $\Vrfy$ outputs either YES or NO. The properties we require from a digital signature scheme are:
%
%\begin{itemize}
%  \item Legitimate signatures are always verified:
%  \item Digital signatures are hard to forge:
%\end{itemize}



%A digital signature scheme $\sig = (\Gen, \Sign, \Vrfy)$ is a triple of $\PPT$ algorithms:
%\begin{itemize}
%  \item $\Gen(1^{\secp})$
%  \item $\Sign(\signsk,\msg)$ output a signature $\sigma$ under the secret key $\signsk$ for a message $\msg$.
%
%  \item $\Vrfy$ ($\vrfproof$)

%Digital signatures allow users to authenticate information to each other without sharing any secret keys. A digital signature scheme consists of three fast algorithms: a probabilistic key generator $\Gen$, a signing algorithm $\Sign$, and a verification algorithm $\Vrfy$. In short, given a security parameter $\secp$, a sufficiently high integer, a user $i$ uses $\Gen$ to produce a pair of $\secp$-bit keys (i.e., strings): a ``public'' key $\pk_i$ and a matching ``secret'' signing key $\sk_i$.

\noindent{\textbf{Unique Digital Signing.}}
A traditional digital signature scheme $\sig = (\Gen, \Sign, \Vrfy)$ is a triple of $\PPT$ algorithms: a probabilistic key generator $\Gen$, a signing algorithm $\Sign$, and a verification algorithm $\Vrfy$. In short, given a security parameter $\secp$, a sufficiently high integer, a user $i$ uses $\Gen$ to produce a pair of $\secp$-bit keys (i.e., strings): a ``public'' key $\pk_i$ and a matching ``secret'' signing key $\sk_i$.
%
We also considering digital signature schemes  $(\uKeyGen, \uKeyVrfy, \uSign, \uVrfy)$~\cite{C:Lysyanskaya02,EPRINT:FanZho17} satisfying the additional \textit{uniqueness} property. Namely that, it is hard to find strings $\pk'$, $\msg$, $\sigstr$ and $\sigstr'$ such that
$ \sigstr\neq \sigstr' ~\text{and}~ \uVrfy(\pk',\msg,\sigstr)=\uVrfy(\pk',\msg,\linebreak \sigstr')=1.$
Note that the uniqueness property holds also for strings $\pk'$ that are not legitimately generated public keys. In particular, however, the uniqueness property implies that, if one used the specified key generator $\Gen$ to compute a public key $\pk$ together with a matching secret key $\sk$, and thus knew $\sk$, it would be essentially impossible also for him to find two different digital signatures for the same message relative to $\pk$.

\zlinote{There are similarities between the VRF and the unique signature. Particularly, the $\uSign(\sk,\msg)$}




\noindent{\textbf{Verifiable Random Function.}}
A function family $\hashH_{\cdot}(\cdot): \set{0, 1}^{a(\secp)} \to \set{0,1}^{b(\secp)}$ is family of VRFs for $a(\secp)$ and $b(\secp)$ in $\poly(\secp)$ time if there exist algorithms $(\Gen, \Prove, \Vrfy)$ such that $\Gen(1^{\secp})$ outputs a pair of keys $(\pk, \sk)$; $\Prove(\sk, \msgx)$ outputs a pair $(\hashH(\sk , \msgx), \zkproof(\sk, \msgx))$, where $\hashH(\sk , \msgx)$ is the function value and $\zkproof(\sk, \msgx)$ is the proof of correctness; and $\Vrfy(\pk, (\msgx, y), \zkproof)$ verifies that $y=\hashH(\sk, \msgx)$ using the proof $\zkproof$. Formally, we require the property of uniqueness, probability and pseudorandomness. Uniqueness implies that no values $(\pk, \msgx, y_1, y_2, \zkproof_1, \zkproof_2)$ can satisfy $\Vrfy(\msgx, y_1, \zkproof_1)=\Vrfy(\msgx, y_2, \zkproof_2)$. Provability implies that if $(y, \zkproof)=\Prove(\sk, \msgx)$, then $\Vrfy(\msgx, y, \zkproof)=1$. Pseudorandomness implies that no value of the function can be distinguished from random, even after seeing any other function values together with corresponding proofs, which can be guaranteed by hashing function $\hashH(\cdot)$. More details are referred to~\cite{FOCS:MicRabVad99}.









%\begin{itemize}
%     \item Uniqueness. It is hard to find strings $\pk'$, $\msg$, $\sigstr$ and $\sigstr'$ such that
%\begin{equation*}
%  \sigstr\neq \sigstr' ~\text{and}~ \Vrfy(\pk',\msg,\sigstr)=\Vrfy(\pk',\msg,\sigstr')=1.
%\end{equation*}
%
%Note that the uniqueness property holds also for strings $\pk'$ that are not legitimately generated public keys.



%\end{itemize}








%
%\begin{definition}[Unique Signature,~\cite{C:Lysyanskaya02,EPRINT:FanZho17}]
%If the signature scheme $(\uKeyGen, \uKeyVrfy, \uSign, \uVrfy)$
%
%\end{definition}



\par\noindent\textbf{Sigma Protocol and Non-interactive Zero-Knowledge Proofs}.
For every $\secp$, let $\cal$ be an efficiently computable binary relation. For pairs $(x,w) \in \calR$, we call $x$ the \emph{statement} and $w$ the \emph{witness}. Let $\calL_\calR$ be the language consisting of statements in $\R$, i.e. $\calL_\calR=\{x|\exists w
\,\, {\rm s.t. } \,\, (x,w)\in \R \}$. 
%there is a relation $\calR_{\secp}=\set{(\stmt, \wits): \stmt\in\calL_{\secp}, \wits\in \calW(\stmt)}$ such that the length of the statement $\stmt$ and the witness $\wits$ is bounded by a polynomial of $\secp$, $\stmt$ is a statement in an NP language $\calL_{\secp}$ and $\calW(\stmt)$ is the set of witness for proving $\stmt\in \calL_{\secp}$. 
In other words, there is an polynomial time algorithm runs in $\poly(\secp)$ that decides whether $(\stmt,\wits)\in \calR_{\secp}$.
%
%
A sigma protocol for $\calR_{\secp}$ consists two polynomial time algorithms, prover $P$ and verifier $V$. The sigma protocol procedure looks like the follows:
\begin{itemize}
  \item $P$ executes $(\aaa, \stt)\gets\Com(1^{\secp}, \sk:=(\stmt, \wits))$, where $\stt$ is its own state and it sends the commitment $\aaa$ to the verifier $V$.
  \item $V$ given $\stmt$ and $\aaa$, generates a challenge $\ccc$ uniformly at random in $\set{0,1}^{\secp}$ where $\secp$ is the security parameter of this protocol.

  \item $P$ given the challenge $\ccc$, generates a response $\zzz\gets \Prove(1^{\secp}, \sk:=(\stmt, \wits), \stt, \ccc)$.

  \item $V$ executes $\Vrfy(1^{\secp}, \pk:=\stmt, \aaa, \ccc, \zzz)$ checks  whether $(\aaa, \ccc, \zzz)$ is valid. If it is, $\Vrfy(1^{\secp}, \pk:=\stmt, \aaa, \ccc, \zzz)$ returns 1.
\end{itemize}
When it is clear in the context, we omit $1^{\secp}$ for convenience. In this setting, $\pk$ is denoted $\stmt$ and $\sk$ is denoted to $(\stmt, \wits)$.

%\par\noindent\textbf{}.
A non-interactive zero-knowledge proof (NIZK) of knowledge can be transformed from any public-coin zero-knowledge proof (\eg, Sigma-protocol) by using the Fiat-Shamir transform.
The NIZK consists of PPT algorithms $(\Prove,\Vrfy,\Sim,\Ext)$, where $\Prove$ is the prover algorithm, $\Vrfy$ is the verification algorithm, $\Sim$ is the simulator, and $\Ext$ is the knowledge extractor.
%Let $\PK$ be the public key, $(c_1,\ldots, c_n)$ be the original ciphertexts,
%$(c'_1,\ldots, c'_n)$ be the shuffled ciphertexts. Let $\Pi\in S_n$ and $(r_1,\ldots,r_n)$ the ranomness. The NIZK is defined as
%
%$$
%\NIZK \left\{
%\begin{array}{r}
%(\PK,(c_1,\ldots,c_n),(c'_1,\ldots,c'_n)),(\Pi,(r_1,\ldots,r_n)): \\
%\forall i\in[n]: c'_i= \Rand(\PK,c_{\Pi(i)} ; r_i)
%\end{array}
%\right\}\enspace.
%$$







%
%\subsection{Nakamoto's Protocol}
%
%
%
%
%The proof of work puzzle can be abstractly described via the following hash inequality
%\[
%H(h_{w},\omega, \record)<T
%\]
%where $h_{\omega}\in\{0,1\}^{\lambda}$ is the hash of previous POW-block for security parameter $\lambda$, $\omega\in\{0,1\}^{\lambda}$ is a suitable of solution for his puzzle, $X$ is the record component of the black, and $T$ denotes the current proof of work target.
%More details will be find in \cite{EC:GarKiaLeo15}.
%
%
%
%\begin{definition}[Block, From \cite{EC:GarKiaLeo15,EC:PasSeeshe17}]
%A POW \emph{block} is any triple of the form %$$\blockB=\inner{\hashs(\text{pre-msg}),\text{record},\text{nonce},\Func(\text{cur-msg)}}$$
%
%\begin{equation*}
%  \blockB=\inner{\hfunch(\text{pre-msg}),\text{record},\text{nonce}}
%\end{equation*}
%
%\begin{equation*}
% \ie,~ \blockB_{i+1}:= \inner{h_i=:\hfunch(\blockB_i),\record, \nonce}, \ie,  \blockB_{i+1}:= \inner{h_i,\record, \nonce}
%\end{equation*}
%for current data ``record'' $\record$ and ``nonce'' $\nonce\in [0,2^{32)}$. Further, where the hash function $\prehash$ that points to the previous record and hash function $\hfunch$ that points current record.
%%
%Hence, there exists a hash function satisfies
%$\Func(\Func(\text{pre-msg})\Vert\text{record}\Vert\text{nonce})< \text{Target~Value}$, namely that
%\[
%\hfunch:=\Func\big(\prehash, \record, \nonce \big)< T
%\]
%%where $\invf$
%\end{definition}
%
%\begin{definition}[Blockchain, From \cite{EC:GarKiaLeo15,EC:PasSeeshe17}]
%A \emph{blockchain}, or simple a ``chain'' is a sequence of \emph{blocks}. We first set the rightmost block as the head of the chain, e.g., $\head(\chain)$. (Note that if the chain is an empty string $\varepsilon$, by convention we set $\head(\varepsilon)=\varepsilon$.)
%
%A chain $\chain(:=(B_0,\cdots,B_{\ell}))$ with
%$\head(\chain)=\inner{ \pref',\record', \nonce',\func'}$ , e.g., a ``genesis'' block $B_0=\inner{\pref=0,\nonce=0, \record=\bot, \Func(0,0,\bot)}$, can be extended to a longer chain by appending a valid block $B_i=\inner{ \func_{i-1}, \record_i, \nonce, \func_i }$ with respect to $B_{i-1}$, where $\func_i$ satisfies $\Func\big(\func_{i-1},\nonce,\record_i\big)$.
%
%An example, $B_1=\inner{ \pref, \record, \nonce, \func }$ with respect to $B_0$, that satisfies $\func=\Func\big(\pref,\nonce,\record\big)$.
%
%\end{definition}
%
%
%
%\textbf{Nakamoto's Protocol:}
%
%Below, we turn to describing Nakamoto's protocol \cite{Nakamoto08}. We first set $(\Pi^p_{Nak},\Chain)$ as a pair of algorithms of blockchain protocol.
%The algorithm $\Pi^p_{Nak}$  takes the security parameter $\lambda$ as input and maintains the local chain $\chain$ which is the sequence of blocks $\vv{\matB}=(B_0,\cdots,B_{\ell})$.
% The ``record chain'' algorithm $\Chain(\lambda,record)$ of a player takes $\lambda$ and
% and $record$ as input and outputs the ordered sequence of records $\vv{\record}:=(\record_1,\cdots,\record_{\ell})$ contained in the sequence of blocks chain.
%
%
% Then, each round of $\Pi^p_{Nak}$ proceeds as follows \cite{EPRINT:PasShi16b}:
%
% At any point of the protocol execution, each miner attempts to increase the length of the blockchain by mining for a new block.
% \begin{enumerate}
%   \item Upon receiving and reading all incoming messages (delivered by the adversary $\calA$)
%   \item
% \end{enumerate}
%
%




%\subsection{PoW Blockchain  Syntax}
%\label{sec:gkl-block}

%\knote{Write intro}

%\hnote{@Alex, please DO spend time with GKL, and come up with a good subsection for blockchain syntax. You should find a way to introduce the syntax in a logic way. The current Bitcoin syntax is far from being ready. Please invest your energy!!!}


%
%
%We define a block $\blockB_j$ (for $ j \in [\numT]$) as a triple $\blockB_j = \angles{\hash_j, \record_j, \nonce_j}$, where $\hash_j \in {\{0,1\}}^\secp, \record_j \in {\{0,1\}}^{*}, \nonce_j \in {\{0,1\}}^\secp$. To generate a block with a user-defined input $\record_j$, a protocol party~(also called a miner) is trying to find such a random nonce $\nonce_j$ for which the inequality $\hfuncH(\hash_j, \record_j, \nonce_j) < \target$ holds, where $\hash_j$ is derived from a previous block $\angles{\hash_{j-1}, \record_{j-1}, \nonce_{j-1}}$ simply as $\hfuncH(\hash_{j-1}, \record_{j-1}, \nonce_{j-1})$, $\hfuncH(\cdot)$ is a cryptographic  hash function, and $\target$ is a hardness parameter~(also called difficulty) for solving the inequality cryptographic puzzle (\ie, PoW and PoS \etc).
%%
%For the first block in the sequence, also called {\em genesis block}, $\hash_0 = 0$.

%\begin{definition}[Block, From \cite{EC:GarKiaLeo15,EC:PasSeeshe17}]
%A PoW \emph{block} is any triple of the form %$$\blockB=\inner{\hashs(\text{pre-msg}),\text{record},\text{nonce},\Func(\text{cur-msg)}}$$
%%
%\begin{equation*}
%  \blockB=\inner{\hfunch(\text{pre-msg}),\text{record},\text{nonce}}
%\end{equation*}
%\ie,~ $
% \blockB_{i+1}:= \inner{h_i=:\hfunch(\blockB_i),\record, \nonce}, \ie,  \blockB_{i+1}:= \inner{h_i,\record, \nonce}
%$
%for current data ``record'' $\record$ and ``nonce'' $\nonce\in [0,2^{32})$. Further, where the hash function $\prehash$ that points to the previous record and hash function $\hfunch$ that points current record.
%%
%Hence, there exists a hash function satisfies
%$\Func(\Func(\text{pre-msg})\Vert\text{record}\Vert\text{nonce})< \text{Target~Value}$, namely that
%\[
%\hfunch:=\hashH\big(\prehash, \record, \nonce \big)< \targetT.
%\]
%%where $\invf$
%\end{definition}
%
%\begin{definition}[Blockchain, From \cite{EC:GarKiaLeo15,EC:PasSeeshe17}]
%A \emph{blockchain}, or simple a ``chain'' is a sequence of \emph{blocks}. We first set the rightmost block as the head of the chain, e.g., $\head(\chain)$. (Note that if the chain is an empty string $\varepsilon$, by convention we set $\head(\varepsilon)=\varepsilon$.)
%%
%A chain $\chain(:=(B_0,\cdots,B_{\ell}))$ with
%$\head(\chain)=\inner{ \pref',\record', \nonce',\func'}$ , e.g., a ``genesis'' block $B_0=\inner{\pref=0,\nonce=0, \record=\bot, \Func(0,0,\bot)}$, can be extended to a longer chain by appending a valid block $B_i=\inner{ \func_{i-1}, \record_i, \nonce, \func_i }$ with respect to $B_{i-1}$, where $\func_i$ satisfies $\Func\big(\func_{i-1},\nonce,\record_i\big)$.
%\end{definition}




%An example, $B_1=\inner{ \pref, \record, \nonce, \func }$ with respect to $B_0$, that satisfies $\func=\Func\big(\pref,\nonce,\record\big)$.
%Further, the PoW puzzle can be abstractly described via the following hash inequality
%\[
%H(h_{w},\record, \nonce)<\targetT
%\]
%where $h_{\omega}\in\{0,1\}^{\lambda}$ is the hash of previous PoW-block for security parameter $\lambda$, $\omega\in\{0,1\}^{\lambda}$ is a suitable of solution for his puzzle, $\record$ is the record component of the black, and $\targetT$ denotes the current proof of work target. More details will be find in \cite{EC:GarKiaLeo15}.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\par\noindent\textbf{Blockchain backgrounds}.
Ouroboros denotes the transaction ledger properties as~\cite{C:KRDO17}, it divides the \textit{physical time} into \textit{epochs}, and each epoch is divided into \textit{slots}, and a slot is a relatively short period of time (i.e., seconds). Meanwhile, each slot has one and only one leader (slot leader, SL). The slot leader has a (sole) right to produce one and only one block during his slot.
%It means that the number of slot leaders strictly equals the number of slots in epoch (let us call this number $N$), so it is impossible to produce more than $N$ blocks during an epoch\psz{is this sentence correct, i.e., do they guarantee that always a leader is elected and that always there is exactly one leader?}.
If the slot leader missed their slot (for example, being offline), the right to produce a block is lost until they are elected again. Notably, one or more slots can remain empty (without generated blocks), but the majority of blocks (at least $50\% + 1$) must be generated during an epoch. Necessary definitions will be provided in the following.









\begin{definition}[Genesis Block]
The genesis block $\blockB_0$ contains the list of stakeholders identified by their public-keys, their respective stakes
$$(\vk_1, \stake_1), (\vk_2, \stake_2),\cdots,(\vk_n, \stake_n).$$
\end{definition}



\begin{definition}[State]
A state is a string $\state\in \set{0,1}^{\secp}$. Notably, the state $\state_i$ of block $\blockB_i$ is equal to $\hashH(\blockB_{i-1})$, where $\hashH$ is a prescribed collision-resistant hash function.
\end{definition}

\begin{definition}[Block]
A block $\blockB$ generated at a slot $\slot_i\in\set{\slot_1,\slot_2,\cdots,\slot_R}$ contains \textbf{1).~} the current state $\state\in\set{0,1}^{\secp}$, \textbf{2).~} data $\data\in\set{0,1}^*$, \textbf{3).~} the slot number $\slot_i$ and \textbf{4).~} a signature $\sigma=\Sign_{\sk_i}(\state,\data,\slot_i)$ computed under $\sk_i$ corresponding to the stakeholder $U_i$ generating the block, \eg, the following block structure:
\begin{equation*}
  \blockB_i=(\state_i, \data_i, \slot_i, \sigma_i):=(\state_i:=\hashH(\blockB_{i-1}), \data_i, \slot_i, \sigma_i).
\end{equation*}
Notably, $\state_i=\hashH(\blockB_{i-1})$, and a $\slot_i$ is corresponding to a PoS-player $P$.
\end{definition}











\begin{definition}[Blockchain]
A blockchain (or simply chain) relative to the genesis block $\blockB_0$ is a sequence of blocks $\blockB_1, \blockB_2, \cdots, \blockB_n$ associated with a strictly increasing sequence of slots for which the state $\state_i$. %of block $\blockB_i$ is equal to $\hashH(\blockB_{i-1})$, where $\hashH$ is a prescribed collision-resistant hash function.


The length of a chain $\strlen(\chainC)=n$ is its number of blocks. The block $\blockB_n$ is the head of the chain, denoted $\head(\chainC)$. We treat the empty string $\empstr$ as a legal chain and by convention set $\head(\empstr)=\empstr$. The structure of blockchain $\chainC$ is as follows:
\begin{equation*}
  \fbox{$\blockB_0$} \gets \fbox{$\blockB_1$} \gets \cdots \gets \fbox{$\blockB_n$}.
\end{equation*}


\end{definition}


\begin{definition}[Epoch]

An epoch is a set of $R$ adjacent slots $S=\set{\slot_1,\cdots,\slot_R}$.

\end{definition}



\noindent\textbf{Leader Election}. As depicted in Figure~\ref{fig:PoS}, slot leaders are elected from the group of all \textit{stakeholders} who hold enough stake.
This community of stakeholders is known as ``electors''. Electors elect slot leaders for the next epoch during the current epoch. Thus, at the end of epoch $N$ it is already known who are slot leaders for the epoch $N+1$, and it cannot be changed.
Notably, anyone from the community of stakeholders can become a slot leader. However, an important idea of PoS is that the more stake stakeholder has, the more chances one has to be elected as a slot leader. Further, for each $0<j\leq R$, a slot leader $SL_j$ is determined who has the (sole) right to generate a block at slot $\slot_j$




\input{body/PoS-structure}




\par\noindent\textbf{Properties}.
Imprecisely speaking, as discussed in \cite{C:KRDO17}, we show that \textit{persistence} and \textit{liveness} can be derived from the following three elementary properties provided that protocol $\Pi$ derives the ledger from a data structure in the form of a blockchain.
%
In this work, we focus on the quantum-resistant PoS blockchain consensus and ignore the quantum-resistant transactions. Hence, we focus on the three elementary properties, \ie, common prefix, chain growth, and chain quality. The properties of persistence and liveness can be derived from the following three elementary properties.



\begin{itemize}
  \item \textbf{Common Prefix (CP or chain consistency)}; with parameters $\compp\in \N$. The chains $\chainC_1$ and $\chainC_2$ possessed by two honest parties at the onset of the slots $\slot_1< \slot_2$ are such that $\chainprefix_1 \preceq \chainC_2$, where $\chainprefix_1$ denotes the chain obtained by removing the last $\compp$ blocks from $\chainC_1$, and $\preceq$ denoted the prefix relation.








  \item \textbf{Chain Growth (CG)}; with parameters $\cgp\in (0, 1]$, $s \in \N$. Consider the chains $\chainC_1$, $\chainC_2$ processed by two honest parties at the onset of two slots $\slot_1$, $\slot_2$ with $\slot_2$ at least $s$ slots ahead of $\slot_1$. Then it holds that $\strlen(\chainC_2)-\strlen(\chainC_1)\geq \cgp\cdot s$. We call $\cgp$ the speed coefficient.



  \item \textbf{Chain Quality (CQ)}; with parameters $\cqp\in (0,1]$ and $\ell\in N$. Consider any portion of length at least $\ell$ of the chain possessed by an honest party at the onset of a round; the ration of blocks originating from the adversary is at most $1-\cqp$. We call $\cqp$ the chain quality coefficient.
\end{itemize}


These security properties have been adopted in many subsequent blockchain designs, such as \cite{EC:PasSeeshe17,C:BMTZ17,PODC:PasShi17,AC:PasShi17,EC:BGMTZ18,CCS:BGKRZ18}.



%You can think of this election as a ``fair lottery''; anyone from the group of stakeholders can become a slot leader. However, an important idea of PoS is that the more stake stakeholder has, the more chances one has to be elected as a slot leader. Notably, one stakeholder can be elected as a slot leader for more than one slot during the same epoch.
%Notably, stakeholder $\to$ electors (\ie, at least 2\% of total stakes) $\to$ slot leader $\to$ ledger or block. In the protocol described in this section, for each $0<j\leq R$, a slot leader $E_j$ is determined who has the (sole) right to generate a block at slot $\slot_j$










%Please note that not all stakeholders participate in this election, but only ones who have enough stake (for example, 2\% of the total stake).


%This group of stakeholders is known as ``electors''. Electors elect slot leaders for the next epoch during the current epoch. Thus, at the end of epoch $N$ it is already known who are slot leaders for the epoch $N+1$, and it cannot be changed. You can think of this election as a ``fair lottery''; anyone from the group of stakeholders can become a slot leader. However, an important idea of PoS is that the more stake stakeholder has, the more chances one has to be elected as a slot leader. Notably, one stakeholder can be elected as a slot leader for more than one slot during the same epoch.





























==> body/VRFinstantiation.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex
\subsection{Verifiable Random Functions}
A verifiable random function (or $\VRF$)~\cite{XXX} consists of four algorithms:
\begin{equation*}
  (\Gen, \Eval, \Prove, \Vrfy)
\end{equation*}
In more detail:
\begin{itemize}
  \item $(\vrfsk,\vrfvk)\gets\Gen(\secp)$. The setup algorithm takes as input a security parameter $\secp$ and outputs a secret key $\vrfsk$ and public verification key $\vrfvk\in\set{0,1}^k$.
  \item $\stry\gets\Eval(\vrfsk, \msgx)$. The algorithm takes as input the secret key $\vrfsk$ and a message $\msgx$ and outputs a string $\stry\in\set{0,1}^m$.
  \item $(\vrfproof,\stry)\gets\Prove(\vrfsk, \msgx)$. The prove algorithm takes as input the secret key $\vrfsk$ and a  message $\msgx$. It produces a proof $\vrfproof$ that $\stry$ is consistent with the verification key $\vrfvk$.
  \item $\Vrfy(\vrfvk, \vrfproof, \msgx, \stry)$. The verification algorithm takes as input the verification $\vrfvk$, a message $\msgx$, a string $\stry$ and a proof $\vrfproof$. It outputs 1 if the proof verifies and 0 otherwise.
\end{itemize}
Meanwhile, the scheme has the following properties:
\begin{enumerate}
  \item \textbf{Completeness.} Informally, it states that given any input $\msgx$, if $\stry$ is generated by running the honest evaluation algorithm and $\vrfproof$ is generated by running the honest prove algorithm, the verification algorithm would output 1 always. Formally,  if $\stry$, $\vrfproof=\Prove(\vrfsk, \msgx)$, then $\Vrfy(\vrfvk, \msgx, \stry, \vrfproof)=1$.


  \item \textbf{Uniqueness.} Informally, it states that for any input $\msgx$ and any verification $\vrfvk$ there exists at most a single $\stry$ for which there is an acceptable proof $\vrfproof$.
      Formally, no values $(\vrfvk, \msgx, (y, \vrfproof), (y', \vrfproof'))$ can satisfy both
      \begin{equation*}
        \Prove(\vrfvk, \msgx, \stry, \vrfproof)=1~\text{and}~\Prove(\vrfvk, \msgx, \stry', \vrfproof')=1
      \end{equation*}
      unless $\stry=\stry'$.






  \item \textbf{Selective Indistinguishability.} The selective security of a $\VRF$ scheme is captured by the following game. In more detail:
      \begin{enumerate}
        \item The adversary $\Adv$ on input the security parameter outputs a challenge $\msgx^*$.
        \item The challenger $\calC$ computes $(\vrfvk, \vrfsk)\gets\Gen(1^{\secp})$, $\vrfvk$ is handed to the adversary $\Adv$.
        \item The adversary can now adaptively make queries of the form $\msgx_i\neq \msgx^*$. On each query, $\calC$ computes $\stry_i\gets \Eval(\vrfsk, \msgx)$ and $\vrfproof_i\gets \Prove(\vrfsk,\msgx)$. Adversary is given $(\stry_i, \vrfproof_i)$.
        \item $\calC$ samples a bit $b\in \set{0,1}$. If $b=0$, $\calC$ sets $\stry^*=\Eval(\vrfsk, \msgx^*)$ and otherwise sets it as a random string in the co-domain of the PRF. $\stry^*$ is given to $\Adv$.
        \item Adversary $\Adv$ then outputs a bit $b'$. It wins the game if $b'=b$.
      \end{enumerate}
  We say that $\VRF$ is selectively secure if for any polynomial time adversary $\Adv$, the adversary wins with a negligible probability in the game described above.


  Formally, for any PPT algorithm $\Adv=(\Adv_E, \Adv_J)$, which runs for a total of $\step(\secp)$ steps when its first input is $1^{\secp}$, and does not query the $\Prove(\cdot)$ oracle on $\msgx$,
      \begin{equation*}
        \Pr\left[ b=b' \middle|
             \begin{array}{l}
               (\vrfvk, \vrfsk)\gets\Gen(1^{\secp}); \\
               (\msgx, \Adv_{st})\gets \Adv_{E}^{\Prove(\cdot)}(\vrfvk); \\
               \stry_0=\Eval(\vrfsk, \msgx);\\
               \stry_1\gets\set{0,1}^{\ell};\\
               b\gets \set{0,1}; b'\gets \Adv_j^{\Prove(\cdot)}(\stry_b, \Adv_{st})
             \end{array}
           \right]\leq \frac{1}{2}+\negl(\secp).
      \end{equation*}


\end{enumerate}


\subsection{Realization of VRF}



In this section, we attempt to realize the $\VRF$ (\ie, verifiable oblivious PRF: {$\hashF(\oprfkey, \oprfmsg)=\hashH(\oprfmsg, \hashG(\oprfmsg)^{\oprfkey})$}) in the random oracle model using two hash functions $\hashH$ and $\hashG$ with ranges $\set{0, 1}^{\vrflength}$ and $\inner{g}$ respectively with $\abs{\inner{g}}=q$. The implementation is based on the 2-Hash-DH verifiable oblivious PRF construction of~\cite{AC:JarKiaKra14}. The 2-Hash-DH construction relies on a group of prime order $q$ with a generator denoted $g$. The secret key is $\oprfkey$ chosen at random in $\Zq$, and the public key $\oprfpk$ is set to $\oprfpk=g^{\oprfkey}$. The function is defined as $\hashF(\oprfkey, \oprfmsg)=\hashH(\oprfmsg, \hashG(\oprfmsg)^{\oprfkey})$ where $\hashH$ and $\hashG$ are hash functions onto, respectively, the group $\inner{g}$ and $\set{0,1}$, $\secp$ is a security parameter. Specifically, the public-key is equal to $\oprfpk=g^{\oprfkey}$ and the output is $\hvH=\hashH(\msgm,\hvG)$ where $\hvG=\hashG(\msgm)^{\oprfkey}$, while the proof is set to $\vrfproof=(\hvG,\eqdlnizk)$ where $\eqdlnizk:=\underline{\EQDL\set{\oprfkey: \log_{\hashG(\msgm)}(\hvG) =\log_g(\oprfpk); \msgm, \oprfpk}}$ is a proof of equality of discrete logarithms. More concretely, the associated verifiable-OPRF is shown as the following Figure~\ref{fig:DH-basedOPRF}. In more detail,

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[ht]
\vspace{-.3cm}
\begin{center}


\fbox{\scriptsize
\begin{protocolm}{2}
%\toprule[0.75pt]

\protocolheader{{\sc Oblivious PRF}}
\midrule[0.5pt]
\participants{\underline{Sender~$S$}}{\underline{Receiver~$R$}}
\participants{\underline{Server}}{\underline{Client}}
\participants{\underline{Prover}}{\underline{Verifier}}
\participants{holds~$\oprfkey$}{holds~$\oprfmsg$}
\midrule[0.5pt]
%&&
&&\mbox{1).~Inputs~} \oprfmsg \mbox{~picks~} \oprfrand\\

&\receives{\hvGrand}&\mbox{2).~computes~} \hvGrand=(\hashG(\oprfmsg))^{\oprfrand} \\

\mbox{3).~verifies~} \hvGrand\in \G  &&\\
\mbox{4).~picks~} \oprfkey\gets\Zq&&\\
\mbox{~and~computes~} \hvGkey=(\hvGrand)^{\oprfkey} &\sends{\hvGkey}&\\
&&\mbox{5).~outputs~} \hashF(\oprfkey, \oprfmsg)\\
&&~~~~~~~~~~~~ =\hashH(\oprfmsg, {\hvGkey}^{1/\oprfrand})\\
&&~~~~~~~~~~~~ =\hashH(\oprfmsg, \hashG(\oprfmsg)^{\oprfkey})\\
&&~~~~~~~~~~~~ =\hashH(\oprfmsg, \hvG)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{protocolm}
}
\vspace{-.3cm}
\end{center}
\caption{\label{fig:DH-basedOPRF} DH-based Oblivious-PRF}
\vspace{-.3cm}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{enumerate}
  \item The receiver (or the client) sends $\hvGrand=\hashG(\oprfmsg)^{\oprfrand}$ to the sender.
  \item Upon receiving $\hvGrand$, the sender (or the server) then checks $\hvG\in \inner{g}$. Then the sender computes $\hvGkey:=\hvGrand^{\oprfkey}$ and returns the pair of public key $\oprfpk=g^{\oprfkey}$ and $\hvGkey$ to the receiver.
  \item The protocol terminates with the receiver returning the value $\hashH(\oprfmsg, \hvGkey^{1/\oprfrand})$ after checking that the tuple $\inner{g, \oprfpk, \hvG, \hvGkey}$ is a valid DDH tuple (which implies that $\inner{g, \oprfpk, \hashG(\oprfmsg), \hvGkey^{1/\oprfrand}}$ is a valid DDH tuple).
\end{enumerate}





To achieve the latter test, the sender transmits a NIZK for equality of discrete
logarithms, specifically showing that the tuple $\inner{g, \oprfpk, \hvG, \hvGkey}$ satisfies the relation $\log_{\hashG(\msgm)}(\hvG) =\log_g(\oprfpk)$, \ie, $\hvG=\hashG(\oprfmsg)^{\oprfkey}$ and $\oprfpk=g^{\oprfkey}$. This is a standard protocol that we recall for completeness: the sender selects a random $\eqdlmask\in \Zq$ to hind (or mask) the key (\ie, witness) $\oprfkey$ and generates a challenge $\eqdlchlg=\hashH_{\zk}(g, \oprfpk, \hvGrand, \hvGkey, g^{\eqdlmask}, \hvGrand^{\eqdlmask})$ as well as $\eqdlproof:=\eqdlchlg\cdot \oprfkey+ \eqdlmask\pmod{q}$, where $g^{\eqdlmask}$ is to mask the partial statement (\ie, public key) $\oprfpk=g^{\oprfkey}$ and $\hvGrand^{\eqdlmask}$ is to mask the residuary
statement (\ie, the second move message sent to the receiver)  $\hvGkey=\hvGrand^{\oprfkey}$. Thus, the proof notation $\underline{\EQDL\set{\oprfkey: \log_{\hashG(\msgm)}(\hvG) =\log_g(\oprfpk); \oprfmsg, \oprfpk}}$ is a proof of equality of discrete logarithms, which we denote as $\NIZK_{\eqdl}^{\hashH_{\zk}[g, \oprfpk, \hvGrand, \hvGkey]}$.
Essentially, the proof notation $\EQDL\set{\oprfkey: \log_{\hashG(\msgm)}(\hvG) =\log_g(\oprfpk); \msgm, \oprfpk}$ stands for the string $(\eqdlchlg,\eqdlproof)$, while the verification of $(\eqdlchlg,\eqdlproof)$ on context $\msgm$, $\oprfpk$ is performed by checking the equality
      \begin{equation*}
        \eqdlchlg=\hashH(g,\oprfpk, \hvGrand, \hvGkey, g^{\eqdlproof}\cdot \oprfpk^{-\eqdlchlg}, \hvGrand^{\eqdlproof} \cdot \hvGkey^{-\eqdlchlg}).
      \end{equation*}

\begin{remark}Considering the same challenge $\eqdlchlg$, mask $\eqdlmask$, and $\eqdlproof=\eqdlchlg\cdot \oprfkey+\eqdlmask\pmod{q}$, there exist the following facts:
\begin{itemize}
  \item regarding the statement $\oprfpk=g^{\oprfkey}$, the verifier verifies $g^{\eqdlproof}=(g^{\oprfkey})^{\eqdlchlg}\cdot g^{\eqdlmask}=\oprfpk^{\eqdlchlg}\cdot g^{\eqdlmask}$.

  \item regarding the statement $\hvGkey=(\hvGrand)^{\oprfkey}$, the verifier verifies    $\hvGrand^{\eqdlproof}=({\hvGrand}^{\oprfkey})^{\eqdlchlg}\cdot {\hvGrand}^{\eqdlmask}=\hvGkey^{\eqdlchlg}\cdot {\hvGrand}^{\eqdlmask}$.
\end{itemize}

\end{remark}

Thus, we present this latter NIZK version as our realization in Figure~\ref{fig:DH-basedVOPRF}.

\begin{figure*}[ht]
\vspace{-.3cm}
\begin{center}


\fbox{\scriptsize
\begin{protocolm}{2}
%\toprule[0.75pt]

\protocolheader{{\sc Oblivious Verifiable PRF}}
\midrule[0.5pt]
\participants{\underline{Sender~$S$}}{\underline{Receiver~$R$}}
\participants{\underline{Server}}{\underline{Client}}
\participants{\underline{Prover}}{\underline{Verifier}}
\participants{holds~$\oprfkey$}{holds~$\oprfmsg$}
\midrule[0.5pt]
%&&
&&\mbox{1).~Inputs~} \oprfmsg \mbox{~picks~} \oprfrand\\

&\receives{\hvGrand}&\mbox{2).~computes~} \hvGrand=(\hashG(\oprfmsg))^{\oprfrand} \\

\mbox{3).~verifies~} \hvGrand\in \G  &&\\
\mbox{4).~picks~} \oprfkey\gets\Zq&&\\
\mbox{~and~computes~} \hvGkey=(\hvGrand)^{\oprfkey} &&\\


\begin{elaboration}
5).~generates~a~mask~$\eqdlmask$~\\
6).~computes~masking~statements\\
~~~~~~~~ $\oprfpk':=g^{\eqdlmask}$~and~$\hvGkey'=\hvGrand^{\eqdlmask}$\\
7).~creates a challenge~\\
~~~~~~~~ $\eqdlchlg=\hashH_{\zk}(g, \oprfpk, \hvGrand, \hvGkey, g^{\eqdlmask}, \hvGrand^{\eqdlmask})$\\
8).~generates~proof~\\
~~~~~~~~$\eqdlproof:=\eqdlchlg\cdot \oprfkey+ \eqdlmask\pmod{q}$

\end{elaboration}&\sends{\hvGkey', \oprfpk', \eqdlproof, \eqdlchlg}&\\

&\mbox{not~} \hvGkey~&\\
&&\mbox{9).~if~$\eqdlproof$~verifies~then}\\
&&\mbox{~outputs~} \hashF(\oprfkey, \oprfmsg)\\
&&~~~~~~~~~~~~ =\hashH(\oprfmsg, {\hvGkey}^{1/\oprfrand})\\
&&~~~~~~~~~~~~ =\hashH(\oprfmsg, \hashG(\oprfmsg)^{\oprfkey})\\
&&~~~~~~~~~~~~ =\hashH(\oprfmsg, \hvG)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{protocolm}
}
\vspace{-.3cm}
\end{center}
\caption{\label{fig:DH-basedVOPRF} DH-based Verifiable Oblivious-PRF}
\vspace{-.3cm}
\end{figure*}



\begin{theorem}
The 2-Hash-DH construction presented above over a group $\G$ of order $p$ realizes $\VRF$ in the random oracle model assuming the computational-DH.
\end{theorem}
Here, we omit the proof since it is out of the scope of this paper, and we refer to \cite{AC:JarKiaKra14,EC:DGKR18} for more details.


\zlinote{TBD}


The implementation is based on the 2-Hash-DH verifiable oblivious PRF construction of~\cite{AC:JarKiaKra14}. Specifically, the public-key is equal to $\oprfpk=g^{\oprfkey}$ and the output is $\hvH=\hashH(\msgm,\hvG)$ where $\hvG=\hashG(\msgm)^{\oprfkey}$, while the proof is set to $\vrfproof=(\hvG,\eqdlproof)$ where $\eqdlproof:=\underline{\EQDL\set{\oprfkey: \log_{\hashG(\msgm)}(\hvG) =\log_g(\oprfpk): \msgm, \oprfpk }}$ is a proof of equality of discrete logarithms. The verification of $(\msgm, \hvH, \vrfproof, \oprfpk)$ proceeds as follows:









\begin{enumerate}
  \item It parses $\vrfproof$ as $(u, \eqdlproof)$. It verifies $\hvH=\hashH(\msgm, \hvG)$ for $\hvG=\hashG(\msgm)^{\oprfkey}$ as well as the proof $\eqdlproof$ and returns 1 if and only if both tests pass. The proof notation $\EQDL\set{k: \log_{\hashG(\msgm)}(u) =\log_g(v): \msgm, v }$ stands for the string $(c,s)$ where $c=\hashH(\msgm, v, g^r, \hashG(\msgm)^r)$, $s=r+kc\pmod{q}$, while the verification of $(c, s)$ on context $\msgm$, $v$ is performed by checking the equality
      \begin{equation*}
        c=\hashH(\msgm, v, g^s\cdot v^{-c}, \hashG(\msgm)^s\cdot u^{-c}).
      \end{equation*}
\end{enumerate}






%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Oblivious PRF}


A pseudorandom function (PRF) \cite{JACM:GolGolMic86} is an efficiently computable keyed function $f_{\prfkey}(\cdot)$ whose values are indistinguishable, for a randomly chosen key $\prfkey$, from random elements in the function range.

An Oblivious Pseudorandom Function (OPRF) \cite{TCC:FIPR05} is a two-party protocol between sender $S$ and receiver $R$ for securely computing a pseudorandom function $f_{\prfkey}(\cdot)$ on key $\prfkey$ contributed by $S$ and input $\prfmsg$ contributed by $R$, in such a way that receiver $R$ learns only the value $f_{\prfkey}(\prfmsg)$ while sender $S$ learns nothing from the interaction. In other words, an OPRF protocol for PRF $f_{\prfkey}(\cdot)$ is a secure computation for functionality $F_{OPRF}:(\prfkey, \prfmsg) \to (\bot, f_{\prfkey}(\prfmsg))$.


\zlimark{
An oblivious pseudorandom function (OPRF) \cite{TCC:FIPR05} is a protocol in which a sender learns (or chooses) a random PRF key (or seed) $\prfkey$ while the receiver learns $f_{\prfkey}(\prfmsg)$, the result of the PRF on a single input $\prfmsg$ chosen by the receiver. Traditionally, the general definition of an OPRF allows the receiver to evaluate the PRF on several inputs.


}


\zlimark{

In an OPRF functionality for a PRF $F$, the receiver provides an input (message) $\prfmsg$; the functionality chooses a random key (or seed) $\prfkey$, gives $\prfkey$ to the sender and $F(\prfkey, \prfmsg)$ to the receiver.

}


The first oblivious PRF construction was given by Naor and Reingold \cite{FOCS:NaoRei97}, based on the PRF construction given in the same paper, $F_{\prfkey}(\prfmsg) = g^{\prod \prfkey_i^{\prfmsg_i}}$, where key $\prfkey$ is the sequence of $T$ random elements $\prfmsg_1,\cdots, \prfmsg_T$ in $\Zq$, $q$ is the order of the group $\G$ in which the Decisional Diffie-Hellman assumption holds, and $T$ is the bit length of elements $\prfkey$ in the PRF domain. This first oblivious PRF protocol required $O(t)$ rounds.










The oblivious pseudorandom function was introduced by Freedman, Ishai, Pinkas, and Reingold \cite{TCC:FIPR05} with follow-up works \cite{CCS:KKRT16}.











OT of random messages shares many properties with oblivious PRF (OPRF). In OT of random messages, the sender learns random $\msg_0$, $\msg_1$ while the receiver learns $\msg_r$ for choice bit $r\in\set{0,1}$. One can think of the function  $\Func((\msg_0,\msg_1),r)=\msg_r$ as a pseudo-random function with input domain $\set{0,1}$. Similarly, one can interpret 1-out-of-$n$ OT of random messages as an oblivious PRF (OPRF) with input domain $\set{1,2,\cdots,n}$.




\zlinote{TBD}



An oblivious pseudo-random function (OPRF) is a protocol in which a sender learns (or chooses) a random PRF key $\prfkey$ (or seed $\seed$) while the receiver learns $\Func(\prfkey,\prfmsg)$ (or $\Func(\seed, \rand)$), the result of the PRF on a single message $\prfmsg$ (or input $\rand$) chosen by the receiver.




While the general definition of an OPRF allows the receiver to evaluate the PRF on several inputs, in this paper we consider only the case where the receiver can evaluate the PRF on a single input.


==> body/ZKPrelated.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex

\subsection{Post-Quantum Zero-Knowledge Proof}

There exist ZKPs that only use collision-resistant hash functions and hence are plausibly post quantum secure. Popular examples include Hyrax, Aurora, or zkSTARK.

Other notable ZKPs like Bulletproofs or libsnark rely on cryptographic assumptions which are known to be vulnerable to quantum attacks (e.g. hardness of discrete log in certain elliptic curve groups).


$\ZKB$

$\ZKBpp$

$\zkstark$

Peikert and Vaikuntanathan first discuss how to design noninteractive statistical zero-knowledge proofs for lattice problems from 2008~\cite{C:PeiVai08}. Many XXXX




The following Table~\ref{XXX} for post-quantum security denotes that it is feasibly post-quantum secure.

{\tiny
%\rowcolor[gray]{0.9}
\definecolor{Gray}{gray}{0.9}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\newcolumntype{a}{>{\columncolor{Gray}}c}
\newcolumntype{b}{>{\columncolor{white}}c}

\begin{table*}[h!]
%\begin{sidewaystable}[h!] % <--
\small
\begin{center}
\begin{threeparttable}

    \caption{Overview of Quantum-Resistant Proof Systems.}
    \label{table:pqnizk}
    \begin{tabular}{l|a b| a  b | a  b }%{ll|*{3}{l}}
      \toprule % <-- Toprule here
      %\multirow{2}{*}
      \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Scheme}}}
      & \multicolumn{2}{c|}{\underline{\textbf{Performance}}}
      & \multicolumn{2}{c|}{\underline{\textbf{Size}}}
      & \multicolumn{1}{c|}{\underline{\textbf{Assumption}}}
      & \multicolumn{1}{c|}{\underline{\textbf{Untrusted Setup}}}\\
      & \textbf{Prover} & \textbf{Verifier} & \textbf{CRS} & \textbf{Proof}  & $\sk$  \\
      [0.5ex]
      \midrule % <-- Midrule here
      %\rowcolor[gray]{0.9}
      \multirow{1}{*}{$\ZKB$~\cite{USENIX:GiaMadOrl16}}
      &  &  &  &   & CRHF & \xmark \\
      \hdashline
      \multirow{1}{*}{$\ZKBpp$~\cite{CCS:CDGORR17}}
      &  &  &  &   & CRHF & \xmark \\
      \hdashline
      \multirow{4}{*}{Picnic}
      & Chase~\etal~\cite{CCS:CDGORR17} & \\
      & Katz~\etal~\cite{CCS:KatKolWan18} &  \\
      & Dinur~\etal~\cite{EC:DKPRR19} &  \\
      & Derler~\etal~\cite{PQCRYPTO:DerRamSla18} &  \\
       \hdashline
      \multirow{1}{*}{Ligero~\cite{CCS:AHIV17}}
      & $n\log{n}$ & $c\log{c}+h\log{h}$  & $0$ & $\sqrt{n}$ & CRHF & \cmark\\
      \hdashline
      \rowcolor[gray]{0.9}
      \multirow{1}{*}{$\zkstark$~\cite{EPRINT:BBHR18}}
      & $n\polylog{n}$ & $\polylog{n}$ & $0$ & $\log^2{n}$ & CRHF & \cmark\\
      \hdashline
      \multirow{1}{*}{Aurora~\cite{EC:BCRSVW19}}
      & $n\log{n}$ & $c\log{c}+h\log{h}$  & $0$ & $\sqrt{n}$ & CRHF & \cmark\\
      \hdashline
      \multirow{1}{*}{Bootle~\etal~\cite{AC:BCGGHJ17}}
      & $n$ & $n$ & $0$ & $\sqrt{n}$ & CRHF & \cmark\\
      \hdashline
      \hline
      \hdashline

      \multirow{1}{*}{Boneh~\etal~\cite{EC:BISW17}(ePrint2017/240)}
      & \\



      \hdashline
      \multirow{1}{*}{Kim and Wu~\etal~\cite{C:KimWu18}(ePrint2018/272)}
      &  \\


      \hdashline
      \multirow{1}{*}{Gennaro~\etal~\cite{CCS:GMNO18}(ePrint2018/275)}
      &  \\
      \hdashline

      \multirow{1}{*}{Baum~\etal~\cite{C:BBCPGL18}(ePrint2018/560)}
      & $n\log{n}$ & $n$ & $\sqrt{n}$ & $\sqrt{n\log{n}}$ & SIS & \cmark \\
      \hdashline
      \multirow{1}{*}{Libert~\etal~\cite{C:LLNW18}(ePrint2018/716)}
      &  \\
      \hdashline
      \multirow{1}{*}{Peikert and Shiehian~\cite{C:PeiShi19}(ePrint2019/158)}
      &  \\
      \hdashline
      \multirow{1}{*}{Lombardi~\etal~\cite{C:LQRWW19}(ePrint2019/242)}
      &  \\
      \hdashline
      \multirow{1}{*}{Esgin~\etal~\cite{C:ESLL19}(ePrint2019/445)}
      &  \\
      \hdashline
      \multirow{1}{*}{Katsumata~\etal~\cite{C:KNYY19}(ePrint2019/623)}
      &  \\
      \hdashline
      \multirow{1}{*}{Yang~\etal~\cite{C:YAZXYW19}(ePrint2019/747)}
      &  \\
      \hdashline
      \multirow{1}{*}{Bootle~\etal~\cite{C:BooLyuSei19}(ePrint2019/642)}
      &  \\

      \hdashline
      \multirow{1}{*}{Chiesa~\etal~\cite{EPRINT:ChiManSpo19}(ePrint2019/834)}
      &  \\

      \bottomrule % <-- Bottomrule here
    \end{tabular}
    \begin{tablenotes}
        \footnotesize
  \item[*] {https://falcon-sign.info/}
  \item[-] Asymptotic efficiency comparison of zero-knowledge proofs for arithmetic circuits. Here n is the number of gates, $d$ is the depth of the circuit, $h$ is the width of the subcircuits, $c$ is the number of copies of the subcircuits, $\ell$ is the size of the instance, and $w$ is the size of the witness. An empty circle denotes that the scheme does not have this property and a full circle denotes that the scheme does have this property.
  \item[-]  DL stands for discrete log, CRHF stands for collision-resistant hash functions, KOE stands for knowledge-of-exponent, and AGM stands for algebraic group model.
  \item [-] \cmark~ denotes that the scheme does have this property.
  \item [-] \xmark~ denotes that the scheme does not have this property.
      \end{tablenotes}
\end{threeparttable}
\end{center}
\vspace{-1em}
%\end{sidewaystable}
\end{table*}
}


%$\ZKBoo$~\cite{USENIX:GiaMadOrl16}, $\ZKBpp$~\cite{CCS:CDGORR17}, and Ligero~\cite{CCS:AHIV17}


Ligero~\cite{CCS:AHIV17} is roughly 4 times shorter than a similar proof of $\ZKBpp$~\cite{CCS:CDGORR17}, an optimized variant of $\ZKB$~\cite{USENIX:GiaMadOrl16}.


Importantly, $\zksnark$s require a trusted setup phase whereas $\zkstark$s use publicly verifiable randomness to create trustlessly verifiable computation systems. $\zkstark$s are more scalable in terms of computational speed and size when compared to $\zksnark$s

Notably, the complexity of $\ZKB$ and $\ZKBpp$ only depends on the number of
Boolean AND gates (as XOR's are for free).

\subsubsection{zk-SNARKs vs. Zk-STARKs vs. BulletProofs}
\zli{updated}

$\zksnark$ implies that (zero-knowledge succinct non-interactive argument of Knowledge).

$\zkstark$ implies that



To our knowledge, at the beginning of 2019, the most popular proof systems are $\zksnark$s, $\zkstark$s, and $\BF$,




$\zksnark$s, $\zkstark$s, and $\BF$ are three major zero knowledge proofs to provide privacy for the blockchain technology. If we can compare them,
\begin{itemize}
  \item $\BF$s and $\zkstark$s require no trusted setup. Unlike $\zksnark$s that require a trusted setup that creates an uncomfortable situation for it.

  \item \Zcash using $\zksnark$s can hide amount address along with sender and recipient. It it not yet clear to me if it is possible to hide sender and recipient by $\BF$s and $\zkstark$s.

  \item Apparently, $\zkstark$s is faster than $\zksnark$s is faster than $\BF$s.

  \item $\BF$s is shorter than $\zksnark$s and $\zkstark$s.
\end{itemize}





Today, two leading technologies are offering their cryptocurrencies, Monero and ZCash, and are striving to solve protection issues. Monero uses the Ring Confidential signature technology. In contrast, Z-Cash takes advantage of zk-SNARK (Zero-knowledge scalable transparent argument of knowledge), a technology that provides the ability to conduct anonymous transactions.

zk-STARKs aim to provide fast, scalable solutions to ensure financial security. In this way, transaction encryption is possible. zk-STARKs were listed as one of the 10 Breakthrough Technologies of 2018. The fact that such widely-known organizations as R3 and Ethereum have already started to implement zk-STARKs in their use cases is proof of the high potential of zk-SNARKS.



\noindent\textbf{Advantages of $\zkstark$}


please see the link \href{https://hackernoon.com/alexs-notes-on-zk-starks-167f8e044ab0}{https://hackernoon.com/alexs-notes-on-zk-starks-167f8e044ab0}






There exist some available $\zksnark$ schemes,
such as
\begin{itemize}
  \item Hyrax~proposed by Wahby~\etal~\cite{SP:WTSTW18}.
  \item Bulletproof~proposed by B{\"{u}}nz~\etal~\cite{SP:BBBPWM18}.
  \item Sonic~proposed by Maller~\etal~\cite{CCS:MBKM19}.
  \item Halo~proposed by~Bowe\etal~\cite{EPRINT:BowGriHop19}.
  \item Spartan~proposed by~Setty~\cite{EPRINT:Setty19}.
  \item Pinocchio~proposed by Parno~\etal~\cite{CACM:PHGR16}.
  \item Bitansky~\etal~\cite{TCC:BCIPO13}, Lipmaa~\cite{AC:Lipmaa13}, Ben{-}Sasson~\etal~\cite{C:BCTV14}, Danezis~\etal~\cite{AC:DFGK14}, Groth~\cite{EC:Groth16}, Groth and Maller~\cite{C:GroMal17}.
\end{itemize}


Bulletproofs are short non-interactive zero-knowledge proofs that require no trusted setup. A bulletproof can be used to convince a verifier that an encrypted plaintext is well formed. For example, prove that an encrypted number is in a given range, without revealing anything else about the number. Compared to SNARKs, Bulletproofs require no trusted setup. However, verifying a bulletproof is more time consuming than verifying a SNARK proof.


==> body/ZKproof.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex

%\section{Building Blocks}





==> body/attacks.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex

\newpage
\clearpage
\subsection{Dynamic committee election}
Snow White proceeds in epochs. In each epochs, a most recent set of stake-holders will be elected as a committee and may be randomly chosen to generate blocks.


To prevent ``\textit{adaptive key selection attacks}'' and ``\textit{randomness-biasing attacks}'', Snow White proposes a novel ``\textit{two-lookback}'' mechanism that addresses the above two challenges simultaneously. Each epoch's new consensus committee and randomness seed are determned in a two-phase process, where each phase spans roughly $\lambda$ blocks of time for some appropriate security parameter $\lambda$.


\par\noindent\textbf{Determine the new consensus commitments}.
Technically, Snow White provides an epoch-based protocol for committee reconfiguration. Firstly, in Snow White, $T_{epoch}$ is a protocol parameter that denotes the length of each epoch. In each $T_{epoch}$, Snow White provides a committee the opportunity to reconfigure. Meanwhile, Snow White sets every block in a valid blockchain along with the time-stamp between $[start(i), end(i)]$ is associated with the $i$-th committee, where $start(i)$ and $end(i)$ denote the beginning and ending times of the $i$-th committee. Then, an alert node determines the $i$-th committee at any time $t\in [start(i), end(i)]$ in the $i$-th epoch as follows:
\begin{itemize}
  \item find the latest block in its local chain whose timestamp $\ell$ is no greater than $\ell\leq start(i)-2\lambda$, where $2\lambda$ must be sufficiently large.
  \item and output the $i$-th new committee by extracting public keys and calling $extractpks(chain[:\ell])$ for time $t$, where $chain[:\ell]$ implies the prefix of its local chain by time $start(i)$.
\end{itemize}


Notably,  $extractpks(chain[:\ell])=pks_{\ell}$ means that $\ell$ is the largest index selected by an honest node satisfying $chain[:\ell].time + 2\lambda \leq rnddown(t)$, $rnddown=\lfloor t/T_{epoch}\rfloor \cdot T_{epoch}$. At the beginning, there is $extractpks(chain[:0])=pks_0$.






\par\noindent\textbf{Extract the new randomness seed}. At any time $t\in [start(i), end(i)]$ an alert node determines the $i$-th hash in the $i$-th epoch as the following manner:
\begin{itemize}
  \item find the latest block its local chain whose timestape is no greater than $start(i)-\lambda$, and suppose this block resides at index $\ell_1$, where $\ell_1\leq start(i)-\lambda$.
  \item output $extractnonce(chain[:\ell_1])$. Notably, alert nodes always embed a random seed in any block they mine, and $extractnonce(chain[:\ell_1])$ can simply use the seeds in the prefix of the chain as a nonce to seed the random oracle $H$.

\end{itemize}









\subsection{Long-range attacks protection}
Long-range attack corruption is discuss in Snow White but named in ``\textit{posterior corruption}'' and ``\textit{costless simulation attack}'', which means if stake-holders sold their stakes, then nothing can prevent them from performing a history-rewrite attacks. Particularly, if a set of nodes denoted $C$ control the majority stake in some past committee. These nodes can collude to fork the history from the point in the past when they control majority-- and in this alternate history money can transfer in a way such that $C$ continues to hold majority stake (possibly transferred to other pseudonyms of the corrupt nodes) such that the attack can be sustained.

In Algorand adopts \textit{erasure model}, and their nodes remove keys to prevent long-range attack.
Conversely, in Snow White, to defend against such a long-range attack (or, posterior corruption attack), the mitigation strategy employed is time-stamps for chain selection and some form of checkpointing mechanism~\cite[ePrint2018/248]{XXX}. In a nutshell, the newly joining user obtain a somewhat recent checkpoint from the set of nodes it can access upon joining. Notably, when nodes join the system they can access a set of online nodes that majority of them are honest.

Particularly, \textbf{1)} in the setting of  no late joining or rejoining, the checkpoint idea is to provide resilience to such posterior corruption as long as there is no late joining or rejoining. Notably, if there is no majority posterior corruption, then the consistency property can be proved easily. If there exists a majority posterior corruption, alert nodes can be used to reject any chain that diverges from its current longest chain at a point sufficiently far back in the past (i.e., at least $\lambda$ time steps ago). In this way, old committee members that have since become corrupt cannot convince alert nodes to revise history that is too far back. In other words, the confirmed transaction log stabilizes and becomes immutable after a while.
Further, \textbf{2)} in the setting of late joining or rejoining. If there are no late spawning nodes, and if there are no nodes who wake up after sleeping for a long time, then the setting of no late joining or rejoining would work.
Thus, in Snow White, they assume that a newly joining node is provided with a list of nodes L the majority of whom must be alert ??? if so, the new node can ask the list of nodes in L to vote on the current state of the
system, and thus it will not be mislead to choose a ``simulated'' version of the history.









\subsection{Preventing an adaptive selection attack}
\par\noindent\textbf{Adaptive selection attack}.
An adaptive key selection attack implies that an adversary can break consistency with constant probability.
Specially, as the random oracle $H$ is chosen prior to protocol start, the adversary can make arbitrary queries to $H$.
Therefore, the adversary can spawn corrupt nodes and seed them with public keys that causes them to be elected leader at desirable points of time.
%
Since the adversary can query $H$, it is able to infer exactly in which time steps honest nodes are elected leader. Then the adversary can manage a corrupt node become a leader by picking corrupt nodes' public keys when an honest node is a leader.


The idea of snow white is to have nodes determine the next epoch's committee first, and then select the next epoch's hash -- in this way, the adversary will be unaware of next epoch's hash until well after the next committee is determined.


In a nutshell, they defeat the adaptively chosen key attack by determining the consensus committee $\lambda$ blocks earlier than the randomness seed, such that when corrupt nodes choose their public keys, they cannot predict the randomness seed, which will be generated much later in time and with sufficient entropy contributed by honest nodes. 




\subsection{Preventing the randomness-biasing attacks}
%\subsection{Achieving security under adversarially biased hashes}
\par\noindent\textbf{Adversarially biased hashes}.
It is easy to see the adversary can bias the nonce used to seed the hash, since the adversary can place arbitrary seeds in the blocks it contributes. In particular, suppose that the nonce is extracted from the prefix $chain[:\ell_1]$
Oblivious, with at least constant probability, the adversary may control the ending block in this prefix. By querying $H$ polynomially many times, the adversary can influence the seed in the last block chain $chain[:\ell_1]$ of the prefix, until it finds one that it likes.


Indeed, if each nonce is used only to select the leader in a small number of time steps (say, $O(1)$ time steps), such adversarial bias would indeed have been detrimental -- in particular, by enumerating polynomial many possibilities, the adversary can cause itself to be elected with probability almost 1 (assuming that the adversary controls the last block of the prefix).


However, as long as the same nonce is used sufficiently many times, the adversary cannot consistently cause corrupt nodes to be elected in many time steps. Specifically, suppose each nonce is used to elect at least $\Omega(\lambda)$ leaders, then except with $negl(\lambda)$ probability, the adversary cannot increase its share by more than an $negl$ function.






































==> body/framework.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex








Recent advances in quantum computing and the threat poses to classical cryptography has increased the interest in post-quantum cryptography research.
In particular, due to Shor's algorithm~\cite{FOCS:Shor94}, a quantum computer could easily factor a big integer in polynomial time, thus effectively break RSA. Implementations
of Shor's algorithm can also solve discrete logarithms and render today's digital signatures, such as DSA, ECDSA, and EdDSA~\footnote{DSA, ECDSA, and EdDSA rely on hardness assumptions about number theoretic problems, namely composite integer factorization and the computation of discrete logarithms.}, useless~\cite{QIC:ProZal03}.



Post-quantum cryptography provides a variety of quantum-resistant alternatives either lattice-based schemes or hash-based schemes to classical digital signature schemes. Below, we first revisit the classical digital signature schemes.


{\tiny
%\rowcolor[gray]{0.9}
\definecolor{Gray}{gray}{0.9}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\newcolumntype{a}{>{\columncolor{Gray}}c}
\newcolumntype{b}{>{\columncolor{white}}c}

\begin{table}[h!]
%\begin{sidewaystable}[h!] % <--
\small
\begin{center}
\begin{threeparttable}

    \caption{Overview of Post-Quantum Signature Schemes.}
    \label{table:pqsystem}
    \begin{tabular}{l l| a | b | a }%{ll|*{3}{l}}
      \toprule % <-- Toprule here
      %\multirow{2}{*}
      \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Performance}}} & \multicolumn{3}{c}{Size[Byte]}\\
      & &$\Sign$ & $\pk$  & $\sk$  \\
      [0.5ex]
      \midrule % <-- Midrule here
      %\rowcolor[gray]{0.9}
      \multirow{3}{*}{NTRU-based}
      & NTRU-GPV~\cite{AC:DucLyuPre14} & $\approx$ 1200 & 1792 &  NONE \\
      & BLISS-BI~\cite{C:DDLL13} & 717 & 896 & 256 \\
      & Falcon-512~\cite{FALCON17}$^{*}$ & 617 & 897 & 4097  \\
      \hdashline
      \multirow{2}{*}{Ring-based}
      & Dilithium-medium~\cite{TCHES:DKLLSSS18} & 2044 & 1184 &  2800 \\
      & Dilithium- & & & \\
      &recommended~\cite{TCHES:DKLLSSS18} & 2071 & 1472 & 3504 \\
      \hdashline
      \multirow{2}{*}{Lattice-based}
      & qTESLA-p-I~\cite{EPRINT:ABBLR19} & 2848 & 14880 & 5184 \\
      & qTESLA-p-III~\cite{EPRINT:ABBLR19} & 6176 & 39712 & 12352 \\
       \hdashline
      \multirow{3}{*}{MQ-based}
      & MQDSS-31-64~\cite{AC:CHRSS16} & 64  & 34032& 24 \\
      & HmFev(256,15,3,16)~\cite{IEICE:CLPYC18} & 61 &  83100& $\approx$20\\
      & Rainbow(16,32,32,32)~\cite{IEICE:CLPYC18} & 48 & 145500 & 18 \\
      \hdashline
      \multirow{3}{*}{Hash-based}
      & SPHINCS$^{+}-128$~\cite{EPRINT:ABBLR19} & 16976 & 32 & 64 \\
      & Picnic\_L1\_FS~\cite{EPRINT:ABBLR19} & 32944 & 33 & 49 \\
      & Picnic2\_L1\_FS~\cite{EPRINT:ABBLR19} & 12062 & 33 & 49 \\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
    \begin{tablenotes}
        \footnotesize
  \item[*] {https://falcon-sign.info/}
  \item[*] {\href{https://github.com/open-quantum-safe/liboqs}{https://github.com/open-quantum-safe/liboqs}}
      \end{tablenotes}
\end{threeparttable}
\end{center}
\vspace{-1em}
%\end{sidewaystable}
\end{table}
}





\subsection{Revisiting Lattice-based Signatures}
To our knowledge, lattice-based cryptography is more versatile than code-based, multivariate-quadratic (MQ), and hash-based cryptography, it has solid theoretical foundation and problems (\eg, CVP, SVP, SIS, and LWE) and can realize signature and encryption schemes. Regarding lattice-based signatures, there are two generic paradigms to obtain the lattice-based signature schemers~\cite{SAC:EFGT16}, one is \textit{hash-and-sign signature} paradigm, such as NTRUSign~\cite{CTRSA:HHPSW03}, Fixed NTRUSign~\cite{PQCRYPT:MBDG14}, Gentry, Peikert and Vaikuntanathan signature (GPVSign)~\cite{STOC:GenPeiVai08}, and Ducas, Lyubashevsky and Prest signature (DLPSign)~\cite{AC:DucLyuPre14}, and another is \textit{Fiat-Shamir signature} paradigm, such as Lyubashevsky signature~\cite{EC:Lyubashevsky12}, PASSSign~\cite{ACNS:HPSSW14},
G\"{u}neysu-Lyubashevsky-P\"{o}ppelmann (GLPSign) \cite{CHES:GunLyuPop12}, and BLISS~\cite{C:DDLL13}. Unfortunately for them, these schemes are less efficient and without the properties of uniqueness, and NTRUSign~\cite{CTRSA:HHPSW03} was already broken. Very recently, some new candidate lattice-based signatures are proposed one after the other and submitted to NIST Post-Quantum Cryptography Project, such as Falcon~\cite{FALCON17} and CRYSTALS-Dilithium~\cite{TCHES:DKLLSSS18} \etc. However, these schemes are still without the property of uniqueness.



%
%\begin{itemize}
%  \item \textbf{Hash-and-Sign Signatures}
%  \begin{itemize}
%    \item  NTRUSign [Hoffstein et al. 2003]~\cite{CTRSA:HHPSW03}  \zlinote{Broken}
%    \item Fixed NTRUSign [Melchor et al. 2014]
%    \item GPV [Gentry et al. 2008]  \zlinote{Less efficient }
%    \item DLP [Ducas et al. 2014]
%  \end{itemize}
%
%
%
%  \item \textbf{Fiat-Shamir Signatures}
%
%  \begin{itemize}
%       \item  LYU [Lyubashevsky 2012] \zlinote{Less efficient }
%    \item PASSSign [Hoffstein et al. 2014]
%    \item  GLP [Güneysu et al. 2012]
%    \item BLISS [Ducas et al. 2013]
%    \item BG [Bai and Galbraith 2014]
%  \end{itemize}


%
%\end{itemize}








%
%
%\paragraph{Falcon}
%
%
%``\emph{Falcon}''~(\ie.,~\href{https://falcon-sign.info}{https://falcon-sign.info}) is a cryptographic signature algorithm submitted to NIST Post-Quantum Cryptography Project on November 30th, 2017.
%In a nutshell, Falcon is based on the theoretical framework of Gentry, Peikert, and Vaikuntanathan~\cite{STOC:GenPeiVai08} for lattice-based signature schemes. We instantiate that framework over NTRU lattices, with a trapdoor sampler called ``fast Fourier sampling''. The underlying hard problem is the short integer solution problem (SIS) over NTRU lattices, for which no efficient solving algorithm is currently known in the general case, even with the help of quantum computers.
%
%\paragraph{Laguillaumie-Langlois-Libert-Stehle}
%
%Lattice-Based Group Signatures with Logarithmic Signature Size
%
%
%
%https://perso.ens-lyon.fr/damien.stehle/downloads/groupsig.pdf
%
%\paragraph{Akleylek-Bindel-Buchmann-Kramer-Marson}
%
%An Efficient Lattice-Based Signature Scheme with Provably Secure Instantiation
%ABBKGM~\cite{AFRICACRYPT:ABBKM16}
%
%
%
%https://eprint.iacr.org/2016/030.pdf
%
%
%
%\paragraph{CRYSTALS-Dilithium}
%CRYSTALS-Dilithium: A Lattice-Based Digital Signature Scheme
%
%
%https://eprint.iacr.org/2017/633.pdf
%
%
%
%
%\paragraph{Practical Lattice-Based Digital Signature Schemes}
%
%
%\href{https://pure.qub.ac.uk/ws/files/17361470/Practical_Lattice_based_Digital_Signature_Schemes_submit_version.pdf}{link}
%
%\href{https://pdfs.semanticscholar.org/2686/eb0daabee218502c4a3535259cef1e908c8d.pdf}{slides}
%







\subsection{Revisiting Practical Hash-based Signatures}
To our knowledge, the security of other post-quantum cryptographic schemes like lattice-based ones still objects to further research, but hash-based signatures are well understood.
There are many reasons to use hash-based signature schemes and to prefer those over other alternatives. In short, perhaps the oldest signature scheme with post-quantum security are one-time Lamport signatures, built using hash functions. In particular, hash-based signatures or Merkel signatures as they are also known, are one of the most promising of these alternatives for post-quantum signatures. Further, using a signature scheme always requires a hash function to reduce a message to a small representation of characters that can be signed easily. Importantly, other signature schemes rely on additional intractability assumptions to generate a signature, a hash-based solution only needs a secure hash function for the same procedure. Therefore the security of the scheme holds with the hash function used.



However, while today's hash-based schemes like XMSS are reasonably fast and yield small signatures, the current quantum-resistant hash-based signatures, such as SPHINCS\footnote{https://sphincs.cr.yp.to/papers.html}~\cite{EC:BHHLNPS15}, SPHINCS$^{+}$\footnote{https://sphincs.org/resources.html}~\cite{SPHINCS+}, and EPID signature~\cite{CTRSA:BonEskFis19} \etc, lack of practical performance and space requirements and lack of the property of uniqueness. Remarkably, Picnic is the first hash-based unique signature from symmetric-key proposed by Chase \etal~\cite{CCS:CDGORR17} using the ``Play-MPC-in-Head'' paradigm~\cite{STOC:IKOS07}. But the trouble is that the signature size of Picnic\footnote{https://microsoft.github.io/Picnic/} is about 40 KBytes, thus, various optimizations are proposed to short the length of the keys and signature and improve the computation performance~\cite{CCS:KatKolWan18,EC:DKPRR19}. In our work, we follow this research line and adopt the optimized Picnic signature with the 12KBytes signature size to design quantum resistant PoS. The detailed construction is shown in the following section.




\begin{comment}


  After that, some op














\subsubsection{Hash based Signature from symmetric-key primitives}  (i.e., one-time signature)


Due to Shor's algorithm, a quantum computer could easily factor a big integer in polynomial time, thus effectively break RSA. Implementations of Shor's algorithm can also solve discrete logarithms and render today's digital signatures, such as DSA, ECDSA, and EdDSA \etc.







While the very early Merkel Signature Scheme lacks practical performance and space requirements, today's hash-based schemes like XMSS are reasonably fast and yield small signatures. Also, the security requirements are compelling.


While other signature schemes rely on additional intractability assumptions to generate a signature, a hash-based solution only needs a secure hash function for the same procedure. Therefore the security of the scheme holds with the hash function used.



If the latter gets compromised, it can be replaced. The underlying Merkel scheme is not affected. Some hash-based schemes even reduce the need for a collision-resistant hash function to one that only needs to withstand attacks on the second-preimage. That gives you will get to know about security issues early as attacks in general aim on the stronger security assumption. As an example, practical attacks in means of the collision-resistance of the MD5 function are known, but we still do not know about virtual attacks on the second-preimage. With some schemes, other desirable features like forward security are available as well. A scheme being forward secure means that an attacker will not be able to get information about formerly used signature keys by getting hold of the current private key.


\end{comment}




%
%
%\zlinote{We need to adopt the signature to design our post-quantum blockchain consensus and distrusted public ledge}
%
%
%The post-quantum signature scheme should contain the following properties
%\begin{itemize}
%  \item Uniqueness, Unique signature (\ie, deterministic)
%  \item \zlinote{Stateless}, in short, the scheme does not require the signer to update the secret key after each invocation.
%
%      \zlimark{[cf.~\href{https://www.cs.bu.edu/~reyzin/teaching/cryptonotes/notes-9.pdf}{note-9}] Merkle's and Naor-Yung signature schemes have a serious drawback: they require the signer to keep some state from one signature to the next. That is, to sign, the signer needs not only the secret key but also information about what happened so far. If that information is incorrect, the signature scheme can be broken (because, for example, the signer might sign two messages with the same one-time key). Basically, in blockchain situation, keeping state is not allowed: the input to the signer is the secret key and the message to be signed, but nothing else.}
%
%
%  \item \zlinote{deterministic}
%  \item Quantum resistance
%  \item efficiency
%\end{itemize}
%
%\begin{remark}[Adopted from Lysyanskaya(EUROCRYPT2002)]
%Unique signatures are stateless. Since a unique signature is a function of the public key and the message, a signature on a given message will be the same whether this was the first message signed by the signer, or the $n$-the message. As a result, it is easy to see that the singer does not need to remember anything about past transactions, \ie, a unique signature must be stateless.
%\end{remark}
%
%
%\zlinote{Unique must be deterministic signature but the deterministic signature may not be a unique signature.}
%
%
%
%%
%%
%%\noindent{\textbf{Unique Digital Signing.}}
%%We also considering digital signature schemes $(\Gen,\Sign,\Vrfy)$ satisfying the following additional property.
%%
%%\begin{itemize}
%%     \item Uniqueness. It is hard to find strings $\pk'$, $\msg$, $\sigstr$ and $\sigstr'$ such that
%%\begin{equation*}
%%  \sigstr\neq \sigstr' ~\text{and}~ \Vrfy(\pk',\msg,\sigstr)=\Vrfy(\pk',\msg,\sigstr')=1.
%%\end{equation*}
%%
%%Note that the uniqueness property holds also for strings $\pk'$ that is not legitimately generated public keys.
%%
%%
%%In particular, however, the uniqueness property implies that, if one used the specified key generator $\Gen$ to compute a public key $\pk$ together with a matching secret key $\sk$, and thus knew $\sk$, it would be essentially impossible also for him to find two different digital signatures for the same message relative to $\pk$.)
%%\end{itemize}
%%
%%
%
%
%
%
%
%
%
%\zlinote{From unique signatures to verifiable random function (VRF).}
%
%Relative to a digital signature scheme with the uniqueness property, the mapping $\msg\to \hfuncH(\sigstr_i(\msg))$ associates to each possible string $\msg$, a unique, randomly selected, 256-bit string, and the correctness of this mapping can be proved given the signature $\sigstr_i(\msg)$.
%
%
%That is, ideal hashing and digital signature scheme satisfying the uniqueness property essentially provide an elementary implementation of a \emph{verifiable random function}, as introduced and by Micali, Rabin, and Vadhan~\cite{FOCS:MicRabVad99}.
%
%\zlinote{From VRF to Verifiable Delay Function}
%
%
%
%







Further, various post-quantum cryptosystems are proposed to prevent quantum computer attacks, such as code-based cryptography, lattice-based cryptography, and hash-based cryptography. Thus, in order to fulfill the main goal, we resort to this post-quantum cryptography. However, depending on our investigation as shown in the following Table~\ref{table:pqsystem}, if we adopt the ring-based or NTRU-based signature schemes, the size of the signature is approximate 2K Bytes and the size of the public key is approximate 17K Bytes. Sadly, if we adopt the hash-based signature scheme, the size of the public shrinks to 10K Bytes, but the size of the signature increases directly to 41K Bytes. Hence, we need to find trade-offs from these schemes.









\subsection{Post-Quantum Zero-Knowledge Proof}

There exist ZKPs that only use collision-resistant hash functions and hence are plausibly post quantum secure. Popular examples include Hyrax, Aurora,
$\ZKB$, $\ZKBpp$, and $\zkstark$.
%
Other notable ZKPs like Bulletproofs or libsnark rely on cryptographic assumptions which are known to be vulnerable to quantum attacks (e.g. hardness of discrete log in certain elliptic curve groups).




Today, two leading technologies are offering their cryptocurrencies, Monero and ZCash, and are striving to solve protection issues. Monero uses the Ring $\zkstark$s (Zero-knowledge scalable transparent argument of knowledge), a technology that provides the ability to conduct anonymous transactions.
%
$\zkstark$s aim to provide fast, scalable solutions to ensure financial security. In this way, transaction encryption is possible. $\zkstark$s were listed as one of the 10 Breakthrough Technologies of 2018. The fact that such widely-known organizations as R3 and Ethereum have already started to implement $\zkstark$s in their use cases is proof of the high potential of $\zksnark$s.
%
The following Table~\ref{table:pqnizk} for post-quantum security denotes that it is feasibly post-quantum secure.




{\tiny
%\rowcolor[gray]{0.9}
\definecolor{Gray}{gray}{0.9}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\newcolumntype{a}{>{\columncolor{Gray}}c}
\newcolumntype{b}{>{\columncolor{white}}c}

\begin{table}[h!]
%\begin{sidewaystable}[h!] % <--
\tiny
\begin{center}
\begin{threeparttable}

    \caption{Overview of Quantum-Resistant Proof Systems.}
    \label{table:pqnizk}
    \begin{tabular}{l|a b| a  b | a  b }%{ll|*{3}{l}}
      \toprule % <-- Toprule here
      %\multirow{2}{*}
      \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Scheme}}}
      & \multicolumn{2}{c|}{\underline{\textbf{Performance}}}
      & \multicolumn{2}{c|}{\underline{\textbf{Size}}}
      & \multicolumn{1}{c|}{\underline{\textbf{Assumption}}}
      & \multicolumn{1}{c|}{\underline{\textbf{Untrusted}}}\\
      & \textbf{Prover} & \textbf{Verifier} & \textbf{CRS} & \textbf{Proof}  & $\sk$ & \textbf{Setup} \\
      [0.5ex]
      \midrule % <-- Midrule here
      %\rowcolor[gray]{0.9}
      \multirow{1}{*}{$\ZKB$~\cite{USENIX:GiaMadOrl16}}
      &  &  &  &   & CRHF & \xmark \\
      \hdashline
      \multirow{1}{*}{$\ZKBpp$~\cite{CCS:CDGORR17}}
      &  &  &  &   & CRHF & \xmark \\
      \hdashline
      \multirow{4}{*}{Picnic}
      & Chase~\etal~\cite{CCS:CDGORR17} & \\
      & Katz~\etal~\cite{CCS:KatKolWan18} &  \\
      & Dinur~\etal~\cite{EC:DKPRR19} &  \\
      & Derler~\etal~\cite{PQCRYPTO:DerRamSla18} &  \\
       \hdashline
      \multirow{1}{*}{Ligero~\cite{CCS:AHIV17}}
      & $n\log{n}$ & $c\log{c}+h\log{h}$  & $0$ & $\sqrt{n}$ & CRHF & \cmark\\
      \hdashline
      \rowcolor[gray]{0.9}
      \multirow{1}{*}{$\zkstark$~\cite{EPRINT:BBHR18}}
      & $n\polylog{n}$ & $\polylog{n}$ & $0$ & $\log^2{n}$ & CRHF & \cmark\\
      \hdashline
      \multirow{1}{*}{Aurora~\cite{EC:BCRSVW19}}
      & $n\log{n}$ & $c\log{c}+h\log{h}$  & $0$ & $\sqrt{n}$ & CRHF & \cmark\\
      \hdashline
      \multirow{1}{*}{Bootle~\etal~\cite{AC:BCGGHJ17}}
      & $n$ & $n$ & $0$ & $\sqrt{n}$ & CRHF & \cmark\\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
    \begin{tablenotes}
        \footnotesize
  \item[*] {https://falcon-sign.info/}
  \item[-] Asymptotic efficiency comparison of zero-knowledge proofs for arithmetic circuits. Here n is the number of gates, $d$ is the depth of the circuit, $h$ is the width of the subcircuits, $c$ is the number of copies of the subcircuits, $\ell$ is the size of the instance, and $w$ is the size of the witness. An empty circle denotes that the scheme does not have this property and a full circle denotes that the scheme does have this property.
  \item[-]  DL stands for discrete log, CRHF stands for collision-resistant hash functions, KOE stands for knowledge-of-exponent, and AGM stands for algebraic group model.
  \item [-] \cmark~ denotes that the scheme does have this property.
  \item [-] \xmark~ denotes that the scheme does not have this property.
      \end{tablenotes}
\end{threeparttable}
\end{center}
\vspace{-1em}
%\end{sidewaystable}
\end{table}
}






Bulletproofs are short non-interactive zero-knowledge proofs that require no trusted setup. A bulletproof can be used to convince a verifier that an encrypted plaintext is well formed. For example, prove that an encrypted number is in a given range, without revealing anything else about the number. Compared to SNARKs, Bulletproofs require no trusted setup. However, verifying a bulletproof is more time consuming than verifying a SNARK proof.





==> body/paper-org.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex

TBD



%\subsection{Paper Organization}
%In Section \ref{sec:Preliminaries} we review related notions. In Section \ref{sec:SPHFfromRegev}, we describe our $\RSPHF$ scheme. In Section \ref{sec:SPHFfromMP}, we describe the improved $\SPHF$ over lattices. In Section \ref{sec:2flowPAKE}, we describe the proposed 2-flow $\PAKE$ protocol via our lattice-based $\SPHF$s. In Section \ref{sec:opt}, we present three ways to extend our scheme. In Section \ref{sec:conclusion}, we give a conclusion.






==> body/related.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex

%\zlinote{@Vishal, could you write the related works?}









Recent advances in quantum computing and the threat poses to classical cryptography has increased the interest in post-quantum cryptography research.
In particular, due to Shor's algorithm~\cite{FOCS:Shor94}, a quantum computer could easily factor a big integer in polynomial time, thus effectively break RSA. Implementations
of Shor's algorithm can also solve discrete logarithms and render today's digital signatures, such as DSA, ECDSA, and EdDSA~\footnote{DSA, ECDSA, and EdDSA rely on hardness assumptions about number theoretic problems, namely composite integer factorization and the computation of discrete logarithms.}, useless~\cite{QIC:ProZal03}.



Post-quantum cryptography provides a variety of quantum-resistant alternatives either lattice-based schemes or hash-based schemes to classical digital signature schemes. Below, we first revisit the classical digital signature schemes.


{\tiny
%\rowcolor[gray]{0.9}
\definecolor{Gray}{gray}{0.9}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\newcolumntype{a}{>{\columncolor{Gray}}c}
\newcolumntype{b}{>{\columncolor{white}}c}

\begin{table*}[h!]
%\begin{sidewaystable}[h!] % <--
\small%\normalsize%
\begin{center}
\begin{threeparttable}
    \caption{Overview of Post-Quantum Signature Schemes.}
    \label{table:pqsystem}
    \begin{tabular}{l l a  b  a }%{ll|*{3}{l}}
      \toprule % <-- Toprule here
      %\multirow{2}{*}
      \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Performance}}} & \multicolumn{3}{c}{Size[Byte]}\\
      & &$\Sign$ & $\pk$  & $\sk$  \\
      [0.5ex]
      \midrule % <-- Midrule here
      %\rowcolor[gray]{0.9}
      \multirow{3}{*}{NTRU-based}
      & NTRU-GPV~\cite{AC:DucLyuPre14} & $\approx$ 1200 & 1792 &  NONE \\
      & BLISS-BI~\cite{C:DDLL13} & 717 & 896 & 256 \\
      & Falcon-512~\cite{FALCON17}$^{*}$ & 617 & 897 & 4097  \\
      \hdashline
      \multirow{2}{*}{Ring-based}
      & Dilithium-medium~\cite{TCHES:DKLLSSS18} & 2044 & 1184 &  2800 \\
      & Dilithium- & & & \\
      &recommended~\cite{TCHES:DKLLSSS18} & 2071 & 1472 & 3504 \\
      \hdashline
      \multirow{2}{*}{Lattice-based}
      & qTESLA-p-I~\cite{EPRINT:ABBLR19} & 2848 & 14880 & 5184 \\
      & qTESLA-p-III~\cite{EPRINT:ABBLR19} & 6176 & 39712 & 12352 \\
       \hdashline
      \multirow{3}{*}{MQ-based}
      & MQDSS-31-64~\cite{AC:CHRSS16} & 64  & 34032& 24 \\
      & HmFev(256,15,3,16)~\cite{IEICE:CLPYC18} & 61 &  83100& $\approx$20\\
      & Rainbow(16,32,32,32)~\cite{IEICE:CLPYC18} & 48 & 145500 & 18 \\
      \hdashline
      \multirow{3}{*}{Hash-based}
      & SPHINCS$^{+}-128$~\cite{EPRINT:ABBLR19} & 16976 & 32 & 64 \\
      & Picnic\_L1\_FS~\cite{EPRINT:ABBLR19} & 32944 & 33 & 49 \\
      & Picnic2\_L1\_FS~\cite{EPRINT:ABBLR19} & 12062 & 33 & 49 \\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
    \begin{tablenotes}
        \footnotesize
  \item[*] {https://falcon-sign.info/}
  \item[*] {\href{https://github.com/open-quantum-safe/liboqs}{https://github.com/open-quantum-safe/liboqs}}
      \end{tablenotes}
\end{threeparttable}
\end{center}
\vspace{-1em}
%\end{sidewaystable}
\end{table*}
}





\subsection{Revisiting Lattice-based Signatures}
To our knowledge, lattice-based cryptography is more versatile than code-based, multivariate-quadratic (MQ), and hash-based cryptography, it has solid theoretical foundation and problems (\eg, CVP, SVP, SIS, and LWE) and can realize signature and encryption schemes. Regarding lattice-based signatures, there are two generic paradigms to obtain the lattice-based signature schemers~\cite{SAC:EFGT16}, one is \textit{hash-and-sign signature} paradigm, such as NTRUSign~\cite{CTRSA:HHPSW03}, Fixed NTRUSign~\cite{PQCRYPT:MBDG14}, Gentry, Peikert and Vaikuntanathan signature (GPVSign)~\cite{STOC:GenPeiVai08}, and Ducas, Lyubashevsky and Prest signature (DLPSign)~\cite{AC:DucLyuPre14}, and another is \textit{Fiat-Shamir signature} paradigm, such as Lyubashevsky signature~\cite{EC:Lyubashevsky12}, PASSSign~\cite{ACNS:HPSSW14},
G\"{u}neysu-Lyubashevsky-P\"{o}ppelmann (GLPSign) \cite{CHES:GunLyuPop12}, and BLISS~\cite{C:DDLL13}. Unfortunately for them, these schemes are less efficient and without the properties of uniqueness, and NTRUSign~\cite{CTRSA:HHPSW03} was already broken. Very recently, some new candidate lattice-based signatures are proposed one after the other and submitted to NIST Post-Quantum Cryptography Project, such as Falcon~\cite{FALCON17} and CRYSTALS-Dilithium~\cite{TCHES:DKLLSSS18} \etc. However, these schemes are still without the property of uniqueness.



%
%\begin{itemize}
%  \item \textbf{Hash-and-Sign Signatures}
%  \begin{itemize}
%    \item  NTRUSign [Hoffstein et al. 2003]~\cite{CTRSA:HHPSW03}  \zlinote{Broken}
%    \item Fixed NTRUSign [Melchor et al. 2014]
%    \item GPV [Gentry et al. 2008]  \zlinote{Less efficient }
%    \item DLP [Ducas et al. 2014]
%  \end{itemize}
%
%
%
%  \item \textbf{Fiat-Shamir Signatures}
%
%  \begin{itemize}
%       \item  LYU [Lyubashevsky 2012] \zlinote{Less efficient }
%    \item PASSSign [Hoffstein et al. 2014]
%    \item  GLP [Güneysu et al. 2012]
%    \item BLISS [Ducas et al. 2013]
%    \item BG [Bai and Galbraith 2014]
%  \end{itemize}


%
%\end{itemize}








%
%
%\paragraph{Falcon}
%
%
%``\emph{Falcon}''~(\ie.,~\href{https://falcon-sign.info}{https://falcon-sign.info}) is a cryptographic signature algorithm submitted to NIST Post-Quantum Cryptography Project on November 30th, 2017.
%In a nutshell, Falcon is based on the theoretical framework of Gentry, Peikert, and Vaikuntanathan~\cite{STOC:GenPeiVai08} for lattice-based signature schemes. We instantiate that framework over NTRU lattices, with a trapdoor sampler called ``fast Fourier sampling''. The underlying hard problem is the short integer solution problem (SIS) over NTRU lattices, for which no efficient solving algorithm is currently known in the general case, even with the help of quantum computers.
%
%\paragraph{Laguillaumie-Langlois-Libert-Stehle}
%
%Lattice-Based Group Signatures with Logarithmic Signature Size
%
%
%
%https://perso.ens-lyon.fr/damien.stehle/downloads/groupsig.pdf
%
%\paragraph{Akleylek-Bindel-Buchmann-Kramer-Marson}
%
%An Efficient Lattice-Based Signature Scheme with Provably Secure Instantiation
%ABBKGM~\cite{AFRICACRYPT:ABBKM16}
%
%
%
%https://eprint.iacr.org/2016/030.pdf
%
%
%
%\paragraph{CRYSTALS-Dilithium}
%CRYSTALS-Dilithium: A Lattice-Based Digital Signature Scheme
%
%
%https://eprint.iacr.org/2017/633.pdf
%
%
%
%
%\paragraph{Practical Lattice-Based Digital Signature Schemes}
%
%
%\href{https://pure.qub.ac.uk/ws/files/17361470/Practical_Lattice_based_Digital_Signature_Schemes_submit_version.pdf}{link}
%
%\href{https://pdfs.semanticscholar.org/2686/eb0daabee218502c4a3535259cef1e908c8d.pdf}{slides}
%







\subsection{Revisiting Practical Hash-based Signatures}
To our knowledge, the security of other post-quantum cryptographic schemes like lattice-based ones still objects to further research, but hash-based signatures are well understood.
There are many reasons to use hash-based signature schemes and to prefer those over other alternatives. In short, perhaps the oldest signature scheme with post-quantum security are one-time Lamport signatures, built using hash functions. In particular, hash-based signatures or Merkel signatures as they are also known, are one of the most promising of these alternatives for post-quantum signatures. Further, using a signature scheme always requires a hash function to reduce a message to a small representation of characters that can be signed easily. Importantly, other signature schemes rely on additional intractability assumptions to generate a signature, a hash-based solution only needs a secure hash function for the same procedure. Therefore the security of the scheme holds with the hash function used.



However, while today's hash-based schemes like XMSS are reasonably fast and yield small signatures, the current quantum-resistant hash-based signatures, such as SPHINCS\footnote{https://sphincs.cr.yp.to/papers.html}~\cite{EC:BHHLNPS15}, SPHINCS$^{+}$\footnote{https://sphincs.org/resources.html}~\cite{SPHINCS+}, and EPID signature~\cite{CTRSA:BonEskFis19} \etc, lack of practical performance and space requirements and lack of the property of uniqueness. Remarkably, Picnic is the first hash-based unique signature from symmetric-key proposed by Chase \etal~\cite{CCS:CDGORR17} using the ``Play-MPC-in-Head'' paradigm~\cite{STOC:IKOS07}. But the trouble is that the signature size of Picnic\footnote{https://microsoft.github.io/Picnic/} is about 40 KBytes, thus, various optimizations are proposed to short the length of the keys and signature and improve the computation performance~\cite{CCS:KatKolWan18,EC:DKPRR19}. In our work, we follow this research line and adopt the optimized Picnic signature with the 12KBytes signature size to design quantum-resistant PoS. The detailed construction is shown in the following section.



\begin{comment}


  After that, some op














\subsubsection{Hash based Signature from symmetric-key primitives}  (i.e., one-time signature)


Due to Shor's algorithm, a quantum computer could easily factor a big integer in polynomial time, thus effectively break RSA. Implementations of Shor's algorithm can also solve discrete logarithms and render today's digital signatures, such as DSA, ECDSA, and EdDSA \etc.







While the very early Merkel Signature Scheme lacks practical performance and space requirements, today's hash-based schemes like XMSS are reasonably fast and yield small signatures. Also, the security requirements are compelling.


While other signature schemes rely on additional intractability assumptions to generate a signature, a hash-based solution only needs a secure hash function for the same procedure. Therefore the security of the scheme holds with the hash function used.



If the latter gets compromised, it can be replaced. The underlying Merkel scheme is not affected. Some hash-based schemes even reduce the need for a collision-resistant hash function to one that only needs to withstand attacks on the second-preimage. That gives you will get to know about security issues early as attacks in general aim on the stronger security assumption. As an example, practical attacks in means of the collision-resistance of the MD5 function are known, but we still do not know about virtual attacks on the second-preimage. With some schemes, other desirable features like forward security are available as well. A scheme being forward secure means that an attacker will not be able to get information about formerly used signature keys by getting hold of the current private key.


\end{comment}




%
%
%\zlinote{We need to adopt the signature to design our post-quantum blockchain consensus and distrusted public ledge}
%
%
%The post-quantum signature scheme should contain the following properties
%\begin{itemize}
%  \item Uniqueness, Unique signature (\ie, deterministic)
%  \item \zlinote{Stateless}, in short, the scheme does not require the signer to update the secret key after each invocation.
%
%      \zlimark{[cf.~\href{https://www.cs.bu.edu/~reyzin/teaching/cryptonotes/notes-9.pdf}{note-9}] Merkle's and Naor-Yung signature schemes have a serious drawback: they require the signer to keep some state from one signature to the next. That is, to sign, the signer needs not only the secret key but also information about what happened so far. If that information is incorrect, the signature scheme can be broken (because, for example, the signer might sign two messages with the same one-time key). Basically, in blockchain situation, keeping state is not allowed: the input to the signer is the secret key and the message to be signed, but nothing else.}
%
%
%  \item \zlinote{deterministic}
%  \item Quantum resistance
%  \item efficiency
%\end{itemize}
%
%\begin{remark}[Adopted from Lysyanskaya(EUROCRYPT2002)]
%Unique signatures are stateless. Since a unique signature is a function of the public key and the message, a signature on a given message will be the same whether this was the first message signed by the signer, or the $n$-the message. As a result, it is easy to see that the singer does not need to remember anything about past transactions, \ie, a unique signature must be stateless.
%\end{remark}
%
%
%\zlinote{Unique must be deterministic signature but the deterministic signature may not be a unique signature.}
%
%
%
%%
%%
%%\noindent{\textbf{Unique Digital Signing.}}
%%We also considering digital signature schemes $(\Gen,\Sign,\Vrfy)$ satisfying the following additional property.
%%
%%\begin{itemize}
%%     \item Uniqueness. It is hard to find strings $\pk'$, $\msg$, $\sigstr$ and $\sigstr'$ such that
%%\begin{equation*}
%%  \sigstr\neq \sigstr' ~\text{and}~ \Vrfy(\pk',\msg,\sigstr)=\Vrfy(\pk',\msg,\sigstr')=1.
%%\end{equation*}
%%
%%Note that the uniqueness property holds also for strings $\pk'$ that is not legitimately generated public keys.
%%
%%
%%In particular, however, the uniqueness property implies that, if one used the specified key generator $\Gen$ to compute a public key $\pk$ together with a matching secret key $\sk$, and thus knew $\sk$, it would be essentially impossible also for him to find two different digital signatures for the same message relative to $\pk$.)
%%\end{itemize}
%%
%%
%
%
%
%
%
%
%
%\zlinote{From unique signatures to verifiable random function (VRF).}
%
%Relative to a digital signature scheme with the uniqueness property, the mapping $\msg\to \hfuncH(\sigstr_i(\msg))$ associates to each possible string $\msg$, a unique, randomly selected, 256-bit string, and the correctness of this mapping can be proved given the signature $\sigstr_i(\msg)$.
%
%
%That is, ideal hashing and digital signature scheme satisfying the uniqueness property essentially provide an elementary implementation of a \emph{verifiable random function}, as introduced and by Micali, Rabin, and Vadhan~\cite{FOCS:MicRabVad99}.
%
%\zlinote{From VRF to Verifiable Delay Function}
%
%
%
%







Further, various post-quantum cryptosystems are proposed to prevent quantum computer attacks, such as code-based cryptography, lattice-based cryptography, and hash-based cryptography. Thus, in order to fulfill the main goal, we resort to this post-quantum cryptography. However, depending on our investigation as shown in the following Table~\ref{table:pqsystem}, if we adopt the ring-based or NTRU-based signature schemes, the size of the signature is approximate 2K Bytes and the size of the public key is approximate 17K Bytes. Sadly, if we adopt the hash-based signature scheme, the size of the public shrinks to 10K Bytes, but the size of the signature increases directly to 41K Bytes. Hence, we need to find trade-offs from these schemes.









\subsection{Revisiting Post-Quantum Zero-Knowledge}

There exist ZKPs that only use collision-resistant hash functions and hence are plausibly post-quantum secure. Popular examples include Hyrax, Aurora,
$\ZKB$, $\ZKBpp$, and $\zkstark$.
%
Other notable ZKPs like Bulletproofs or libsnark rely on cryptographic assumptions that are known to be vulnerable to quantum attacks (e.g. hardness of discrete log in certain elliptic curve groups).




Today, two leading technologies are offering their cryptocurrencies, Monero and ZCash, and are striving to solve protection issues. Monero uses the Ring $\zkstark$s (Zero-knowledge scalable transparent argument of knowledge), a technology that provides the ability to conduct anonymous transactions.
%
$\zkstark$s aim to provide fast, scalable solutions to ensure financial security. In this way, transaction encryption is possible. $\zkstark$s were listed as one of the 10 Breakthrough Technologies of 2018. The fact that such widely-known organizations as R3 and Ethereum have already started to implement $\zkstark$s in their use cases is proof of the high potential of $\zksnark$s.
%
The following Table~\ref{table:pqnizk} for post-quantum security denotes that it is asymptotic efficiency comparison of zero-knowledge proofs for arithmetic circuits.



{
%
%\rowcolor[gray]{0.9}
\definecolor{Gray}{gray}{0.9}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\newcolumntype{a}{>{\columncolor{Gray}}c}
\newcolumntype{b}{>{\columncolor{white}}c}

\begin{table*}[h!]
%\begin{sidewaystable}[h!] % <--
\normalsize%\small%\tiny
\begin{center}
\begin{threeparttable}
    \caption{Overview of Feasibly Quantum-Resistant Proof Systems.}
    \label{table:pqnizk}
    \begin{tabular}{l a b a  b  a  b }%{ll|*{3}{l}}
      \toprule % <-- Toprule here
      %\multirow{2}{*}
      \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Scheme}}}
      & \multicolumn{2}{c}{\underline{\textbf{Performance}}}
      & \multicolumn{2}{c}{\underline{\textbf{Size}}}
      & \multicolumn{1}{c}{\underline{\textbf{Assumption}}}
      & \multicolumn{1}{c}{\underline{\textbf{Untrusted}}}\\
      & \textbf{Prover} & \textbf{Verifier} & \textbf{CRS} & \textbf{Proof}  & $\sk$ & \textbf{Setup} \\
      [0.5ex]
      \midrule % <-- Midrule here
      %\rowcolor[gray]{0.9}
      \multirow{1}{*}{$\ZKB$~\cite{USENIX:GiaMadOrl16}}
      & $n\log{n}$ & $c\log{c}+h\log{h}$  & $n$ & $\sqrt{n}$ & CRHF & \xmark\\
      \hdashline
      %\multirow{1}{*}{$\ZKBpp$~\cite{CCS:CDGORR17}}
      %& $n\log{n}$ & $c\log{c}+h\log{h}$  & $n$ & $\sqrt{n}$ & CRHF & \xmark \\
      % \hdashline
      \multirow{1}{*}{Ligero~\cite{CCS:AHIV17}}
      & $n\log{n}$ & $c\log{c}+h\log{h}$  & $0$ & $\sqrt{n}$ & CRHF & \cmark\\
      \hdashline
      \rowcolor[gray]{0.9}
      \multirow{1}{*}{$\zkstark$~\cite{EPRINT:BBHR18}}
      & $n\polylog{n}$ & $\polylog{n}$ & $0$ &  $\log^2{n}$ & CRHF & \cmark\\
      \hdashline
      \multirow{1}{*}{Aurora~\cite{EC:BCRSVW19}}
      & $n\log{n}$ & $c\log{c}+h\log{h}$  & $0$ & $\sqrt{n}$ & CRHF & \cmark\\
      \hdashline
      \multirow{1}{*}{Bootle~\etal~\cite{AC:BCGGHJ17}}
      & $n$ & $n$ & $0$ & $\sqrt{n}$ & CRHF & \cmark\\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
    \begin{tablenotes}
        %\footnotesize
  %\item[*] {https://falcon-sign.info/}
  \item [-] The communication complexity of $\ZKBpp$ is more than halved compared to $\ZKB$, not affecting the computational complexity. This is done by using six different optimizations that are designed to compress all messages sent as much as possible.
  \item[-]  Here $n$ is the number of gates, $d$ is the depth of the circuit, $h$ is the width of the subcircuits, $c$ is the number of copies of the subcircuits, $\ell$ is the size of the instance, and $w$ is the size of the witness.
  %\item[-] An empty circle denotes that the scheme does not have this property and a full circle denotes that the scheme does have this property.
  \item[-]  %DL stands for discrete log, KOE stands for knowledge-of-exponent, and AGM stands for algebraic group model,
  CRHF stands for collision-resistant hash functions.
  \item [-] \cmark~ denotes that the scheme does have this property.
  \item [-] \xmark~ denotes that the scheme does not have this property.
      \end{tablenotes}
\end{threeparttable}
\end{center}
\vspace{-1em}
%\end{sidewaystable}
\end{table*}
}
%       Chase~\etal~\cite{CCS:CDGORR17} & \\
%       Katz~\etal~\cite{CCS:KatKolWan18} &  \\
%       Dinur~\etal~\cite{EC:DKPRR19} &  \\
%       Derler~\etal~\cite{PQCRYPTO:DerRamSla18} &  \\




Bulletproofs are short non-interactive zero-knowledge proofs that require no trusted setup. A bulletproof can be used to convince a verifier that an encrypted plaintext is well-formed. For example, prove that an encrypted number is in a given range, without revealing anything else about the number. Compared to SNARKs, Bulletproofs require no trusted setup. However, verifying a bulletproof is more time consuming than verifying a SNARK proof.















\subsection{Revisiting Blockchain}
The security of the blockchain is motivated by the strength of their consensus schemes. The hosted platform can be secured based on the security of the ledger sharing between the entities. The nodes having quantum powers are theoretically bound to affect the blockchain's consensus. Thus, it is desired to understand the existing consensus schemes from the perspectives of the post-quantum era. The liveliness and security of the distributed ledgers cannot be assured through the existing PoW or PoS mechanisms in the quantum world. Especially, the synchronization by the non-quantum nodes may prove to be extremely difficult leading to several attacks from the quantum nodes by modifying the chains from earlier instances~\cite{karame2016bitcoin}. It has to be seen with considerable importance that attacks such as stake-grinding may lead to unwanted centralization, thus, giving control to a single quantum node. Furthermore, the group-quantum attack may fail several applications which are based on the correctness of the underlying blockchain architecture. Quantum attacks have the ability to violate the core principles of the public ledgers as these may control the openness and availability of the participants. Additionally, easiness of crypto constructions with quantum is a huge challenge to be taken care of by the construction schemes used for defining the consensus in the present blockchain architectures.

At present, the solutions pertaining to different types of consensus are efficient and secure against several known attacks, but their worth for security against unknown cyber threats is yet to be proven. Considering PoW, there are many studies as well as variants proposed to increase its efficiency without compromising the performance in terms of the number of transactions per second. Although the studies define PoW provably secure against known attacks, especially towards the 51\% attacks, it becomes severe if any of the network nodes show quantum-level computations. Under such circumstances, the current solutions may not comply because of their computational limitations and the inability to identify such threats. Stewart et al.\cite{stewart2018committing} proposed an approach that utilizes slow commit–delay–reveal protocol to allow users to move their funds in case of quantum threats to the ongoing blockchain. Although, their approach provides a strongly favorable aspect over~\cite{bonneau2014fawkescoin}, yet it requires a key aspect of delay-modeling. Because of such an issue, this approach may not be handy when large consensus is exploited using quantum computations. Moreover, the group quantum attacks may hinder the applicability of this approach. Abelian Coin (ABE)~\cite{liukey} offers a strong platform for building blockchain which is secure against the post-quantum attacks. The article lists the technicalities which can help to attain the common blockchain platform resilient to post-quantum attacks.

The fixed assumptions of the BFT consensus and performance security trade-offs of Nakamoto's consensus prohibit any approach which is ideally based on their flow to be used in the post-quantum era~\cite{xiao2019survey}. Compared to PoW, the PoS consensus is computationally inexpensive to attack, but a proper penalty method and attack resilience framework can make it a worthy candidate for the quantum-resilient blockchain. Moreover, lesser dependencies on the computational resources of the nodes make it an ideal candidate to be used in futuristic-blockchain. However, there are certain limitations of the existing PoS consensus schemes which prohibit their utility in the post-quantum era. For instance, the committee-based PoS (Ouroboros~\cite{C:KRDO17} and Ouroboros Praos~\cite{EC:DGKR18}) require participants to form an efficient regime to operate the consensus. With quantum computations, an attacker may obtain major stakes in the chain while populating the entire chain with its own blocks leading to nondeterministic folks as well as long-range attacks. Chain-based PoS (Ppcoin~\cite{king2012ppcoin} and Nxt~\cite{wiki:xxx}) are the most dominant types of PoS consensus which are also the primary target of the permissionless blockchain formations. However, such a consensus suffers from the waiting issues, which decreases participation. Considering this, a quantum node can resist the joining of new blocks from the other participants, thus, taking control over the entire chain. Such an issue is yet open and not provably secured from the perspectives of post-quantum applications. Similar issues are exploitable in delegated PoS (EOS.IO~\cite{io2018eos}) with major of them having concerns of falling prey to Nothing-at-stake attacks in the post-quantum era. All these consensus schemes are difficult to operate because of their quantum vulnerabilities, especially blockchain's with digital signatures are easier to fail as quantum computations are expected to solve exponential time problems in few minutes~\cite{ben2018scalable}. Thus, the current batch of PoS schemes cannot be leveraged for post-quantum blockchain deployment. Additionally, cold staking (https://particl.io) is one of the emerging applications of the blockchain which enables stakeholders to earn passive income by keeping their shares online. Such an application possesses an extreme requirement of quantum resilience platform as a quantum attack can remodel the entire chain from the long-history causing losses to many users.







\subsection{Revisiting potential attacks}

\zlinote{New, TBD}
\par\noindent\textbf{Grinding attacks} implies that a miner re-creates a block multiple
times until it is likely that the miner can create a second block
shortly afterwards. This attack can be mitigated (even thwarted) by ensuring
that a miner is not able to influence the next leader election
by using an unbiasable source of randomness or a deterministic
leader election. 



\par\noindent\textbf{Long-range attack} implies that
an attacker can bribe miners to sell their private keys






























\begin{comment}



%
%
%In this setting, the unique digital is proposing inevitably\psz{don't get the sentence}.
%To our knowledge, the unique digital signatures have only one valid signature for the message $m$ with the corresponding public key $\pk$, and can be constructed from standard cryptographic assumptions.
%\psz{this sentence sounds a bit strange too. To our knowledge? I thought it is just a fact}

%\begin{figure}[h]
%  \centering
%  \includegraphics[width=0.4\textwidth]{Ours.png}
%  \caption{XXXXX}\label{table:pqsystem}
%\end{figure}

%
%{\tiny
%\begin{table}[h!]
%%\begin{sidewaystable}[h!] % <--
%\small
%\begin{center}
%\begin{threeparttable}
%
%    \caption{Parameters.}
%    \label{tab:table1}
%    \begin{tabular}{c*{4}{l}}
%      \toprule % <-- Toprule here
%      \multicolumn{2}{*}{\multirow{2}{*}{\textbf{Performance}}}  & \multicolumn{3}{*}{Size [Bytes]} \\
%       & $\Sign$ & $\pk$  & $\sk$  \\
%      [0.5ex]
%      \midrule % <-- Midrule here
%     \multirow{3}{*}{One-round}
%     & NTRU-GPV~\cite{AC:DucLyuPre14} & $\approx$ 1200 & 1792 &  \\
%       \rowcolor[gray]{0.9}
%     & BLISS-BI~\cite{C:DDLL13} & 717 & 896 & 256 \\
%     & Falcon-512~\cite{FALCON17}\footnote{https://falcon-sign.info/} & 617 & 897 & 4097 \\
%
%
%      \bottomrule % <-- Bottomrule here
%    \end{tabular}
%    \begin{tablenotes}
%        \footnotesize
%  \item[-]
%      \end{tablenotes}
%
%\end{threeparttable}
%
%\end{center}
%%\vspace{-3em}
%%\end{sidewaystable}
%\end{table}
%}








%To design the size-efficiency unique signature scheme, we investigate existing efficient post-quantum signature schemes.
%As shown in the following Table~\ref{table:pqsystem}, if we adopt the ring-based or NTRU-based signature schemes, the size of the signature is approximate 2K Bytes and the size of the public key is approximate 17K Bytes. Sadly, if we adopt the hash-based signature scheme, the size of the public shrinks to 10K Bytes, but the size of the signature increases directly to 41K Bytes. In this case, we attempt to target the hash-based optimized Picnic scheme which signature size is about 12K Bytes, it's a great trade-off in terms of the size of the public key and signature compared with lattice-based and hash-based schemes.
%%












\zlidel{
%
Goldwasser and Ostrovsky~\cite{C:GolOst92} introduced invariant signature that is called unique signature afterwards, and they shown how to build VRFs via unique signature. In Algorand~\cite{Algorand16}, Chen and Micali mentioned how to obtain VRFs from a unique signature. Thus, the key to the instantiation of post-quantum VRF is how to design a post-quantum unique signature scheme.









In Algorand~\cite{Algorand16}, the authors observed that if a digital signature scheme with the uniqueness property, then ideal hashing and unique signature provide an elementary implementation of a VRF, as introduced and by Micali, Rabin, and Vadhan~\cite{FOCS:MicRabVad99}. Thus, if we can obtain a quantum-resistance \textit{unique} signature, then we can obtain post-quantum VRF via the quantum-resistance unique signature in a fairly straightforward way. Sadly, to construct a practical unique signature is non-trivial. For example, ECDSA signatures are malleable: if $(x(R),s)$ is an ECDSA signature, then so is $(x(-R),-s)=(x(R),-s)$. EdDSA signatures, of the form $(R,s)$ instead, hash $R$ together with the message so it can't be changed any more than the message can, but $(R,s+\ell)$ makes another valid signature if encodable, where $\ell$ is the order of the standard base point.
%
%
%Further, ECDSA, and EdDSA are necessarily randomized, and the signer can choose any per-signature secret nonce they want without the verifier noticing. Standard EdDSA prescribes a particular nonce so that the signer doesn't accidentally leak the private key when signing two different messages, but verifiers can't tell if a signer uses a different nonce.
%
%
Furthermore, to design the size-efficiency unique signature scheme, we investigate existing efficient post-quantum signature schemes as shown in the Table~\ref{table:pqsystem}.
\zli{MAC+ZK-SNARK}




%
However, both these schemes (and many others) use cryptographic primitives and constructions insecure in the post-quantum world. To tackle this problem, in this work we design a practical quantum-resistance PoS protocol.
}



%\zlinote{The following references can be considered. }

\begin{itemize}
     \item Bitcoin Backbone~: Garay, Kiayisa and Leonardo~\cite{EC:GarKiaLeo15,C:GarKiaLeo17}
  \item Ouroboros:~Kiayias, Russell, David, Oliynkov~\cite{C:KRDO17}~eprint2016/889.
  \item Snow white:~Bentov, Pass, and Shi~\cite{EPRINT:BenPasShi16b}~eprint2016/919.
  \item Ouroboros~Praos:~David, Gazi, Kiayias, Russell~\cite{EC:DGKR18}.
  \item Ouroboros~Crypsionous:~\cite{EPRINT:KKKZ18}~eprint2018/1132.
  \item iChang: Fan and Zhou~\cite{EPRINT:FanZho17}~eprint2017/666.
  \item Ouroboros-BFT: Kiayias and Russell~\cite{EPRINT:KiaRus18}~eprint2018/1049.
\end{itemize}


\begin{table*}[ht!]%[ht]
\begin{center}
\begin{threeparttable}
%\vspace{-0.6mm}
\vspace{10pt}
\caption{Comparetion of Blockchain Consensus }\label{table:XXXX}
%\resizebox{\textwidth}{15mm}{
%r l l l l
\begin{tabular}{l @{\quad}l   @{\quad}l  @{\quad}l  @{\quad}l}
\hline\rule{0pt}{12pt} %\toprule
  Scheme & Static Setting & Permissionless & Players are fixed & Synchronous \\
    \hdashline
 & Dynamic &  Permissioned &  & Asynchronous \\
\hline \hline\rule{0pt}{12pt} %\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  Nakamoto &\cmark &\cmark &\cmark &\cmark\\
  GKL &\cmark &\cmark &\cmark &\cmark(without delays, i.e.,$\Delta=1$)\\
  PSS &\cmark &\cmark &\cmark &\xmark($\Delta$-bounded delays)\\
\hline
%\end{longtable}
\end{tabular}
%}

\vspace{1ex}

\centering
\begin{tablenotes}
        \footnotesize
\begin{minipage}{0.4\textwidth}%{2in}
    %\begin{itemize}
    \item[-]
    %\end{itemize}
  \end{minipage}%
%\hspace*{17mm}
  \begin{minipage}{0.4\textwidth}%{2in}
     %\begin{itemize}
 \item [-] C: check;
    %\end{itemize}
\end{minipage}
\vspace{1ex}
\item[*] We remark that XXXX in Table~\ref{table:XXXXX}.
\end{tablenotes}
\end{threeparttable}

\end{center}
\end{table*}
%\vspace{-5pt}














\begin{table*}[ht!]%[ht]
\begin{center}
\begin{threeparttable}
%\vspace{-0.6mm}
\vspace{10pt}
\caption{Blockchain Consensus Classification}\label{table:XXXX}
%\resizebox{\textwidth}{15mm}{
%r l l l l
\begin{tabular}{ @{\quad}l @{\quad}l @{\quad}l @{\quad}l  @{\quad}l }
\hline\rule{0pt}{12pt} %\toprule
 POW  & POS & DPOS &  PBFT\\
\hline \hline\rule{0pt}{12pt} %\midrule
Bitcoin Backbone~\cite{EC:GarKiaLeo15} & Ouroboros~\cite{C:KRDO17} &  \\
&  Snow white~\cite{EPRINT:BenPasShi16b} &\\
& iChang~\cite{EPRINT:FanZho17}\\
& Ouroboros~Praos~\cite{EC:DGKR18}& \\
& Ouroboros~Crypsionous:~\cite{EPRINT:KKKZ18} &\\
 &&& Ouroboros-BFT~\cite{EPRINT:KiaRus18} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline
%\end{longtable}
\end{tabular}
%}

\vspace{1ex}

\centering
\begin{tablenotes}
        \footnotesize
\begin{minipage}{0.4\textwidth}%{2in}
    %\begin{itemize}
\item[-] DPOS: Delegated POS
     \item[-] PBFT:~Pratical Byzantine fault tolerant mechanism.
    %\end{itemize}
  \end{minipage}%
%\hspace*{17mm}
  \begin{minipage}{0.4\textwidth}%{2in}
     %\begin{itemize}
 \item [-] C: check;
    %\end{itemize}
\end{minipage}
\vspace{1ex}
\item[*] We remark that XXXX in Table~\ref{table:XXXXX}.
\end{tablenotes}
\end{threeparttable}

\end{center}
\end{table*}
%\vspace{-5pt}












\noindent{\textbf{Blockchain Protocols.}}
In a blockchain protocol, the goal of all parties is to maintain a (consistent) global ordered set of records.  The set of records is ``append only'', and publicly visible. Furthermore, the record can only be added using a special mechanism to reach a consensus on what must be added to the existing blockchain. A protocol can employ any arbitrary technique or mechanism for participants to converge on a uniform and reliable blockchain state.
In most cryptocurrencies instantiated in the blockchain model, the special mechanism to reach consensus is called a mining procedure.
It is used by all parties to extend the blockchain (\ie, add new blocks) and in turn (potentially) receive rewards for successfully generating a new block consistent with respect to the current blockchain state.



The mining procedure is meant to simulate a \emph{puzzle-solving} race between protocol participants and could be run by any party. The rewards mostly consist of freshly generated currency. Presently, the mining procedures employed by most cryptocurrencies could be classified into two broad categories ---- proof-of-work (PoW) and proof-of-state (PoS) based puzzles. The basic difference being that
\begin{itemize}
  \item [-] In PoW puzzles, the probability of successful mining is proportional to the amount of computational power;
  \item [-] whereas in PoS, it is proportional to the number of coins in the possession of a miner.
\end{itemize}

Therefore, PoW miners have to spend a significant portion of their computational resources (and in turn, monetary resources) to extend the blockchain and in turn get rewarded, whereas POS miners spend significantly less computational resources and just need to have a sufficient balance.






\paragraph{POW}

To Be Done



\paragraph{POS}


To Be Done

\paragraph{Delegated POS}

Delegated Proof of Stake (DPoS) is a robust and flexible blockchain consensus mechanism invented by Larimer~\cite{DPOS14} in 2014, which leverages the voting power of the stakeholder to resolve consensus issue in a fair and democratic manner.


DPoS was first applied by Larimer to power the blockchain project BitShares~\cite{BitShares} and further refined in his subsequent projects Steem \cite{Steem} and EOS~\cite{EOS}. Other
blockchain projects, such as Ark~\cite{Ark}, Lisk~\cite{Lisk}, Tezos~\cite{Tezos}, etc., also adopted a similar DPoS framework with certain feature changes.



\paragraph{Byzantine Agreement}

To Be Done



\paragraph{Post-Quantum Signatures.}
Perhaps the oldest signature scheme with post-quantum security is one-time Lamport signatures~\cite{Lamport79}, built using hash functions. As Grover's quantum search algorithm can invert any black-box function [52] with a quadratic speed-up over classical algorithms, one has to double the bit size of the hash function's domain, but still requires no additional assumptions to provably achieve post-quantum security.

Combined with Merkle-trees, this approach yields \emph{stateful} signatures for any polynomial number of messages [71], where the state ensures that a one-time signature key from the tree is not reused. By making the tree very large, and randomly selecting a key from it (cf. [47]), along with
%other optimizations yield practical stateless hash-based signatures [17].



















%
%%%%%%%%%%%%55
%\begin{table*}[t!]%[ht]
%\begin{center}
%\begin{threeparttable}
%%\vspace{-0.6mm}
%\vspace{10pt}
%\caption{Blockchain Consensus Classification}\label{table:XXXX}
%%\resizebox{\textwidth}{15mm}{
%%r l l l l
%\begin{tabular}{c @{\quad}l  }
%\hline\rule{0pt}{12pt} %\toprule
%  Consensus & Schemes \\
%\hline \hline\rule{0pt}{12pt} %\midrule
%POW & Bitcoin Backbone~\cite{EC:GarKialeo15}  \\
%POS &  Ouroboros~\cite{C:KRDO17}, Snow white~\cite{EPRINT:BenPasShi16}, Ouroboros~Praos~\cite{EC:DGKR18}\\
%Delegated POS & \\
%Proof of Burn & \\
%Byzantine & Ouroboros-BFT~\cite{EPRINT:KiaRus18} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\hline
%%\end{longtable}
%\end{tabular}
%%}
%
%\vspace{1ex}
%
%\centering
%\begin{tablenotes}
%        \footnotesize
%\begin{minipage}{0.4\textwidth}%{2in}
%    %\begin{itemize}
%    \item[-] Pratical Byzantine fault tolerant mechanism.
%    %\end{itemize}
%  \end{minipage}%
%%\hspace*{17mm}
%  \begin{minipage}{0.4\textwidth}%{2in}
%     %\begin{itemize}
% \item [-] C: check;
%    %\end{itemize}
%\end{minipage}
%\vspace{1ex}
%\item[*] We remark that XXXX in Table~\ref{table:XXXXX}.
%\end{tablenotes}
%\end{threeparttable}
%
%\end{center}
%\end{table*}
%%\vspace{-5pt}






\subsubsection{Signature Schemes}



\paragraph{Boneh-Eskandarian-Fisch Signature Scheme~(CT-RSA 2019)}   EPID signature~\cite{CTRSA:BonEskFis19} \etc,
EPID signatures are used extensively in real-world systems for hardware enclave attestation. As such, there is a strong interest in making these schemes post-quantum secure. In this paper, we initiate the study of EPID signature schemes built only from symmetric primitives, such as hash functions and PRFs. We present two constructions in the random oracle model. The first is a scheme satisfying the EPID signature syntax and security definitions needed for private hardware attestation used in Intel's SGX. The second achieves significantly shorter signatures for many applications, including the use case of remote hardware attestation. While our EPID signatures for attestation are longer than standard post-quantum signatures, they are short enough for applications where the data being signed is large, such as analytics on large private data sets, or streaming media to a trusted display. We evaluate several instantiations of our schemes so that the costs and benefits of these constructions are clear. Along the way, we also give improvements to the zero-knowledge Merkle inclusion proofs of Derler et al. (2017).




\paragraph{\href{https://sphincs.cr.yp.to/index.html}{SPHINCS}: practical stateless hash-based signatures}

such as SPHINCS\footnote{https://sphincs.cr.yp.to/papers.html}~\cite{EC:BHHLNPS15},


SPHINCS-256 is a high-security post-quantum stateless hash-based signature scheme that signs hundreds of messages per second on a modern 4-core 3.5GHz Intel CPU. Signatures are 41 KB, public keys are 1 KB, and private keys are 1 KB. SPHINCS-256 is designed to provide long-term 2128 security even against attackers equipped with quantum computers. Unlike most hash-based signature schemes, SPHINCS-256 is stateless, allowing it to be a drop-in replacement for current signature schemes.



\paragraph{\href{https://sphincs.org/index.html}{SPHINCS$^+$}}



SPHINCS$^{+}$\footnote{https://sphincs.org/resources.html}~\cite{SPHINCS+},





\paragraph{Jonathan-Kolesnikov-Wang Signature Scheme~(CCS2018)}

Following the research line, Jonathan, Kolesnikov, and Wang proposed a new post-quantum signature scheme using the improved non-interactive zero knowledge~\cite{CCS:JonKolWan18}.


\end{comment}


==> header/Packages.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex

\usepackage[utf8]{inputenc} % Allows the usage of non-english characters
%\usepackage{times} % Use the Times font
\usepackage{graphicx} % Allows including images
\usepackage{booktabs} % Allows the use of \toprule, \midrule and \bottomrule in tables
\usepackage{framed}  %文字加边框
\newcommand{\structureopacity}{0.75} % Opacity (transparency) for the structure elements (boxes and circles)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 自定义补充 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\useinnertheme[shadow]{rounded} % 对 box 的设置: 圆角、有阴影.

%\usefonttheme{serif}  % 字体. 个人偏好有轮廓的字体. 去掉这个设置编译, 就看到不同了.
%\setbeamertemplate{footline}[frame number]%%(自己添加)导言中加上，自动添加页码
%\setbeamertemplate{navigation symbols}{}   %% 去掉页面下方默认的导航条.


%\def\hilite<#1>{\temporal<#1>{\color{blue!35}}{\color{magenta}}{\color{blue!75}}}
%% 自定义命令, 源自 beamer_guide. item 逐步显示时, 使已经出现的item、正在显示的item、将要出现的item 呈现不同颜色.

%\newcolumntype{H}{>{\columncolor{blue!20}}c!{\vrule}}
%\newcolumntype{H}{>{\columncolor{blue!20}}c}  %% 表格设置
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 自定义补充 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{graphicx}
\usepackage{subfig}
%\usepackage{indentrst} %%%%%%%%%%%%补充，段落段首缩进
%\usepackage{bm} %%%%%%%%%%%%%%%%%%%%%补充
%\usepackage{amsfonts} %%%%%%%%%%%%%%%%%% 补充，数学
%\usepackage{subfigure} %%图形或表格并排排列
\usepackage{xmpmulti}  %%支持文中的 \multiinclude 等命令, 使 mp 文件逐帧出现. 具体讨论见 beamer 手册.
\usepackage{colortbl,dcolumn}     %% 彩色表格

\usepackage{fancyhdr}



\usepackage{wallpaper}
%\setbeamertemplate{background}{\includegraphics[height=\paperheight]{bg}}

\usepackage{CJK}
%\usepackage{xmpmulti}
%\usepackage[utf8]{inputenc} % Allows the usage of non-english characters
\usepackage[all]{background}
\usepackage{draftwatermark}
\SetWatermarkScale{5}%设置水印的显示大小
\renewcommand{\raggedright}{\leftskip=0pt \rightskip=0pt plus 0cm}
\raggedright %% 中文对齐
\def\hilite<#1>{\temporal<#1>{\color{blue!35}}{\color{magenta}}{\color{blue!75}}}
%% 自定义命令, 源自 beamer_guide. item 逐步显示时, 使已经出现的item、正在显示的item、将要出现的item 呈现不同颜色.
%\renewcommand{\labelitemii}{$\bullet$}%%%%\renewcommand{\labelitemi}{$\bullet$} 注意这个和上面的不一样，上面是 \labelitemii（最后是两个 i）
\usepackage{color}
\usepackage{xcolor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{thmtools}
%\usepackage{pgfplots}
\usepackage{tikz-3dplot}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{fit,calc,positioning,decorations.pathreplacing,matrix}
\usetikzlibrary{patterns,snakes}
\usepackage{calc}
\usepackage{color}
\usepackage{tikz}
\usepackage{hyperref}
%\hypersetup{pdfpagemode=FullScreen}
\usepackage{ifthen}
\usepackage{animate}
\newcounter{angle}
\setcounter{angle}{0}
%\usepackage[latin1]{inputenc}
%\usepackage{pgfplots}
%\usetikzlibrary{arrows.meta}
\usetikzlibrary{arrows, decorations.markings}


%%%%%%%%%
%\usepackage{mathtools}
\usepackage{amsmath,amssymb,amsfonts}
%\usepackage{mathtools}

\usepackage{xspace}

% if mathtools doesn't work, adapting the following method.
\usepackage{mleftright,xparse}

\NewDocumentCommand\xDeclarePairedDelimiter{mmm}
 {%
  \NewDocumentCommand#1{som}{%
   \IfNoValueTF{##2}
    {\IfBooleanTF{##1}{#2##3#3}{\mleft#2##3\mright#3}}
    {\mathopen{##2#2}##3\mathclose{##2#3}}%
  }%
 }
%\xDeclarePairedDelimiter{\set}{\lbrace}{\rbrace}
\xDeclarePairedDelimiter{\inner}{\langle}{\rangle}


\usepackage{mathtools}
\usepackage{etoolbox}


\DeclarePairedDelimiter{\avg}{\langle}{\rangle}


\usepackage{protocolj,arydshln}




==> header/SlidesHeader.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%重定义字体、字号命令 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\songti}{\CJKfamily{song}}        % 宋体
\newcommand{\fangsong}{\CJKfamily{fs}}        % 仿宋体
\newcommand{\kaishu}{\CJKfamily{kai}}         % 楷体
\newcommand{\heiti}{\CJKfamily{hei}}          % 黑体
\newcommand{\lishu}{\CJKfamily{li}}           % 隶书
\newcommand{\youyuang}{\CJKfamily{you}}       % 幼圆
\newcommand{\sihao}{\fontsize{14pt}{\baselineskip}\selectfont}      % 字号设置
\newcommand{\xiaosihao}{\fontsize{12pt}{\baselineskip}\selectfont}  % 字号设置
\newcommand{\wuhao}{\fontsize{10.5pt}{\baselineskip}\selectfont}    % 字号设置
\newcommand{\xiaowuhao}{\fontsize{9pt}{\baselineskip}\selectfont}   % 字号设置
\newcommand{\liuhao}{\fontsize{7.875pt}{\baselineskip}\selectfont}  % 字号设置
\newcommand{\qihao}{\fontsize{5.25pt}{\baselineskip}\selectfont}    % 字号设置
%---------------------------------------------------------------------------------------------------


\renewcommand\figurename{\rm Figure}
\renewcommand\tablename{\bf Table}
%%---------------------------------------------------------------------------------------------------










\newcommand{\coin}{\mathsf{coin}}
%\newcommand{\CPA}{\mathsf{CPA}}
%\newcommand{\CCA}{\mathsf{CCA}}
\newcommand{\GAME}{\mathsf{Game}}
\newcommand{\DDH}{\mathsf{DDH}}
\newcommand{\sfH}{\mathsf{H}}
%%%%%%%%%%%%%%%
% End Trapdoor function
%%%%%%%%%%%%%%%


\newcommand{\BB}{\mathbf{B}}
%\newcommand{\b}{\mathbf{b}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Diffie-Hellman
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\DifHel}{\mathsf{DH}}
%\newcommand{\DDH}{\mathsf{DDH}}
\newcommand{\CDH}{\mathsf{CDH}}
\newcommand{\RH}{\mathsf{RH}}
\newcommand{\Rk}{\mathsf{Rk}}
\newcommand{\RP}{\mathsf{RP}}
\newcommand{\DRP}{\mathsf{DRP}}
\newcommand{\LWEE}{\mathsf{LWEE}}




%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\footnotemark{}
\renewcommand\footnoterule{}












==> header/header-Fixed-theorem.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex

%%% THEOREM COMMANDS

%\theoremstyle{plain}            % following are "theorem" style
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{openproblem}[theorem]{Open Problem}

%\theoremstyle{definition}       % following are def style
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{protocol}[theorem]{Protocol}

%\theoremstyle{remark}           % following are remark style
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
%\newtheorem{note}[theorem]{Note}
%\newtheorem{exercise}[theorem]{Exercise}


%\theoremstyle{assumption}       %
\newtheorem{assumption}[theorem]{Assumption}


% equation numbering style
\numberwithin{equation}{section}


==> header/header-MAG.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex

\newcommand{\Const}{\ensuremath{\mathsf{Const}}\xspace}
\newcommand{\ConstEval}{\ensuremath{\mathsf{ConstEval}}\xspace}
\newcommand{\ReEnc}{\ensuremath{\mathsf{ReEnc}}\xspace}
\newcommand{\ReKeyGen}{\ensuremath{\mathsf{ReKeyGen}}\xspace}


\newcommand{\CPRF}{\ensuremath{\mathsf{CPRF}}\xspace}
% counter
\newcommand{\ctr}{\ensuremath{\mathsf{ctr}}\xspace}

\newcommand{\kkey}{\ensuremath{k}\xspace}
\newcommand{\kkeyi}{\ensuremath{{k^{i}}}\xspace}
\newcommand{\kkeyj}{\ensuremath{{k^{j}}}\xspace}
\newcommand{\kkeyctr}{\ensuremath{{k^{\ctr}}}\xspace}

\newcommand{\bit}{\ensuremath{b}\xspace}
\newcommand{\ctij}{\ensuremath{c}^{(i\to j)}\xspace}
\newcommand{\rkij}{\ensuremath{\rk}^{(i\to j)}\xspace}


% constrained PRF
\newcommand{\cPRF}{\ensuremath{\calF}\xspace}
% symmetric encryption
\newcommand{\Sym}{{\textsf{Sym}}\xspace} % symmetric encryption
%\newcommand{\PRE}{{\textsf{PRE}}\xspace}
% symmetric encryption
%public parameters
\newcommand{\pubp}{\ensuremath{\mathsf{pparams}}\xspace}
% PRF key
\newcommand{\prfkey}{\ensuremath{\mathsf{key}_{\mathrm{prf}}}\xspace}
\newcommand{\prfrekey}{\ensuremath{\mathsf{rekey}_{\mathrm{prf}}}\xspace}
\newcommand{\cprfrekey}{\ensuremath{ \mathsf{rekey}_{\mathrm{cprf}}  }\xspace}
\newcommand{\cprfrekeyF}[1]{\ensuremath{\mathsf{rekey}^{#1}_{\mathrm{cprf}}}\xspace}

\newcommand{\prfkeyctr}{\ensuremath{\mathsf{key}_{\mathrm{prf}}^{\ctr}}\xspace}
% constrained PRF key
\newcommand{\cprfkey}{\ensuremath{\mathsf{key}_{\mathrm{cprf}}}\xspace}
%% constrained PRF master secret key
%\newcommand{\cprfmsk}{\ensuremath{\mathsf{msk}_{\mathrm{cprf}}}\xspace}
\newcommand{\cprfsk}{\ensuremath{\mathsf{sk}_{\mathrm{cprf}}}\xspace}


\newcommand{\cprfkeyC}{\ensuremath{\cprfkey^{C_{f,\veck}}}\xspace}


%
\newcommand{\cprfmsk}{\ensuremath{\mathsf{msk}_{\mathrm{cprf}}}\xspace}
%
\newcommand{\cprfmskF}[1]{\ensuremath{\mathsf{msk}^{#1}_{\mathrm{cprf}}}\xspace}

% random key
\newcommand{\randkey}{\ensuremath{\kappa_{\mathrm{rnd}}}\xspace}

% PRF randomness
\newcommand{\prfrand}{\ensuremath{r_{\mathrm{prf}}}\xspace}
% constrained PRF randomness
\newcommand{\cprfrand}{\ensuremath{r_{\mathrm{cprf}}}\xspace}

% circuit class
\newcommand{\circuitset}{\ensuremath{\calC}\xspace}

\newcommand{\msgx}{\ensuremath{x}\xspace}

\newcommand{\domainX}{\ensuremath{\calX}\xspace}
\newcommand{\rangY}{\ensuremath{\calY}\xspace}


%%% functional encryption
\newcommand{\femsk}{\ensuremath{\mathsf{msk}}\xspace}

\newcommand{\fesk}{\ensuremath{\mathsf{sk}_{\mathrm{FE}}}\xspace}

\newcommand{\fect}{\ensuremath{\mathsf{ct}_{\mathrm{FE}}}\xspace} 




%% Attribute based encryption

%\newcommand{\ABE}{\ensuremath{\mathsf{ABE}}\xspace}
\newcommand{\CPABE}{\ensuremath{\mathsf{CPABE}}\xspace}
\newcommand{\KPABE}{\ensuremath{\mathsf{KPABE}}\xspace}

% attribute set
\newcommand{\attset}{\ensuremath{\mathbb{A}}\xspace}

% ACCESS  policy
\newcommand{\acsp}{\ensuremath{\Gamma}\xspace}

\newcommand{\abemsk}{\ensuremath{\mathsf{msk}}\xspace}
\newcommand{\cpabemsk}{\ensuremath{\mathsf{msk}}\xspace}

\newcommand{\abesk}{\ensuremath{\mathsf{sk}}\xspace}
\newcommand{\abesks}{\ensuremath{\mathsf{sk}_{\attset}}\xspace}
\newcommand{\cpabesk}{\ensuremath{\mathsf{sk}_{\attset}}\xspace}
\newcommand{\kpabesk}{\ensuremath{\mathsf{sk}_{\acsp}}\xspace}

% ciphertext 
\newcommand{\abect}{\ensuremath{\mathsf{ct}}\xspace}
\newcommand{\abectp}{\ensuremath{\mathsf{ct}_{\acsp}}\xspace}
\newcommand{\cpabect}{\ensuremath{\mathsf{ct}_{\acsp}}\xspace}
\newcommand{\kpabect}{\ensuremath{\mathsf{ct}_{\attset}}\xspace}


% LW
\newcommand{\LW}{\ensuremath{\mathsf{LW}}\xspace}
% master key
\newcommand{\cpabpmsk}{\ensuremath{\mathsf{msk}}\xspace}
\newcommand{\abpsk}{\ensuremath{\mathsf{sk}}\xspace}
% secret key
\newcommand{\cpabpsk}{\ensuremath{\mathsf{sk}_{\attset}}\xspace}
% ciphertext
\newcommand{\cpabpct}{\ensuremath{\mathsf{ct}_{\acsp}}\xspace}
% re-encryption ciphertext
\newcommand{\cpabprect}{\ensuremath{\mathsf{rect}_{\acsp}}\xspace}
% re-encryption key
\newcommand{\cpabprk}{\ensuremath{\mathsf{rk}_{(\attset,\acsp)}}\xspace}

==> header/header-diy-PAKE.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex
% MSG
\newcommand{\MSG}{\ensuremath{M}\xspace}
%Smooth Projective Hash Functions
\newcommand{\SPHF}{\ensuremath{\mathsf{SPHF}}\xspace}
% Cramer and Shoup
\newcommand{\CSSPHF}{\ensuremath{\mathsf{CS}\text{-}\mathsf{SPHF}}\xspace}
% Gennaro and Lindell
\newcommand{\GL}{\ensuremath{\mathsf{GL}}\xspace}
\newcommand{\GLSPHF}{\ensuremath{\mathsf{GL}\text{-}\mathsf{SPHF}}\xspace}
% Katz and Vaikuntanathan
\newcommand{\KVSPHF}{\ensuremath{\mathsf{KV}\text{-}\mathsf{SPHF}}\xspace}





%%% hash proof system




\newcommand{\hashvalue}{\ensuremath{\mathsf{h}}}
\newcommand{\projvalue}{\ensuremath{\mathsf{p}}}



% hashing key
\newcommand{\hashkey}{\ensuremath{\key{hk}}\xspace}
%\newcommand{\hashkey}{\ensuremath{\key{hk}}\xspace}
% projection hashing key
\newcommand{\projkey}{\ensuremath{\key{ph}}\xspace}
\newcommand{\projhashkey}{\ensuremath{\projkey}\xspace}
% hash value
\newcommand{\hashSPHF}{\ensuremath{\key{H}}\xspace}
% projection hash value
\newcommand{\projhashSPHF}{\ensuremath{\key{P}}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% hashing key vector
\newcommand{\vechashkey}{\ensuremath{\mathbf{h}}\xspace}
% project hashing key vector
\newcommand{\vecprojkey}{\ensuremath{\mathbf{p}}\xspace}
% hash value vector
\newcommand{\vechashvalue}{\ensuremath{\mathbf{h}}\xspace}
% projection hash value vector
\newcommand{\vecprojhashvalue}{\ensuremath{\mathbf{h}}\xspace}
%%% algorithm
% HashKG
\newcommand{\HashKG}{\ensuremath{\mathsf{HashKG}}\xspace}
% ProjKG
\newcommand{\ProjKG}{\ensuremath{\mathsf{ProjKG}}\xspace}
% Hash
\newcommand{\Hash}{\ensuremath{\mathsf{Hash}}\xspace}
% ProjHash
\newcommand{\ProjHash}{\ensuremath{\mathsf{ProjHash}}\xspace}
\newcommand{\Proj}{\ensuremath{\mathsf{Proj}}\xspace}
%%%%%%%%%%
% witness
\newcommand{\witness}{\ensuremath{w}\xspace}
% vector witness
\newcommand{\vecwitness}{\ensuremath{\mathbf{s}}\xspace}
% \Keyspace
\newcommand{\Keyspace}{\ensuremath{\mathbb{K}}\xspace}
% \Ctspace
\newcommand{\Ctspace}{\ensuremath{\mathbb{C}}\xspace}
% \Projspace
\newcommand{\Projspace}{\ensuremath{\mathbb{P}}\xspace}
%% user set
\newcommand{\setuser}{\ensuremath{\mathsf{U}}\xspace}
%% user
\newcommand{\user}{\ensuremath{U}\xspace}
%% password
\newcommand{\pw}{\ensuremath{pw}\xspace}
%% password function
\newcommand{\pwfunc}[2]{\ensuremath{pw_{{#1},{#2}}}\xspace}
%% user instance
\newcommand{\userinst}[1]{\ensuremath{\Pi_{\user}^{#1}}\xspace}
\newcommand{\userinstC}{\ensuremath{{\Pi_{\user_C}^{i}}}\xspace}
\newcommand{\userinstS}{\ensuremath{{\Pi_{\user_S}^{j}}}\xspace}
%% session id
\newcommand{\sid}{\ensuremath{\mathsf{sid}}\xspace}
\newcommand{\sidfunc}[1]{\ensuremath{\mathsf{sid}_{\user}^{#1}}\xspace}
\newcommand{\sidU}{\ensuremath{\mathsf{sid}_{\user}^{i}}\xspace}
\newcommand{\sidC}{\ensuremath{\mathsf{sid}_{\user_C}^{i}}\xspace}
\newcommand{\sidS}{\ensuremath{\mathsf{sid}_{\user_S}^{j}}\xspace}
%% partner id
\newcommand{\pid}{\ensuremath{\mathsf{pid}}\xspace}
\newcommand{\pidfunc}[1]{\ensuremath{\mathsf{pid}_{\user}^{#1}}\xspace}
\newcommand{\pidU}{\ensuremath{\mathsf{pid}_{\user}^{i}}\xspace}
\newcommand{\pidC}{\ensuremath{\mathsf{pid}_{\user_C}^{i}}\xspace}
\newcommand{\pidS}{\ensuremath{\mathsf{pid}_{\user_S}^{j}}\xspace}

%% session key
\newcommand{\skey}{\ensuremath{\mathsf{skey}}\xspace}
\newcommand{\skeyfunc}[1]{\ensuremath{\mathsf{skey}_{\user}^{#1}}\xspace}
\newcommand{\skeyU}{\ensuremath{\mathsf{skey}_{\user}^{i}}\xspace}
\newcommand{\skeyC}{\ensuremath{\mathsf{skey}_{\user_C}^{i}}\xspace}
\newcommand{\skeyS}{\ensuremath{\mathsf{skey}_{\user_S}^{j}}\xspace}


%% acceptance
\newcommand{\acc}{\ensuremath{\mathsf{acc}}\xspace}
\newcommand{\accfunc}[1]{\ensuremath{\mathsf{acc}_{\user}^{#1}}\xspace}
\newcommand{\accU}{\ensuremath{\mathsf{acc}_{\user}^{i}}\xspace}
\newcommand{\accC}{\ensuremath{\mathsf{acc}_{\user_C}^{i}}\xspace}
\newcommand{\accS}{\ensuremath{\mathsf{acc}_{\user_S}^{j}}\xspace}
\newcommand{\LSB}{\ensuremath{\mathsf{LSB}}\xspace}
%% termination,
\newcommand{\term}{\ensuremath{\mathsf{term}}\xspace}
\newcommand{\termfunc}[1]{\ensuremath{\mathsf{term}_{\user}^{#1}}\xspace}
\newcommand{\termU}{\ensuremath{\mathsf{term}_{\user}^{i}}\xspace}
\newcommand{\termC}{\ensuremath{\mathsf{term}_{\user_C}^{i}}\xspace}
\newcommand{\termS}{\ensuremath{\mathsf{term}_{\user_S}^{j}}\xspace}

%% state
\newcommand{\state}{\ensuremath{\mathsf{state}}\xspace}
\newcommand{\statefunc}[1]{\ensuremath{\mathsf{state}_{\user}^{#1}}\xspace}
\newcommand{\stateU}{\ensuremath{\mathsf{state}_{\user}^{i}}\xspace}
\newcommand{\stateC}{\ensuremath{\mathsf{state}_{\user_C}^{i}}\xspace}
\newcommand{\stateS}{\ensuremath{\mathsf{state}_{\user_S}^{j}}\xspace}

%% used
\newcommand{\used}{\ensuremath{\mathsf{used}}\xspace}
\newcommand{\usedfunc}[1]{\ensuremath{\mathsf{used}_{\user}^{#1}}\xspace}
\newcommand{\usedU}{\ensuremath{\mathsf{used}_{\user}^{i}}\xspace}
\newcommand{\usedC}{\ensuremath{\mathsf{used}_{\user_C}^{i}}\xspace}
\newcommand{\usedS}{\ensuremath{\mathsf{used}_{\user_S}^{j}}\xspace}

%% the following oracles
%% send oracle
\newcommand{\Send}{\ensuremath{\mathsf{Send}}\xspace}
\newcommand{\Sendfixed}{\ensuremath{\mathsf{Send}(\user,i,\msg)}\xspace}
\newcommand{\Sendorac}[1]{\ensuremath{\mathsf{Send}(#1)}\xspace} %% send %% execute oracle
\newcommand{\Execute}{\ensuremath{\mathsf{Execute}}\xspace}
\newcommand{\Executefixed}{\ensuremath{\mathsf{Execute}(\user_i,i,\user_j,j)}\xspace}
\newcommand{\Executeorac}[1]{\ensuremath{\mathsf{Execute}(#1)}\xspace}

%% Reveal oracle
\newcommand{\Reveal}{\ensuremath{\mathsf{Reveal}}\xspace}
\newcommand{\Revealfixed}{\ensuremath{\mathsf{Reveal}(\user_i,i)}\xspace}
\newcommand{\Revealorac}[1]{\ensuremath{\mathsf{Reveal}(#1)}\xspace}

%% Test oracle
\newcommand{\Test}{\ensuremath{\mathsf{Test}}\xspace}
\newcommand{\Testfixed}{\ensuremath{\mathsf{Test}(\user_i,i)}\xspace}
\newcommand{\Testorac}[1]{\ensuremath{\mathsf{Test}(#1)}\xspace}
%% PAKE
%\newcommand{\PAKE}{\ensuremath{\textsf{PAKE}}\xspace}
%% word
\newcommand{\word}{\ensuremath{W}\xspace}
%% domain
\newcommand{\domain}{\ensuremath{X}\xspace}
%% point
\newcommand{\point}{\ensuremath{x}\xspace}
%% adversary function
\newcommand{\advanfunc}[1]{\ensuremath{\advan_{#1,\Pi}(\secp)}\xspace}
%% ElGamal
\newcommand{\ElGamal}{\ensuremath{\textsf{ElGamal}}\xspace}
%% $\EGSPHF$
\newcommand{\EGSPHF}{\ensuremath{\textsf{EG}\text{-}\SPHF}\xspace}
%% $\CSSPHF$
%\newcommand{\CSSPHF}{\ensuremath{\textsf{CS}\text{-}\SPHF}\xspace}
%% Miccianio-Peikert Scheme
\newcommand{\MP}{\ensuremath{\textsf{MP}}\xspace}
%% Cramer-Shoup  Scheme
\newcommand{\CS}{\ensuremath{\textsf{CS}}\xspace}
%% $\MPSPHF$
\newcommand{\MPSPHF}{\ensuremath{\textsf{MP}\text{-}\SPHF}\xspace}
%% $\RSPHF$
\newcommand{\RSPHF}{\ensuremath{\mathsf{Reg}\text{-}\SPHF}\xspace}



%-------------------------------


%% password based authenticated key exchange
\newcommand{\PAKE}{\ensuremath{\mathsf{PAKE}}\xspace}
\newcommand{\vPAKE}{\ensuremath{\mathsf{vPAKE}}\xspace}


% password hashing
%-verifier
\newcommand{\ver}{\ensuremath{\mathsf{ver}}\xspace}
%-password length
\newcommand{\pwdlength}{\ensuremath{\ell}\xspace}
%-password hashing algorithms
\newcommand{\PreSalt}{\ensuremath{\mathsf{PreSalt}}\xspace}
\newcommand{\PreHash}{\ensuremath{\mathsf{PreHash}}\xspace} \newcommand{\PHash}{\ensuremath{\mathsf{PHash}}\xspace}
\newcommand{\Salt}{\ensuremath{\mathsf{Salt}}\xspace}
\newcommand{\Checkable}{\ensuremath{\mathsf{Checkable}}\xspace}

%-salt
\newcommand{\salt}{\ensuremath{s}\xspace}
%-pre salt
\newcommand{\presalt}{\ensuremath{\bar{s}}\xspace}
%- salt space
\newcommand{\saltset}{\ensuremath{\mathbb{S}_H}\xspace}
%- pre salt space
\newcommand{\psaltset}{\ensuremath{\mathbb{S}_P}\xspace}
% pre-hash value
\newcommand{\phvalue}{\ensuremath{{\bar{y}}}\xspace}
% hash value
\newcommand{\hvalue}{\ensuremath{{y}}\xspace}




%-- PIN
\newcommand{\PIN}{\ensuremath{\mathsf{PIN}}\xspace}

%device
\newcommand{\devc}{{{\textsf{D}}}\xspace}
%%% user

\newcommand{\usr}{\textsf{U}\xspace}
\newcommand{\server}{\textsf{S}\xspace}
%\terminal
\newcommand{\trml}{\textsf{T}\xspace}
%\newcommand{\QR}{\textsf{QR}\xspace}





%%KG
\newcommand{\KG}{\textsf{KG}\xspace}

%% channel capacity

\newcommand{\ccpt}{\ensuremath{t}\xspace}

\newcommand{\comHash}{\ensuremath{\mathsf{Com}_H}\xspace}

\newcommand{\oprfHash}{\ensuremath{\mathsf{H}_{\mathrm{oprf}}}\xspace}


%%% message sent from user to device
\newcommand{\msgSAS}{\ensuremath{\mathsf{M}_{\usr\devc}}\xspace}




%%% random string
\newcommand{\rstr}{\ensuremath{\mathrm{str}}\xspace}



%% string length

\newcommand{\rstrlen}{\ensuremath{t}\xspace}


% open commentment parameter

\newcommand{\comprm}{\ensuremath{d}\xspace}

% length of commitment

\newcommand{\complen}{\ensuremath{\kappa}\xspace}
% common key
\newcommand{\comkey}{\ensuremath{\mathsf{key}}\xspace}

% commitment outputs

\newcommand{\com}{\ensuremath{\mathsf{com}}\xspace}
% checksum
\newcommand{\checksum}{\ensuremath{\mathsf{checksum}}\xspace}

%% one-way transformation


\newcommand{\tft}{\ensuremath{{\mathsf{v}}}\xspace}







%%%%%%%%%%%%%%%%%%%
\newcommand{\ellq}{\ensuremath{\ell_q}\xspace}
\newcommand{\bitlength}{\ensuremath{\ell_q}\xspace}
% distribution
\newcommand{\distb}[2]{\ensuremath{\calD^{#1}_{#2}}\xspace}
% label
\newcommand{\labell}{\ensuremath{\mathsf{label}}\xspace}
\newcommand{\labellu}{\ensuremath{u}\xspace}
% label space
\newcommand{\labelspace}{\ensuremath{\calU}\xspace}
% encode
\newcommand{\encode}{\ensuremath{\mathsf{encode}}\xspace}
% decode
\newcommand{\decode}{\ensuremath{\mathsf{decode}}\xspace}
% \Invert algorithm
\newcommand{\Invert}{\ensuremath{\mathsf{Invert}}\xspace}
% Katz-Vaikuntanathan (KV)
\newcommand{\KV}{\ensuremath{\textsf{KV}}\xspace}
% LWE assumption
\newcommand{\LWEp}{\ensuremath{\LWE_{n,m,q,\chi}}\xspace}
% hash function H and G
\newcommand{\hashH}{\ensuremath{H}\xspace}
\newcommand{\hashG}{\ensuremath{G}\xspace}
% hash value of H
\newcommand{\hashh}{\ensuremath{\Theta}\xspace}% already done
\newcommand{\barhashh}{\ensuremath{\bar{\Theta}}\xspace}% already done
\newcommand{\hashg}{\ensuremath{g}\xspace}% already done
%% label
\newcommand{\Label}{\ensuremath{\ell}\xspace}% already done
\newcommand{\barLabel}{\ensuremath{\bar{\ell}}\xspace}% already done
%% DDH
\newcommand{\DDH}{\ensuremath{\mathsf{DDH}}\xspace}
%\newcommand{\DH}{\ensuremath{\mathsf{DH}}\xspace}
%% query
\newcommand{\query}{\ensuremath{q}\xspace}
% password
%\newcommand{\pwd}{\ensuremath{\mathsf{pwd}}\xspace}
% common key
%\newcommand{\comkey}{\ensuremath{\mathsf{key}}\xspace}
%%% Experiment
%\newcommand{\Expt}{\ensuremath{\mathsf{Expt.}}\xspace}

%%% Adversary
\newcommand{\ADV}[1]{\ensuremath{\mathsf{Adv}_{\calA}^{\Expt{#1}}(\secp)}\xspace}
%%% CPA Enc
\newcommand{\CPAEnc}{\ensuremath{\mathsf{Enc}^{cpa}}\xspace}
%%% CCA Label Enc
\newcommand{\CCAEnc}{\ensuremath{\mathsf{Enc}^{label}}\xspace}
%%% ECC
\newcommand{\ECC}{\ensuremath{\mathsf{ECC}}\xspace}
\newcommand{\invECC}{\ensuremath{\mathsf{ECC}^{-1}}\xspace}
%%% Hash
\newcommand{\HASH}{\ensuremath{\mathsf{HASH}}\xspace}
%%%
\newcommand{\BDDSolve}{\ensuremath{\mathsf{BBDSolve}}\xspace}
%%%
%\newcommand{\Invert}{\ensuremath{\mathsf{Invert}}\xspace}
%%% Hamming distance
\newcommand{\HD}{\ensuremath{\mathsf{HD}}\xspace}
%%% NULL
\newcommand{\NULL}{\ensuremath{\textrm{NULL}}\xspace}
%%% True
\newcommand{\TRUE}{\ensuremath{\textrm{TRUE}}\xspace}
%%%
\newcommand{\Sgn}{\ensuremath{\mathsf{Sgn}}\xspace}
\newcommand{\Sign}{\ensuremath{\mathsf{Sign}}\xspace}
\newcommand{\Vrfy}{\ensuremath{\mathsf{Vrfy}}\xspace}
%%%
\newcommand{\Labellu}{\ensuremath{\theta}\xspace}

%\newcommand{\userinstS}{\ensuremath{S}\xspace}
%\newcommand{\userinstC}{\ensuremath{C}\xspace}



\newcommand{\pwd}{\ensuremath{\textsf{pwd}}\xspace}
\newcommand{\rwd}{\ensuremath{\textsf{rwd}}\xspace}
%\newcommand{\rand}{\ensuremath{{r}}\xspace}
\newcommand{\oprfkey}{\ensuremath{{k}}\xspace}
% Group
\newcommand{\Group}{\ensuremath{{\G}}\xspace}
% order
\newcommand{\order}{\ensuremath{{r}}\xspace}
% generator
\newcommand{\grt}{\ensuremath{{g}}\xspace}




%%%%%


%\newcommand{\Gen}{\ensuremath{{\mathsf{Gen}}}\xspace}
\newcommand{\Rep}{\ensuremath{{\mathsf{Rep}}}\xspace}

%% template

\newcommand{\temp}{\ensuremath{{\mathsf{w}}}\xspace}
\newcommand{\Temp}{\ensuremath{{\mathcal{T}}}\xspace}
% extracted string
\newcommand{\extstr}{\ensuremath{{\mathsf{R}}}\xspace}
% public string
\newcommand{\pubstr}{\ensuremath{{\mathsf{P}}}\xspace}


% uniform string
\newcommand{\unistr}{\ensuremath{{\mathsf{U}_{\ell}}}\xspace}

% statistical distance
\newcommand{\SD}{\ensuremath{{\mathsf{SD}}}\xspace}

% distance
%\newcommand{\dist}{\ensuremath{{\mathsf{dist}}}\xspace}




% biometric distribution

%\newcommand{\biodistb}{\ensuremath{\calD_{B(C)}}\xspace}

\newcommand{\biodistb}[1]{\ensuremath{\calD_{B(#1)}}\xspace}

%\newcommand{\algo}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\dvcdistb}[1]{\ensuremath{\calD_{\textsf{dvc}(#1)}}\xspace}
% device random number
\newcommand{\dvcrand}{\ensuremath{{\gamma}}\xspace}


% user information
\newcommand{\uinfo}{\ensuremath{{\mathsf{uinfo}}}\xspace}
% user id
\newcommand{\uid}{\ensuremath{{\mathsf{uid}}}\xspace}
% oblivious PRF
\newcommand{\OPRF}{\ensuremath{{\mathsf{OPRF}}}\xspace}
\newcommand{\oprfvalue}{\ensuremath{{\mathsf{ov}}}\xspace}

% HMAC
\newcommand{\HMAC}{\ensuremath{{\mathsf{HMAC}}}\xspace}

% Password Hashing
\newcommand{\PH}{\ensuremath{{\mathsf{PH}}}\xspace}
\newcommand{\ph}{\ensuremath{{\mathsf{ph}}}\xspace}

% Label
\newcommand{\lbl}{\ensuremath{{\ell}}\xspace}

% CHRtoINT
\newcommand{\CHRtoINT}{\ensuremath{{\mathsf{CHR2INT}}}\xspace}
% PWDtoINT
\newcommand{\PWDtoINT}{\ensuremath{{\mathsf{PWD2INT}}}\xspace}
% character
\newcommand{\cha}{\ensuremath{{c}}\xspace}
% ASCII

\newcommand{\ASCII}{\ensuremath{{\mathsf{ASCII}}}\xspace}


% Commitment salt set
\newcommand{\csaltset}{\ensuremath{{\mathbb{S}_{\com}}}\xspace}




% Abort
\newcommand{\abort}{\ensuremath{\mathsf{abort}}\xspace}

% Accept
\newcommand{\accept}{\ensuremath{\mathsf{accept}}\xspace}

%%% SMP set membership proof
\newcommand{\SMP}{\ensuremath{\mathsf{SMP}}\xspace}
%%% ZKPOK zero-knowledge proof of knowledge
\newcommand{\ZKPOK}{\ensuremath{\mathsf{ZKPOK}}\xspace}




%%% IND-PCA
\newcommand{\INDPCA}{\ensuremath{\mathsf{IND}\text{-}\mathsf{PCA}}\xspace} 

==> header/headers.tex <==
% !TEX encoding =UTF-8 Unicode
%!TEX root = ../mainVRFarxiv.tex

\newcommand{\ignore}[1]{}


%\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{corollary}{Corollary}
%\newtheorem{proposition}{Proposition}
%\newtheorem{example}{Example}
%\newtheorem{remark}{Remark}
%\newtheorem{claim}{Claim}

\newcommand{\SwitchKeyGen}{\mathsf{SwitchKeyGen}}
\newcommand{\SlotSwitch}{\mathsf{SlotSwitch}}
\newcommand{\UniEnc}{\mathsf{UniEnc}}
\newcommand{\Extend}{\mathsf{Extend}}
\newcommand{\Expand}{\mathsf{Expand}}
\newcommand{\PartDec}{\mathsf{PartDec}}
\newcommand{\FinDec}{\mathsf{FinDec}}

\newcommand{\GG}{\mathbf{G}}
\newcommand{\GGh}{\tilde{\mathbf{G}}}
\newcommand{\WW}{\mathbf{W}}
\newcommand{\MM}{\mathbf{M}}
\renewcommand{\SS}{\mathbf{S}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\PP}{\mathbf{P}}
\renewcommand{\r}{\mathbf{r}}
\newcommand{\m}{\mathbf{m}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\calV}{\mathcal{V}}



\newcommand{\negl}{\mathsf{negl}}
\newcommand{\ssk}{\mathsf{ssk}}
\newcommand{\PK}{\mathsf{PK}}
\newcommand{\CT}{\mathsf{CT}}
\newcommand{\User}{\mathsf{User}}
\newcommand{\LCP}{\mathsf{LCP}}
\newcommand{\OLCP}{\mathsf{OLCP}}
\newcommand{\w}{\mathsf{w}}

\newcommand{\C}{\mathcal{C}}

\newcommand{\Z}{{\mathbb Z}}
\newcommand{\F}{{\mathbb F}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\Q}{{\mathbb Q}}

\newcommand{\X}{{\mathcal X}}
\newcommand{\Y}{{\mathcal Y}}

\renewcommand{\b}{\mathbf{b}}
\newcommand{\e}{\mathbf{e}}
\renewcommand{\u}{\mathbf{u}}
\renewcommand{\v}{\mathbf{v}}
\renewcommand{\w}{\mathbf{w}}
\newcommand{\s}{\mathbf{s}}
\renewcommand{\t}{\mathbf{t}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\g}{\mathbf{g}}
\renewcommand{\r}{\mathbf{r}}
\newcommand{\p}{\mathbf{p}}


\renewcommand{\e}{\mathbf{e}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}


\renewcommand{\AA}{\mathbf{A}}
\newcommand{\AAb}{\bar{\mathbf{A}}}
\newcommand{\BBb}{\bar{\mathbf{B}}}
\newcommand{\BB}{\mathbf{B}}
\newcommand{\CC}{\mathbf{C}}
\newcommand{\ZZ}{\mathbf{Z}}
%\newcommand{\WW}{\mathbf{W}}
%\newcommand{\Abf}{\mathbf{A}}
\newcommand{\RR}{\mathbf{R}}
\newcommand{\RRh}{\tilde{\mathbf{R}}}
\newcommand{\XX}{\mathbf{X}}
%\newcommand{\PP}{\mathbf{PP}}
\newcommand{\UU}{\mathbf{U}}
\newcommand{\draft}[1]{}
\newcommand{\calT}{\mathcal{T}}

%%%\introduce by Edurao
\newcommand{\GSW}{\mathsf{GSW}}
\newcommand{\Reg}{\mathsf{Reg}}
\newcommand{\GPV}{\mathsf{GPV}}
%\newcommand{\MReg}{\mathsf{\pi_1}}
\newcommand{\MReg}{\mathsf{MReg}}

\newcommand{\MGPV}{\mathsf{MGPV}}
%\newcommand{\MGSW}{\mathsf{\pi_m}}
\newcommand{\MGSW}{\mathsf{MGSW}}

\newcommand{\DMGSW}{\mathsf{DMGSW}}
\newcommand{\LRMGSW}{\mathsf{LRMGSW}}
%\renewcommand{\Reg}{\mathrm{Reg05}}
%\renewcommand{\GPV}{\mathrm{GPV08}}
%\newcommand{\MWGSW}{\mathsf{MWGSW}}
%\newcommand{\MMFHE}{\mathsf{\Pi_m}}
\newcommand{\MMGSW}{\mathsf{MMGSW}}


\newcommand{\MMFHE}{\mathsf{MMFHE}}



%\newcommand{\MFHE}{\mathsf{\Pi_1}}
\newcommand{\MFHE}{\mathsf{MFHE}}

\newcommand{\Bra}{\mathsf{Bra}}

\newcommand{\KeyGen}{\mathsf{KeyGen}}
\newcommand{\SecretKeyGen}{\mathsf{SecretKeyGen}}
\newcommand{\PublicKeyGen}{\mathsf{PublicKeyGen}}
\newcommand{\Setup}{\mathsf{Setup}}
\newcommand{\SymEnc}{\mathsf{SymEnc}}
\newcommand{\Enc}{\mathsf{Enc}}
\newcommand{\Dec}{\mathsf{Dec}}
\newcommand{\bitDec}{\mathsf{bitDec}}
\newcommand{\Eval}{\mathsf{Eval}}
\newcommand{\pk}{\mathsf{pk}}
\newcommand{\sk}{\mathsf{sk}}
\newcommand{\params}{\mathsf{params}}



\newcommand{\SHE}{\mathrm{SHE}}
\newcommand{\HE}{\mathrm{HE}}
\newcommand{\LWE}{\mathsf{LWE}}
\newcommand{\SIS}{\mathsf{SIS}}
\newcommand{\SearchLWE}{\mathsf{Seacrh.LWE}}
\newcommand{\DecisionLWE}{\mathsf{Decision.LWE}}
\newcommand{\DualLWE}{\mathsf{Dual.LWE}}
\newcommand{\PrimalLWE}{\mathsf{Primal.LWE}}
\newcommand{\PrimeLWE}{\mathsf{Prime.LWE}}
\newcommand{\DualFerrLWE}{\mathsf{DualFerr.LWE}}
\newcommand{\FerrLWE}{\mathsf{Ferr.LWE}}
\newcommand{\Ferr}{\mathsf{Ferr}}
\newcommand{\NTRU}{\mathsf{NTRU}}


\newcommand{\CCA}{\mathsf{CCA}}
\newcommand{\CPA}{\mathsf{CPA}}
\newcommand{\INDCPA}{\mathsf{IND-CPA}}

\newcommand{\A}{\mathcal{A}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\D}{\mathcal{D}}

\newcommand{\PKE}{\mathsf{PKE}}
\newcommand{\FHE}{\mathsf{FHE}}
\newcommand{\NAND}{\mathsf{NAND}}
\newcommand{\Add}{\mathsf{Add}}
\newcommand{\Mult}{\mathsf{Mult}}
\newcommand{\GSWFHE}{\mathsf{GSWFHE}}


\newcommand{\PowerOftwo}{\mathsf{PowerOf2}}
\newcommand{\BitDecomp}{\mathsf{BitDecomp}}
\newcommand{\Flatten}{\mathsf{Flatten}}


\newcommand{\Abf}{\mathbf{A}}
\newcommand{\tsmall}{\mathrm{small}}
\newcommand{\error}{\mathbf{error}}
\newcommand{\Error}{\mathbf{Error}}
\newcommand{\Noise}{\mathbf{Noise}}
\newcommand{\noise}{\mathbf{noise}}


\newcommand{\final}{\mathrm{final}}
\newcommand{\diag}{\mathrm{diag}}
\renewcommand{\e}{\mathbf{e}}
\newcommand{\PPT}{\mathcal{PPT}}

